Influence Maximization in Real-World Closed Social Networks

In the last few years, many closed social networks such as WhatsAPP and WeChat have emerged to cater for people's growing demand of privacy and independence. In a closed social network, the posted content is not available to all users or senders can set limits on who can see the posted content. Under such a constraint, we study the problem of influence maximization in a closed social network. It aims to recommend users (not just the seed users) a limited number of existing friends who will help propagate the information, such that the seed users' influence spread can be maximized. We first prove that this problem is NP-hard. Then, we propose a highly effective yet efficient method to augment the diffusion network, which initially consists of seed users only. The augmentation is done by iteratively and intelligently selecting and inserting a limited number of edges from the original network. Through extensive experiments on real-world social networks including deployment into a real-world application, we demonstrate the effectiveness and efficiency of our proposed method.

==> imcsnvldb2023 copy/.git/objects/00/f0c579bb6d16d75389df652c86ff3dc5e7a185 <==
x+)JMU0µ4e040031QH,(HÍKɬÐ+I­`ñL|uiý"köÒ¦Yßlߙ½½ª.µ¢ µ(375¯¬²p§ÉÜ/E…ßE±o;pò]T¥-†Jc°Ò¸\c¡ÉmõÞ[™:ÊÜyºyò¢ J3‹RòR‹‹ÁêxuUz¼)‹e%%½a•L9«x9ª.3¯¤(?¥4¹$3?¬6´Ôþýu·SjÌqÞgõ8«6lœU››˜\"Vô]'måª	>Âß4í'%uŠ%?³Â¦(µ$#?%-¿(·4§$³ '¬áBWÜ‰}uYÒÛ33÷F½Ùœ(‡®¡83/ªüອûŊ%¼'Êf†Æ¥~_ög9L9ÔؤҔôTHˆÉ"6ZóMn8­×µ¾ñ­«±ÓVo¨ê'¢ÔœÌÜ̼ĢJ°;V/vYn2KÅwκÖI¼>"ˠJ*KRSÊó‹²ÁJMVoÙTÓïQË}Ö)ÕôǛ7m)÷A•–¤æ€Õ¬»~û™¯™šdä?—D†â¼O꣩ÑK,­`­«*j¼:-=l‹å§Í\§Æ_¶ƒª+Ë,.MÌɬJ"Ç@Ôɼœf>œãÿ
_¡yÿÔz~?ð^

==> imcsnvldb2023 copy/.git/objects/55/7e7a7281d5966756b439f2b3e05045955fd33e <==
xuTÁnÛ0Ý9_Ñ/ØÖvö›'ņ;
»,;H2m'EE¢²t†ÿ}tܱdß>Š'²¨nnï?}y³`åéf³ó¦]']µû þZ©Àþ¾ûÓEJûì!Œ9DºÎHï=õ§wˇ¡ßìÆ8&Gz/ú{®z"C'dÐ
ýûp©3ËѵðJüXT©É!q7içW!/°Œµv¦¢\=iËDǤ^¡Û¹ìºB³þ˜E6Aú¶¤Jj¬M"«Í¸H*[ÎàÇö§Ð
†olküº:/…¸ïdØóf{©€K~˜‹½\–‰ZQVU€!4—Dþ9˜¦%^ÃÎĸ´8èȸÕ£EYzRQA¼ÈCÿyÞNäÇ d©\ht<•}}ÿEüŠvÙÁËÈ3_屜½Åºb"¶7³Šï-»uÖêÑr½íӃHÎRÙÃY㖁°°ã…–LíÖ6øt.õq>iɀ®'–Léñפ‹!LPöž¤	Þ(½€"ìü¸æwó¨<«Éø-ðoX8ZAmœ™s¶Ä//YX8'=Ó›ÿ·Þ-ù

==> imcsnvldb2023 copy/.git/objects/5a/c9e00d09e099e19e5fd8e04fa84d129efe268d <==
xÍK1Å=篈W¡iµÔƒàIP{ð$èa³H>&»ÙِdëGØÿÝTK)xsnï
ï7¼Ñ~Ô|½¹<":¤â°›"\ÌÍync2MÚùQåæQ
)Cl"HÆOº¨B&5ïhs»™á#ÿ¨¶ˆå/*]-Ñ7‹)+2 u3›Oà[ª›Êþƒ?†ÿ¨ö#
G*/˜&åñKí
RǓéa€Äïï¶äÀ~rE¶O¯ÏCÌÒ+
¾€s`òÍî"VÛìRPÊb%Ö×f¨=þóúƒË

==> imcsnvldb2023 copy/.git/objects/7c/9497f9d49f8a011978b76917136d4bb0bf0e1d <==
x+)JMU0µ4e040031QH,(HÍKɬÐ+I­`ñL|uiý"köÒ¦Yßlߙ½½ª.µ¢ µ(375¯¬²(|æí«?®4ZÆMu÷Üù—Ìßa¨4+Ë5šÜVu©£üǝ§›'/:ðª4#±(%/µ¸¬ŽWW¥Çû²XVBPÒVɔ³Š—S¡ê2óJŠòSJ"K2óóÀj_:çÂ(aÁûÅéÂü
f	ÉbPµ¹‰ÉEù`EßuÒV®šà#üMÓ~RR§XÒù3+`ŠRK2òSÒò‹rKsJ2rRÁrç¬>WQQ8]Š;ùâŸM·÷öÌB×Pœ™—U®'x¥ñpØ2eí™'æœ>¡ö·X²è;L9ÔؤҔôTHˆÉ"6ZóMn8­×µ¾ñ­«±ÓVo¨ê'¢ÔœÌÜ̼ĢJ°;V/vYn2KÅwκÖI¼>"ˠJ*KRSÊó‹²ÁJMVoÙTÓïQË}Ö)ÕôǛ7m)÷A•–¤æ€Õ¬»~û™¯™šdä?—D†â¼O꣩ÑK,­`­«*j¼:-=l‹å§Í\§Æ_¶ƒª+Ë,.MÌɬJ"Ç@Ôɼœf>œãÿ
_¡yÿÔzݳóÉ

==> imcsnvldb2023 copy/.git/objects/e3/2c86f598ca4c8ce677b7d5beecc46292156af8 <==
xÒÍjÃ0Àñ÷~I–déÜÁèaPú)u·±|".{ÿ9éÚkðt2A&?þɱÁԞípûp¹æÍn»Ù
ç(´ç)_ïOTؗÃÛ~¿ìHj"01ù<Œòw᱀ 
€§è0sÓgŸ4 ¦ÍGqŒàá»í/]ގ?ÃÂW 妏<µó
§Ü•#<¿ä÷kÎ+^Œ±ÒëÜ
ÇòŠyìÁ%Ó$dŽÂ "ê¸Û±ïÇa…KΕ\"'…T4-\òtÏ«,j%,b21«¬;¿¬¢Uc½Ä-–[\¾a±awT$Ž-Ô¶}]£üƒŠ
šxé*x"
§Ò›™ÑMë~'_2#éü

==> imcsnvldb2023 copy/.git/objects/f5/88ef2e333a9c0cee1fec782f143e074bdc2c88 <==
x'MNÃ0…YsŠ¹@£ù³Ç^§ê©ê
RÕD~ªîIÚ°‹d¼ëåoޛs;œ!hx:5ýeèà6¦Ý¡Þú+(4×)+»Y<½³+Ãèˆq>âý½}m`©…L—4˜>ºX!‰YRQs¢à«énmª‡ï~‡ð	Œ+˜ÞÓÔÌ/à'Ú\æߞ÷émLi‹ÔÊI)0º¸²ñŠÊꑕò¦Y´Œµºnè·X})+W"1Ì?XÿlU¯âc U'"+òõ7¸-ÒbW¹òÊH÷ø	WWÅԙ¨ä)"2Îúe‹ò[êƒ&¹°dO'*–÷šØ"|åP>äŸ

==> imcsnvldb2023 copy/.git/objects/f6/eee0072798aee980093a51ecf2caaf7d0e13bb <==
x+)JMU0µ4e040031QH,(HÍKɬÐ+I­`ñL|uiý"köÒ¦Yßlߙ½½ª.µ¢ µ(375¯¬ÒkBåۈŸ3ÖÌ]\"~¢cÁZÃû*ÁJãr…&·Õ{oeê(ÿqçéæɋü*ÍH,JÉK-.«ãÕUéñ>¤,–•"ô†U2å¬âåT¨ºÌ¼'¢ü"Òä'Ìü<°ÚB•L"ë&VLm'G}ÜÜâøF"ª671¹(¬è»NÚÊU|"¿iÚOJêK:f…LQjIF~JZ~QniNIfAN*XƒæýÛ×=ʞ¾«®¼´Ï1ÿJ™Ûrst
řyéPå6y*lÝÓ<U:níñãÆ'le˜r¨±I¥)驐")l´æ›ÜpZ¯k}ã[Wc§­Þ>PÕE©9™¹™y‰E•`wÜx'Þö,(XY[0¹ätüÕÛ«—]ÚU
T™X'šRž_"
Vz¹®¿àõÌ	=ÜîîÞÎÌw˃6B•–¤æ€Õ¬»~û™¯™šdä?—D†â¼O꣩ÑK,­`­«*j¼:-=l‹å§Í\§Æ_¶ƒª+Ë,.MÌɬJ"Ç@Ôɼœf>œãÿ
_¡yÿÔz+ðe

==> imcsnvldb2023 copy/tex/experiment.tex <==
\section{Experiment}\label{sec:experiment}
{In this section, we will conduct experiments on three problems to demonstrate the robustness and effectiveness of our methods:  }

\begin{itemize}[leftmargin = *]
\item The first problem is maximizing the influence in \emph{open} social networks via edge insertions, where existing baselines including the state-of-the-art~\cite{chaoji2012recommendations} are compared (Section~\ref{sec:exp-open}). 
\item The second is our proposed problem, \short{},  where the extensions of the methods in the first problem are compared (Section~\ref{sec:exp-closed}). Note that the core difference between these two problems has been illustrated and please refer to Section~\ref{sec:relatedwork} for details.
\item The third problem is maximizing users' Click-trough Rate in an activity of an online Tencent application, where we deploy our method and evaluate how it helps improve user retentions and interactions (Section~\ref{sec:deploy}). 
\end{itemize}


\smallskip
\noindent\textbf{Datasets}. Table~\ref{table:dataset} presents all the real-world undirected social networks used. In particular, MOBA and MOBAX correspond to two friendship networks of Tencent multiplayer online battle arena games, RPG corresponds to a friendship network of a role-playing game, and the other datasets are available in~\cite{konect}. Note that each edge is represented twice since the influence propagation is directed. To obtain experimental results in a reasonable time under different problem settings, the first four datasets, the next four datasets and the last dataset will be used for the first, the second and the third problem,  respectively.


\smallskip
\noindent \textbf{Environments}. We conduct all experiments on a Linux server with Intel Xeon E5
(2.60 GHz) CPUs and 512 GB RAM. All algorithms are implemented in
Python and our code is available at~\cite{TR}. 





\begin{table}[]
\caption{Dataset Statistics}\label{table:dataset}
\begin{tabular}{cccc}
\hline
\textbf{Dataset} & \textbf{|V|} & \textbf{|E|} & \textbf{Avg. Degree} \\ \hline
EU-Core & 1,005 & 51,142 & 51 \\
Hamster & 2,426 & 33,261 & 14 \\
CiaoDVD & 4,658 & 80,266 & 17 \\
Brightkite & 58,228 & 428,156 & 7 \\ 
%Livemocha & 104,103 & 4,386,166 & 42\\
Catster &149,700 & 10,898,550 & 73\\
MOBA & 503,029 & 9,372,022 & 19 \\
RPG  & 2,331,047 & 88,227,562 & 38\\
Orkut & 3,072,441 & 234,369,798 & 76\\
MOBAX & 36,201,207&3,281,207,036&90\\ \hline
\end{tabular}
\end{table}


\subsection{Experiment with the Open Sharing Model}\label{sec:exp-open}
In this section, we study maximizing the influence in open social networks. Here, we insert a set $X'$ of edges from the candidate set $X$ into the original social network such that (1) at most $k$ edges in $X'$ share the same source node and (2) the influence sum of the seed nodes is maximized. The purpose of this section is twofold: 
\begin{itemize}[leftmargin = *]
\item Our proposed method \outtermethod{} is able to effectively maximize the influence of multiple seed nodes, as compared to the state-of-the-art called continuous greedy \method{CG}~\cite{chaoji2012recommendations} on this problem.
 %Specifically, \method{CG}~\cite{chaoji2012recommendations} studies a slightly different problem where at most $k$ edges in $X'$ share the same source \emph{or} end nodes. 
\item Our proposed method \outtermethod{} is robust to different variations of influence maximization via edge recommendations.
\end{itemize}

\smallskip
\noindent \textbf{Baselines}. Baselines are listed below where \method{Degree} and \method{FoF} (i.e., Friend of Friend) were also compared by \method{CG}~\cite{chen2009efficient}. For ease of description, we assume out-degrees of nodes in the original network to be greater than $k$.

\begin{itemize}[leftmargin = *]
\item \method{Degree} based method where, for candidates sharing the same source node, top $k$ edges with the highest degrees of end nodes are selected.

\item \method{FoF} based method where,  for candidates sharing the same source node, top $k$ edges whose source and end nodes share the highest number of common friends are selected.

\item \method{Random} based method where $k$ edges are randomly selected from candidates sharing the same source node. Its performance is reported as the average over five independent runs.

\item \method{CG}~\cite{chaoji2012recommendations} where edges are inserted based on a continuous greedy method followed by randomized rounding. We set all parameters as recommended by the original work.
\end{itemize}


\smallskip
\noindent \textbf{Edge Weight Settings}. We follow the previous work~\cite{chaoji2012recommendations} to adopt the constant model where each edge in the original network and candidate edge for insertion is assigned with a constant influence probability and we set it as 0.1. Note that the constant model and the influence probability setting are also commonly used by existing studies in the classical influence maximization problem~\cite{arora2017debunking,goyal2011celf++,Kempe03}.
 
\smallskip
\noindent \textbf{Parameter Settings}. Considering that \method{CG} is not scalable to a large number of seed nodes and edge candidates, we conduct experiments on small-scale datasets. Specifically, we randomly select five nodes from the top 1\% nodes with the highest degrees in the original network as the seed nodes. Afterwards, we generate 50 outgoing edges from each node within two hops away from the seed nodes as candidates, and these candidates are generated randomly by following the setup of~\cite{chaoji2012recommendations} where an edge candidate can be added between any pair of nodes without group information. We set $k$ as 20, the error ratio $\epsilon$ of \outtermethod{} as $10^{-4}$, and follow the common standard~\cite{arora2017debunking} to estimate the influence of any solution under the IC model via 10,000 Monte Carlo simulations.



\smallskip
\noindent \textbf{Experimental Results}. Table~\ref{table:openinf} compares the influence spread achieved by different methods under the RMPP model  and the IC model, respectively. It is obvious that there is a positive correlation between influence under the RMPP model and the one under the IC model. That is, greater influence under the former one also indicates larger influence under the latter. Hence, the idea of optimizing the RMPP-based influence spread to approximate the IC-based influence is effective. \outtermethod{} significantly outperforms \method{Degree}, \method{FoF} and \method{Random}, and achieves very competitive results with \method{CG}. Furthermore, \outtermethod{} achieves up to five-orders-of-magnitude speedup over \method{CG} as shown in Table~\ref{table:opentime}. These results demonstrate the efficiency, effectiveness and robustness of \outtermethod{}, in terms of maximizing the  influence of multiple seed nodes via edge recommendations/insertions. 



\begin{table}[]
\caption{Comparison of influence achieved by different methods under the RMPP model (RP) and the IC model.}\label{table:openinf}
\begin{tabular}{ccccccccc}
\hline
\multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c}{\textbf{EU-Core}} & \multicolumn{2}{c}{\textbf{Hamster}} & \multicolumn{2}{c}{\textbf{CiaoDVD}} & \multicolumn{2}{c}{\textbf{Brightkite}} \\ \cline{2-9} 
 & \textbf{RP} & \textbf{IC} & \textbf{RP} & \textbf{IC} & \textbf{RP} & \textbf{IC} & \textbf{RP} & \textbf{IC} \\ \hline
Degree & 65 & 2801 & 65 & 2513 & 92 & 5891 & 80 & 8912 \\
FoF & 68 & 3012 & 67 & 2789 & 95 & 6013 & 75 & 8134 \\
Random & 70 & 3189 & 64 & 2445 & 100 & 6231 & 73 & 7986 \\
\outtermethod{} & 76 & 3684 & 72 & 3142 & 109 & 6618 & 88 & 12034 \\
CG & 78 & 3769 & 74 & 3221 & 109 & 6680 & 89 & 12851 \\ \hline
\end{tabular}
\end{table}



\begin{table}[]
\caption{Running time comparison between CG and \outtermethod{}.}\label{table:opentime}
\begin{tabular}{ccccc}
\hline
\textbf{Method} & \textbf{EU-Core} & \textbf{Hamster} & \textbf{CiaoDVD} & \textbf{Brightkite} \\ \hline
\outtermethod{} & 5.8E-1 & 1.7E-1 & 1.5E0 & 1.7E1 \\
CG & 3.56E4 & 3.0E4 & 5.5E4 & 4.6E4 \\ \hline
\end{tabular}
\end{table}




\begin{table}[]
\caption{Effectiveness comparison with $k=30$ and $|S|=50$.}\label{table:orgvsbst}
\begin{tabular}{cccccccc}
\hline
\multirow{2}{*}{\textbf{Dataset}} & \multicolumn{2}{c}{\textbf{Degree}} & \multicolumn{2}{c}{\textbf{FoF}} & \multicolumn{2}{c}{\textbf{Random}} & \multirow{2}{*}{\textbf{\outtermethod{}}} \\ \cline{2-7}
 & \textbf{Ori} & \textbf{Bst} & \textbf{Ori} & \textbf{Bst} & \textbf{Ori} & \textbf{Bst} &  \\ \hline
%Livemocha & 6.1E2 & 7.8E5 &7.9E2& 8.0E5&2.9E3&8.3E5&\textbf{9.8E5}\\
Catster & 3.1E2 & 4.2E5 & 3.8E2 & 4.8E5 & 3.6E3 & 6.3E5 & \textbf{8.6E5} \\
MOBA & 5.0E6 & 7.4E6 & 6.5E6 & 7.7E6 & 7.0E6 & 8.0E6 & \textbf{9.8E6} \\
RPG & 1.1E6 &2.1E7 &   2.4E6 &2.2E7 &1.9E7 & 2.4E7 & \textbf{3.2E7} \\
Orkut & 7.0E2 & 5.4E7 & 6.8E2 & 5.6E7 & 9.6E5 & 5.9E7 & \textbf{8.2E7} \\ \hline
\end{tabular}

\end{table}


\iffalse
\begin{table}[]
\caption{Running time (s) comparison with $k=30$ and $|S|=50$ where the numbers in brackets under \outtermethod{} refers to the time cost in the graph expansion stage which is also involved in boosted baselines. Note that the number of common friends is pre-computed in \method{Bst-FoF}.}\label{table:orgvsbsttime}
\small
\begin{tabular}{cccccccc}
\hline
\textbf{Dataset} & \textbf{Bst-Degree} & \textbf{Bst-FoF} & \textbf{Bst-Random} & \textbf{\outtermethod{}} \\ \hline
Catster & 106.16 & 100.85 & 97.82 & 120.22 \\
MOBA &135.99& 129.19 & 125.31 & 177.63 \\
RPG & 957.20& 909.34 & 882.06 & 982.03\\
Orkut & 4436.54& 4214.71 & 4088.27 & 5094.28\\ \hline
\end{tabular}

\end{table}
\fi


\begin{table}[]
\caption{ Running time (s) comparison with $k=30$ and $|S|=50$ where the numbers in brackets under \outtermethod{} refers to the time cost in the graph expansion stage which is also involved in boosted baselines. Note that the number of common friends is pre-computed in \method{Bst-FoF}.}\label{table:orgvsbsttime}
\small
\begin{tabular}{cccccccc}
\hline
\textbf{Dataset} & \textbf{Bst-Degree} & \textbf{Bst-FoF} & \textbf{Bst-Random} & \textbf{\outtermethod{}} \\ \hline
Catster & 1.1E2 & 1.0E2 & 9.8E1 & 1.2E2 (9.1E1)\\
MOBA &1.4E2& 1.3E2 & 1.2E2 & 1.8E2 (1.3E2)\\
RPG & 9.6E2& 9.1E2 & 8.8E2 & 9.8E2 (7.3E2)\\
Orkut & 4.4E3& 4.2E3& 4.1E3 & 5.1E3 (3.6E3)\\ \hline
\end{tabular}

\end{table}





\begin{figure*}[t]
\includegraphics[width=0.5\textwidth]{./drawing2/legend1}
\vspace{-0.25cm}

\centering

\centering


\subfloat[Catster]{
\includegraphics[width=0.24\textwidth]{./drawing2/difft_Catster.pdf}\hspace{-1em}
}
\hspace{0.5mm}
\subfloat[MOBA]{
\includegraphics[width=0.24\textwidth]{./drawing2/difft_LOL.pdf}\hspace{-1em}
} 
\hspace{0.5mm}
\subfloat[RPG]{
\includegraphics[width=0.24\textwidth]{./drawing2/difft_RPG.pdf}\hspace{-1em}
}
\hspace{0.5mm}
\subfloat[Orkut]{
\includegraphics[width=0.24\textwidth]{./drawing2/difft_Orkut.pdf}\hspace{-1em}
}

\vspace{-0.7em}
\caption{Performance Comparison with different $|S|$.}\label{fig:diffs}
\vspace{-2.5em}
\end{figure*}



\begin{figure*}[t]
%\includegraphics[width=0.5\textwidth]{./drawing2/legend1}
%\vspace{-0.25cm}

\centering

\hspace{0.5mm}
\subfloat[Catster]{
\includegraphics[width=0.24\textwidth]{./drawing2/diffk_Catster.pdf}\hspace{-1em}
}
\subfloat[MOBA]{
\includegraphics[width=0.24\textwidth]{./drawing2/diffk_LOL.pdf}\hspace{-1em}
} 
\hspace{0.5mm}
\subfloat[RPG]{
\includegraphics[width=0.24\textwidth]{./drawing2/diffk_RPG.pdf}\hspace{-1em}
}
\hspace{0.5mm}
\subfloat[Orkut]{
\includegraphics[width=0.24\textwidth]{./drawing2/diffk_Orkut.pdf}\hspace{-1em}
}

\vspace{-0.7em}
\caption{Performance Comparison with different $k$.}\label{fig:diffk}
%\vspace{-1.5em}

\end{figure*}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\iffalse
\begin{figure*}[t]
\centering


\subfloat[Catster]{
\includegraphics[width=0.24\textwidth]{./drawing2/difftalltime_Catster.pdf}\hspace{-1em}
}
\hspace{0.5mm}
\subfloat[MOBA]{
\includegraphics[width=0.24\textwidth]{./drawing2/difftalltime_LOL.pdf}\hspace{-1em}
} 
\hspace{0.5mm}
\subfloat[RPG]{
\includegraphics[width=0.24\textwidth]{./drawing2/difftalltime_RPG.pdf}\hspace{-1em}
}
\hspace{0.5mm}
\subfloat[Orkut]{
\includegraphics[width=0.24\textwidth]{./drawing2/difftalltime_Orkut.pdf}\hspace{-1em}
}

\vspace{-0.7em}
\caption{Efficiency Comparison with different $|S|$.}\label{fig:diffsalltime}
\vspace{-2.5em}
\end{figure*}



\begin{figure*}[t]
%\includegraphics[width=0.5\textwidth]{./drawing2/legend1}
%\vspace{-0.25cm}

\centering

\hspace{0.5mm}
\subfloat[Catster]{
\includegraphics[width=0.24\textwidth]{./drawing2/diffkalltime_Catster.pdf}\hspace{-1em}
}
\subfloat[MOBA]{
\includegraphics[width=0.24\textwidth]{./drawing2/diffkalltime_LOL.pdf}\hspace{-1em}
} 
\hspace{0.5mm}
\subfloat[RPG]{
\includegraphics[width=0.24\textwidth]{./drawing2/diffkalltime_RPG.pdf}\hspace{-1em}
}
\hspace{0.5mm}
\subfloat[Orkut]{
\includegraphics[width=0.24\textwidth]{./drawing2/diffkalltime_Orkut.pdf}\hspace{-1em}
}

\vspace{-0.7em}
\caption{Efficiency Comparison with different $k$.}\label{fig:diffkalltime}
%\vspace{-1.5em}

\end{figure*}

\fi




\subsection{Experiment on the \short{} problem}\label{sec:exp-closed}
 We conduct seven experiments to demonstrate that: (1) the extension of existing baselines on open social networks cannot well address our problem but their performance can be significantly boosted with the help of our method \outtermethod{} (Exp1); (2) \outtermethod{} consistently and significantly outperforms all the boosted baselines with different $|S|$ and $k$ (Exp2-3); (3) how $k$ and $|S|$ impact the convergence of \outtermethod{} (Exp4); (4) \outtermethod{} is highly scalable to handle large-scale datasets (Exp5); (5) the influence convergence is also a good indicator of the node size convergence in the diffusion network (Exp6); (6) the influence of seeds in the diffusion network, produced by \outtermethod{} with a small edge size, is very competitive with the influnce of the seeds in the original network (Exp7).




\iffalse
\begin{table}[]
\caption{The percentage of edges recommended by the expansion stage of \outtermethod{} over the total edge size of the diffusion network produced by boosted baselines with $k=30$ and $|S|$. Note that the total edge size is the same across different boosted baselines since they are built upon the same input diffusion network.}\label{table:edgeparticapation}
\begin{tabular}{cccc}
\hline
\textbf{Livemocha}& \textbf{Catster} & \textbf{MOBA} & \textbf{Orkut} \\ \hline
					27\%		&		19\%				&			17\%&21\% \\ \hline
\end{tabular}
\end{table}
\fi



\smallskip
\noindent \textbf{Baselines}. We compare six baselines which include the aforementioned methods, \method{Degree}, \method{FoF} and \method{Random}, as well as their respective boosted versions. Since each baseline has two versions, original and boosted, we use the prefixes `Ori' and `Bst' to distinguish them. The boosted versions are built upon the diffusion network generated by the \emph{expansion} stage of \outtermethod{} (i.e., Lines 5-9 in Algorithm~\ref{alg:practicalframework}) and work similar to the original ones. The only difference is that, in the boosted version, some important edges have been inserted by \outtermethod{} and these baselines only `fill up' recommendations for those nodes in the generated diffusion network. Hence, if we assume that the out-degrees of nodes in the original network are greater than $k$ and our method has already inserted $h <k$ outgoing edges from $u$, these boosted versions just need to select $k-h$ outgoing edges for $u$. For the reason why \method{CG}~\cite{chaoji2012recommendations} cannot be extended, please refer to Section~\ref{sec:relatedwork} and its scalability issue in Section~\ref{sec:exp-open} for details.




\iffalse
\noindent \textbf{Baselines}. Six baselines are listed below. 
%Notably,  \method{Ori-Degree} and \method{Ori-FoF} were also compared by the state-of-the-art~\cite{chaoji2012recommendations} in open social networks. \bao{can remove the previous sentence.} 
For ease of description, we assume that the out-degrees of nodes in the original network are greater than $k$, and emphasize that all edges in the original network are candidates for insertion into the diffusion network which initially contains seed nodes only.

\begin{itemize}[leftmargin=*]
\item \method{Ori-Degree}: for candidates sharing the same source node, top $k$ edges whose end nodes have the highest degrees are selected.

\item \method{Ori-FoF}: for candidates sharing the same source node, top $k$ edges whose source and end nodes share the highest number of common friends are selected.

\item \method{Ori-Random}: $k$ edges are randomly selected from candidates sharing the same source node. Its performance is reported as the average performance over five independent runs.

\item \method{Bst-Degree}, \method{Bst-FoF} and \method{Bst-Random} are the boosted extension of the previous three methods, respectively. The boosted versions are built upon the diffusion network generated by the \emph{expansion} stage of \outtermethod{} (i.e., lines 5-9 in Algorithm~\ref{alg:practicalframework}) and work similarly to the original ones. The only difference is that, in the boosted version, some important edges have already been recommended/inserted by \outtermethod{} and these baselines just `fill up' recommendations for nodes in the generated diffusion network. Hence, if our method has already inserted $h<k$ outgoing edges from $u$, these boosted versions just need to select at $k-h$ outgoing edges for $u$. Since each baseline has two versions, original and boosted, we use the prefixes `Ori' and `Bst' to distinguish them.
\end{itemize}

%The method in~\cite{chaoji2012recommendations} is not considered, because in the input diffusion network which only contains seed nodes, it fails to help seeds influence the nodes that are more than one hop away. Moreover, there is no non-trivial extension of \method{CG} that is scalable to large-scale networks and can notably outperform our proposed method, as evidenced by experiments on a variation of our problem in open social networks~\cite{TR}.
\fi


\smallskip
\noindent \textbf{Edge Weight Settings}. Considering that the influence probability of edges are different in practice, we adopt the commonly used trivalency model~\cite{chen2010scalable} for Catster and Orkut without edge attributes. It randomly assigns a weight for each edge, from $\{10^{-1},10^{-2},10^{-3}\}$. 

For MOBA and RPG, we assign edge weights based on the intimacy of friendship. In MOBA and RPG, each pair of friends has different levels of intimacy which describes the number of interactions (e.g., the number of games they play together, the number of gifts sent from one to another). Since the pair-wise intimacy in both  MOBA and RPG is represented as integers, here we transform it into an influence probability within [0,1] for deployment in the IC model. According to the Susceptible-Infected-Recovered (SIR) model~\cite{anderson1992infectious} and heterogeneous mean-filed theory~\cite{newman2002spread,cohen2011resilience,castellano2010thresholds,xie2021detecting}, the lowest influence probability should not be smaller than a constant $\lambda$ times $\beta_c= \sum_{v \in V} |N_{out}(v)| / (\sum_{v \in V} |N_{out}(v)|^2- \sum_{v \in V} |N_{out}(v)|)$, where $\beta_c$ is the epidemic threshold in the SIR model and calculated as 0.024 and 0.001 on MOBA and RPG, respectively. If $\lambda \beta_c$ is too small, the influence of the seeds will be quite limited. If $\lambda \beta_c$ is too large, the influence spread can cover a large percentage of nodes, irrespective of where it originated, and the methods' performance cannot be well compared. By following existing studies~\cite{shu2015numerical,lu2016h}, we
determine $\lambda$ by simulation on real networks. Specifically, we determine $\lambda_1$ and $\lambda_2$ and control the edge weights within the range $[\lambda_1\beta_c, \lambda_2\beta_c]$. Each influence probability $p_{(u,v)}= ((u,v)_{I} - \min_{e\in E} e_{I}) / (\max_{e\in E} e_{I} -\min_{e\in E} e_{I}  ) (\lambda_2 -\lambda_1)\beta_c +\lambda_1\beta_c$ where $(u,v)_{I}$ denotes the intimacy between $u$ and $v$. Note that we have checked several settings of $\lambda_1$ and $\lambda_2$ and these different settings will not affect the conclusion (i.e., performance ranking of methods). To test these methods' robustness to the influence probability distributions, in both MOBA and RPG, we set the range $[\lambda_1\beta_c, \lambda_2\beta_c]$ as $[0.007,0.01]$ which has a dramatically different distribution from the trivalency model deployed for other datasets.





\smallskip
\noindent \textbf{Parameter Settings}. We randomly select $|S|$ (50 by default) nodes from the top 1\% nodes with the highest degrees in the original network as the seed nodes, set $k=20$ and the error ratio $\epsilon=10^{-4}$ by default. We evaluate solution quality based on the IC-based influence spread via 10,000 Monte Carlo simulations. 


\smallskip
\noindent \textit{\textbf{Exp1 - Case study on the two versions of baselines}}. Table~\ref{table:orgvsbst} and Table~\ref{table:orgvsbsttime} compare the effectiveness and efficiency with $k=30$ and $|S|=50$. We have four main observations:
%The main observation is that the boosted versions can achieve about five-order-of-magnitude larger influence than their original counterparts but can be still outperformed by \outtermethod{}. Specifically, \outtermethod{} outperforms the second best performer by at least 23\%-39\% on different datasets respectively. More observations are in Appendix~\ref{appendix:casestudy}. Due to the poor performance of the original baselines, we only use the boosted versions for comparison in the rest of experiments.  
%\subsection{Case study on two versions of baselines}\label{exp:casestudy}
%We have two observations in Table~\ref{table:orgvsbst}:
%(1) the performance gap between original versions of baselines and \outtermethod{} is much more greater than the one in Section 6.1 such that \outtermethod{} can achieve up to five-order-of-magnitude larger influence (e.g., on Orkut). This observation is mainly caused by the significant difference in the topological information of the input diffusion network and the size of edge insertions. Specifically, in Section 6.1, the diffusion network is the original network which contains rich topological information and the size of edge insertions is quite small. On the other hand, in this section, the original versions start from a diffusion network which initially only contains seed nodes and face considerable edge insertions which contribute all influence increment of seeds.
\vspace{-1mm}
\begin{enumerate}[leftmargin = *]
\item \method{Org-Random} is more effective than the original versions of other baselines. The reason is that nodes with high degrees will `attract' much more incoming edges in other strategies (i.e., \method{Org-Degree} and \method{Org-FoF}) which `waste' a lot of recommendation opportunities to repeatedly influence/activate these nodes. 
\item The boosted versions can achieve about five-orders-of-magnitude larger influence than their original counterpart but can still be notably outperformed by \outtermethod{}. Specifically, \outtermethod{} can still outperform the second best performer by at least 23\%-39\% on different datasets respectively, which demonstrates the effectiveness of both two stages (i.e., the expansion and filling stages). 
\item We also compute the constitution of the edges recommended by \outtermethod{} in the boosted baselines, and the result shows that \outtermethod{} only contributes 17\%-27\% of total edges in the diffusion network. The significant performance improvement of baselines with limited involvement of \outtermethod{} further demonstrates the effectiveness of \outtermethod{} in terms of identifying important edges and nodes for increasing the seeds' influence. 

\item \outtermethod{} is very competitive with other boosted baselines in terms of running time, because all methods involve the \emph{expansion} stage of \outtermethod{} (i.e., Lines 5-9 in Algorithm~\ref{alg:practicalframework}) which dominates the total computational cost. 
\end{enumerate}
\vspace{-1mm}

Due to the poor performance of the original baselines, we only use the boosted versions for comparison in the rest experiments.  



\smallskip
\noindent \textit{\textbf{Exp2 - Effectiveness comparison with different $|S|$}}. 
%\subsection{Effectiveness Comparison with Different $|S|$}\label{exp:|S|effectiveness}
Figure~\ref{fig:diffs} compares the performance with different $|S|$. Our method \outtermethod{} consistently outperforms other methods across all instances while the performance of other methods is not stable, e.g., \method{Bst-Random} outperforms \method{Bst-Degree} on Catster but the latter is more effective on Orkut. Another interesting observation is that the performance ranking of methods on the same dataset is consistent across different $|S|$. We think that a good edge recommendation for a non-seed user $u$ under an instance with a small $|S|$ can also be an effective recommendation for $u$ as the seed user under an instance with a great $|S|$. Thus, the diffusion networks generated by the expansion stage of \outtermethod{} under different $S$ can be similar such that edges chosen by a specific baseline upon these networks have large overlaps, which explains this observation and reflects the superiority of \outtermethod{}.


\smallskip
\noindent \textit{\textbf{Exp3 - Effectiveness comparison with different $k$}}. 
%\subsection{Effectiveness comparison with different $k$}\label{exp:keffectiveness}
Figure~\ref{fig:diffk} compares the performance at different $k$ across all datasets. We have four main observations: 
\vspace{-1mm}
\begin{enumerate}[leftmargin = *]
\item \outtermethod{} outperforms the boosted baselines and can achieve up to two-orders-of-magnitude larger influence (e.g., on Orkut). 
\item The performance gap becomes smaller when $k$ is larger. The reason is that all methods make almost the same recommendation strategy to low-degree nodes since their out-degrees are close to or even smaller than $k$. In this case, the number of combinations of $k$ outgoing edges of these nodes is very limited. This observation also explains why the performance gap is larger on datasets with greater average degrees. 
\item When $k$ is small (e.g., 10), all methods achieve similar influence since it is barely possible for any method to achieve large influence with very limited edges. 
\item The performance gap on MOBA and RPG is not as significant as that on other datasets. That is because the average edge weight on MOBA and RPG are notably larger. Thus, regardless of how the diffusion network is generated, seeds can easily influence many nodes with sufficient influence probabilities. 
\end{enumerate}
\vspace{-1mm}
      
Note that the performance difference may not be easily distinguished visually due to the log scale of y axis, but we have shown the notable performance difference with $k=20$ and $k=30$ in Figure~\ref{fig:diffs} and Table~\ref{table:orgvsbst} at a finer granularity already. 

\begin{figure}[t]
\includegraphics[width=0.4\textwidth]{./drawing2/legend2}
\vspace{-0.45cm}

\centering
\subfloat[varing $k$]{
\includegraphics[width=0.24\textwidth]{./drawing2/diffkiter_RMPP.pdf}\hspace{-1em}
} 
\hspace{0.5mm}
\subfloat[varing $|S|$]{
\includegraphics[width=0.24\textwidth]{./drawing2/difftiter_RMPP.pdf}\hspace{-1em}
}

\vspace{-1.em}
\caption{The number of iterations in the expansion stage with different $k$ and $|S|$.}\label{fig:convergence}
\vspace{-1.em}
\end{figure}


\begin{figure}[t]
%\includegraphics[width=0.4\textwidth]{./drawing2/legend2}
%\vspace{-0.45cm}

\centering
\subfloat[varing $k$]{
\includegraphics[width=0.24\textwidth]{./drawing2/diffktime_RMPP.pdf}\hspace{-1em}
} 
\hspace{0.5mm}
\subfloat[varing $|S|$]{
\includegraphics[width=0.24\textwidth]{./drawing2/diffttime_RMPP.pdf}\hspace{-1em}
}

\vspace{-1.em}
\caption{Running time of \outtermethod{} with different $k$ and $|S|$.}\label{fig:efficiency}
\end{figure}


\begin{figure}[t]
%\includegraphics[width=0.4\textwidth]{./drawing2/legend2}
%\vspace{-0.45cm}

\centering
\includegraphics[width=0.24\textwidth]{./drawing2/nodeparti_RMPP.pdf}\hspace{-1em}

\vspace{-1.5em}
\caption{The percentage of the nodes in the diffusion network over the one in the original network with different iterations in the expansion stage of \outtermethod{}, where the iterations with solid fill refer to the convergence points under different datasets repsectively.}\label{fig:noderatio}

\end{figure}


\begin{figure}[t]
\includegraphics[width=0.33\textwidth]{./drawing2/legend3}
%\vspace{-0.45cm}

\centering
\subfloat[RPG]{
\includegraphics[width=0.24\textwidth]{./drawing2/INEratio_RPG.pdf}\hspace{-1em}
} 
\hspace{0.5mm}
\subfloat[Orkut]{
\includegraphics[width=0.24\textwidth]{./drawing2/INEratio_Orkut.pdf}\hspace{-1em}
}

%\vspace{-1.em}
\caption{The influence ratio (I-Ratio), edge ratio (E-Ratio) and node ratio (N-Ratio) in the diffusion network produced by \outtermethod{} with different $k$.}\label{fig:INERatio} 

\end{figure}







\smallskip
\noindent \textit{\textbf{Exp4 - Impact of $k$ and $|S|$ on \outtermethod{} convergence}}. 
%\subsection{Impact of $k$ and $|S|$ on \outtermethod{} Convergence}\label{exp:convergence}
Figures~\ref{fig:convergence} (a) and (b) show the number of iterations in the expansion stage of \outtermethod{} when varing $k$ and $|S|$ respectively. Interestingly, when $k$ or $|S|$ increases, the number of iterations for convergence is non-increasing. This is because \outtermethod{} will include more nodes into the current \ksubnetwork{} in each iteration such that it may take fewer iterations to identify all important nodes for influence spread.


\smallskip
\noindent \textit{\textbf{Exp5 - Scalability study on \outtermethod{}}}. 
%\subsection{Scalability Study on \outtermethod{}}\label{exp:scalability}
Figures~\ref{fig:efficiency} (a) and (b) show the runtime of our (full-stage) \outtermethod{} when varing $k$ and $|S|$. As $k$ grows, more nodes tend to be included in the diffusion network and more edges tend to be `filled up' in the filling stage, hence costing more time. On the other hand, increasing $|S|$ does not notably incur more computation costs, for two reasons: 1) we transform the case of multiple seeds into the one of a single virtual node by introducing only $|S|$ extra edges into the diffusion network; 2) the size of the diffusion networks generated under instances of different $|S|$ can be similar as discussed earlier. It is obvious to see that \outtermethod{} is highly scalable and efficient, since it can produce good recommendation on datasets with millions of nodes and hundred millions of edges within two hours (e.g., Orkut). This performance is promising since such recommendation is usually deployed for a long-term usage.


\smallskip
\noindent \textit{\textbf{Exp6 - Impact of iterations on the diffusion network node size}}. 
%\subsection{Impact of iterations on the network size}\label{exp:interation}
Figure~\ref{fig:noderatio} shows how the node size of the diffusion network in the expansion stage of \outtermethod{} grows iteratively. Here, the iterations with solid fill refer to the convergence points. Note that the expansion stage is terminated after convergence for other experiments and here we force it to run 10 iterations. It is obvious that, the node size in the diffusion network converges as the influence spread, which indicates the effectiveness of the convergence criteria.
% in \outtermethod{} and its effectiveness in identifying important nodes for spreading influence. 

\smallskip
\noindent \textit{\textbf{Exp7 - Case study with large $k$}}. 
%\subsection{Case Study with Large $k$}\label{exp:largek}
Here, we conduct a case study on the two largest datasets, RPG and Orkut. Our goal is to show how the statistics of the diffusion network produced by \outtermethod{} and influence spread of seed nodes in this network will change when we further increase $k$ up to 50. Specifically, we use the \emph{influence ratio} (I-Ratio) to denote the percentage of the influence of seeds in the diffusion network over their full influence in the original network, \emph{edge ratio} (E-Ratio) and \emph{node ratio} (N-Ratio) to denote the percentage of the edge and node size of the diffusion network over the ones of the original network, respectively. As shown in Figure~\ref{fig:INERatio}, as $k$ increases, \outtermethod{} is able to achieve an I-Ratio of 90\% with only an E-Ratio of 36\%, and an I-Ratio of 94\% with only an E-Ratio of 46\% on RPG and Orkut respectively. These again demonstrate the superiority of \outtermethod{}. 
Furthermore, when the N-Ratio converges, the I-Ratio can still notably increase as $k$ grows, and even the converged N-Ratio can be notably smaller than 1 (e.g., on RPG). These indicate that \outtermethod{} can identify important nodes for spreading the influence. 


\iffalse
\smallskip
\noindent \textbf{More Experiments on open social networks}. We also conduct experiments on the problem of maximizing the seeds' influence in \emph{open} social networks. Specifically, this problem assumes \emph{all} friends to be recipients for further information propagation, and aims to insert a limited number of edges (i.e., constructing new friendships) into the network to maximize the seeds' influence. We compare our method \outtermethod{} with several baselines including the state-of-the-art~\cite{chaoji2012recommendations} with approximation guarantees. The results show that: 1) \outtermethod{} is able to effectively maximize the influence of multiple seed nodes while achieving five-orders-of-magnitude speedups than~\cite{chaoji2012recommendations}; 2) \outtermethod{} is robust to different edge insertion constraints for maximizing the seeds' influence. Please refer to our technical report~\cite{TR} for details.
\fi


\subsection{Deployment}\label{sec:deploy}
In order to demonstrate the practical effectiveness of our \short{} problem, we deployed our solution into an activity in a multi-player online battle arena game of Tencent of which the friendship network is MOBAX in Table~\ref{table:dataset}.

\smallskip
\noindent \textbf{Summary of the activity}.
Users join this activity by interacting (e.g., sending gifts and gaming invitation) with their friends recommended by the system and will obtain rewards via such interactions. This form of interaction could trigger domino effects such that the interactions can stimulate the message receiver to further interact with other users. The aim of this activity is to improve user retention and interactions. Note that, in this activity, we do not specifically designate seeds and every user could be a potential and spontaneous seed. Specifically, users who log in the game will see this activity and may perform three possible behaviors: (1) proactively start interactions as a seed, (2) start interactions as a message receiver (i.e., a non-seed) and (3) ignore this activity. 

\smallskip

{ \noindent \textbf{Edge weights and the diffusion model}. We adopt the same settings as we use for generating edge weights on MOBA and RPG, and generate the diffusion network based on the IC model. Note that the IC model is only used for generating the diffusion network but not used for evaluation since it is very likely that the real-world influence will not spread in a way specified by the IC model or any other classical diffusion models (e.g., Linear Threshold model~\cite{Kempe03}).}

\smallskip
\noindent \textbf{Methods for comparison}. Four methods, namely \method{Random}, \method{Degree}, \method{FoF} and \outtermethod{}, are deployed. For evaluation, we use an online A/B testing. Specifically, it randomly assigns each online user to one of these four methods which recommend a list of friends for each assigned user.
% and the graph induced by users assigned to \outtermethod{} forms the MOBA dataset in Table~\ref{table:dataset}. 
The list size $k$ is set as 20 for all methods because, in this application, only 20 friends are shown due to several reasons (e.g., the screen size and resolution settings of most mobile devices).
{Based on our observations made in Section~\ref{sec:exp-closed}, the k-subnetwork generated based on a given seed set could also be effective for different seed sets.
Thus, for \outtermethod{}, we first generate the \ksubnetwork{} with top 10\% of assigned users with the highest degrees as the seeds, and then use this generated \ksubnetwork{} for this activity where every user could be a potential seed or non-seed.}



\smallskip
\noindent \textbf{Experimental results}. {The number of users who interact with recommended friends directly indicates the quality of the underlying recommendation system and can effectively reflect the potential size of users who are impacted by others to performance interactions. 
Thus, we adopt the Click-through Rate (CTR) to evaluate the performance.} The CTR denotes the number of users who interacted with recommended friends divided by the total number of users who log in the game during this activity. %Since it is intractable to capture the influence spread in practice, CTR is a good alternative metric for evaluation in industry. 
The CTR achieved by \method{Random}, \method{Degree}, \method{FoF} and \outtermethod{} are 81.87\%, 82.73\%, 82.81\% and \textbf{88.14\%} respectively, which again demonstrates the effectiveness of \outtermethod{}. Despite that CTR is a very popular evaluation metric for recommendation systems in industry, there still exist some other evaluation metrics (e.g., the actual influence spread of seeds via knowing the propagation paths and who are the seeds) worthy of explorations. However, due to the privacy restriction of this activity, we have no access to the detailed information in user logs to compute the performance under other potential metrics. In future, we would like to see how our proposed method will perform in other activities under various evaluation metrics.




==> imcsnvldb2023 copy/tex/experiment3.tex <==
\section{Experiments}


In this section, we will conduct extensive experiments on real-world datasets to evaluate the quality of \constraint{} pricing schemes produced by different methods according to the interests of stakeholders as shown in Figure~\ref{plan}. Specifically, we outline the following progressive questions to guide our evaluations, with the exact solution \fcexact{} under limited integer price choices as the reference:

\smallskip
Q1. Whether the pricing scheme is able to hire candidates with reasonable prices so as to maintain a good balance between conflict interests of the brand and influencers in the charges on the campaign plan?

\smallskip
Q2. Whether the pricing scheme is able to help the brand to achieve large advertising exposure?

\smallskip 
Q3. Whether the pricing scheme attracts considerable investments from the brand?

\smallskip
Q4. Whether the pricing scheme can be produced efficiently?

\smallskip
Q5. How far the performance of the pricing scheme is away from the converged \fcexact{} with increasingly sizes of price choices?

\smallskip
In Section 8.1, we will systematically analyze the interests of stakeholders and introduce the corresponding evaluation metrics. In Section 8.2, we will use the introduced metrics to evaluate different methods so as to answer the questions above. 

\subsection{Experimental Setup}


\begin{figure}[!t]

\centering

\subfloat[LastFm]{
\includegraphics[width=0.2355\textwidth]{./distributions/Lastfm.pdf}
}
\subfloat[Orkut]{
\includegraphics[width=0.24\textwidth]{./distributions/Orkut.pdf}
}
\vspace{-0.36cm}
\caption{Degree distributions and influencer categorization.}\label{distributions}

\end{figure}

\noindent \textbf{Datasets}. We collect four public undirected real-world datasets~\cite{konect} for experiments whose statistics are shown in Table~\ref{dataset}. Due to consistent observations on the experimental results across datasets, we only report experiments on LastFM and Orkut with drastically different scales where we can better compare the scalability of different methods. Furthermore, the expensive \fcexact{} is able to produce most of the results on these two datasets within our time limit (i.e., 60 hours) such that we can more comprehensively compare methods' performance.

{
\color{red} \noindent \textbf{Influencer categorization}. To test the robustness of our methods to candidate sets with different degree distributions, we coarsely divide influencers into three classes, Macro, Micro and Nano, with the naming convention in this domain~\cite{category}. Specifically, we order online users in non-increasing order of their degrees and group influencers based on this order into the same tier (i.e., Macro, Micro or Nano influencer) if their total degrees constitute 20\% of the total degrees in the social network, as shown in Figure~\ref{distributions}. 

}



\input{tex/datasets.tex}
\smallskip
\noindent \textbf{Methods for comparison}. In this experiments, we use the following methods for comparison.

\begin{enumerate}
 \item  \textbf{\bcexact{}}. The binary-choice based dynamic programming (i.e., Algorithm~\ref{BC-DP}) which produces the minimum divergence score when we can either hire each influencer $v$ with the price equal to her influence (i.e., $p_v=\delta(v)$) or do not hire her (i.e., $p_v=0$).
 
 \item \textbf{\bcmg{}}. The binary-choice and minimum gain based algorithm (i.e., Algorithm~\ref{BC-Greedy}) which approximates the optimal divergence score by computing the complement set of the solution set through iteratively choosing influencers with the minimum gain of $f()$ score per unit price. 
  
  \item \textbf{\fcexact{}}. The flexible-choice based exact algorithm (i.e., Algorithm~\ref{FC-DP}) which is able to find the optimal solution when each influence $v$ is assigned with an integer price choice set $R_v$ which consists of her influence plus a number $num$ of integer prices evenly dividing the continuous range $[0.5*\delta(v), 1.5*\delta(v)]$ in a coarse-grained level. That is, $R_v$ consists of integers which are floors of floats in the set $\{\delta(v)(0.5+1/num), \delta(v)(0.5+2/num),..., \delta(v),..., 1.5\delta(v)   \}$ where $|R_v|$ is set as 10 by default.
  
 \item \textbf{\fcinf{}}. The flexible-choice and influence based greedy algorithm (i.e., Algorithm~\ref{FCInf-Greedy}) which iteratively satisfies the profit expectation of the influencer with the greatest influence given a continuous range of price choices for hiring each influencer. In experiments, we set the range as between zero and the input budget.
 
 \item \textbf{\fcmws{}}. The flexible-choice and maximum-weighted subsequence based algorithm (i.e., Algorithm~\ref{FCMWS-Greedy}) which first finds the subsequence of influencers whose profit expectation can be exactly satisfied with the greatest total $f()$ scores among all qualified subsequences, and then adjusts the remaining influencers' prices and greedily choose them based on their gains of $f()$ scores per unit price. 

 
\end{enumerate}




\smallskip
\noindent \textbf{Parameter settings}. We describe the settings of parameters needed for modeling the fundamental procedure involving all stakeholders in the influencer marketing as shown in Figure~\ref{model}, and they are the maximum investment budget from the brand, the candidate set recommended from the agency and profit expectations of candidate influencers:

\begin{enumerate}
\item \textbf{The investment budget}. The brand offers the maximum budget $B$ it can invest to the agency. The agency then will look for suitable candidature influencers who have high alignments with the brand's product to be promoted, and whose total influence should match with the budget considering the standard price rate (price per follow) in this market~\cite{pricerate}. For simplicity, we assume the standard price rate to be one since it does not impact our judgment on the performance of each method.

 
 \item \textbf{The candidate influencers}. Here we assume that the candidate set has been found since this process is orthogonal to our study. Considering the charges on contracted influencers for agent commission (usually 20\%~\cite{commission}) and that it may not be possible to find suitable candidates perfectly matched with the budget, we create the candidate set $\candidates{}$ by randomly selecting a number of candidates ($|\candidates{}|=90$ by default) from the aforementioned three tiers of influencers (i.e., Macro, Micro and Nano), and set $B$ as 80\% of the total influence of candidates. To show the robustness of our methods to combinations of influencers of different tiers, we create the candidate set with the following different sampling distributions: \{Macro:0.5, Micro:0.25, Nano:0.25\}, \{Macro:0.25, Micro:0.5, Nano:0.25\}, \{Macro:0.25, Micro:0.25, Nano:0.5\} and \{Macro:0.33, Micro:0.33, Nano:0.33\}. For simplicity, we call these four sampling distributions as Macro-focused, Micro-focused, Nano-focused and Uniform sampling distributions respectively. Due to space limit, we only report results under Micro-focused and Uniform sampling distributions, and we have similar observations on the rest.

\item \textbf{Profit Expectation}. Since each candidate influencer $v$ values her own influence differently in reality based on the detail of the campaign contract and personal factors (e.g., exclusive collaboration with this brand, likeness towards the product to be promoted, choices of media channels, etc.)~\cite{pricing,factorreport}, we use the weighted influence sampled from 
 $[\delta(v), 1.5\delta(v)]$ to include these realistic factors. The profit expectation or expected profit sharing of each influencer controlled by the agency is a weighted-influence related percentage over the budget and we compute this percentage as the weighted influence of the influencer over the total one of all candidates.
\end{enumerate}


\smallskip
\noindent \textbf{Interests-oriented evaluation metrics}. We evaluate the performance of different methods by considering the interests of different stakeholders corresponding to Figure~\ref{plan}: 
\begin{enumerate}
\item From the perspective of the brand, the campaign plan should be \constraint{}. Otherwise, the brand will not fully accept the plan or even reject the it. Furthermore, the \constraint{} campaign plan should be budget-friendly and able to achieve large advertising exposure. In terms of the cost of the plan, the agency cannot make the charges on influencers as low as possible to satisfy the brand which will harm influencers' interests. Even though the information of influencers' expectations is not public to the brand, to protect the brand's benefits, the plan should try to  
make sure that the actual charges of influencers match with rather than larger than their controlled expectations, which is measured by the overall profit divergence score. In terms of advertising exposure, the brand expects the plan to be influential which is measured by the total influence of influencers involved in the campaign plan.

\item From the perspective of candidates, the campaign plan should be able to bring them significant profits. Due to the conflicts of interests between the brand and candidates, blindly increasing influencers' prices will compromise the brand's interests. To protect the benefits of both influencers and the brand, the plan should try to make sure that the actual profits match with rather than smaller than the controlled expectations from influencers, which can be also measured by the overall profit divergence score.

\iffalse
to satisfy their profit expectations which is quantified based on the total profit divergence $\divergence{}$. Directly comparing divergence scores of different methods without any reference is not informative since the divergence score can vary significantly across different settings and datasets and it is hard to know whether the performance difference is significant or not. To control the measured performance in the same scale, we use $\divergence{}/B$ as the evaluation metric considering that the maximum possible divergence score cannot be greater than the input budget $B$, and this metric could give better indication on how far the performance of each method is away from the worst possible case. 
\fi

\item From the perspective of the agency, a good \constraint{} campaign plan should be able to attract large investments from the brand besides protecting benefits of the brand and influencers. Large investment will not only bring the agency considerable profit on agent commission and campaign management, but also be beneficial to involving more contracted influencers and satisfying their profit expectations. The level of investment is measured by how much budget is spent by the campaign plan. 

\end{enumerate}



To summarize, we compare effectiveness of different methods based on three metrics, namely the overall divergence score, the total influence of hired candidates and the invested budget. The importance of these three metrics is ranked as the same order as the aforementioned one since protecting of benefits and improving the satisfaction of involved candiates and the brand is the first priority of the agency. Due to the timeliness of marketing, efficiency also plays a critical role in ensuring success of the business and thus a method which is very effective but incurs exorbitantly computational time is not acceptable.





\smallskip
\noindent \textbf{Environments}. We conduct all experiments on a Linux server with Intel Xeon E5 (2.60 GHz) CPUs and 512 GB RAM. All codes are implemented in Python and any method which cannot finish within 60 hours will be terminated. 

\subsection{Experimental Results}
In this section, we will evaluate the extent to which different methods protect benefits and improve satisfaction of different stakeholders under four evaluation metrics (i.e., divergence score, influence of involved influencers, the invested budget and efficiency). Furthermore, we will conduct ablation study on the impact of the size of price choices on \fcexact{} to demonstrate the effectiveness of \fcexact{} and \fcmws{}.

\input{tex/smalldataset}

\smallskip
\noindent \textbf{Profit divergence comparison}. One simple way for this evaluation is to directly comparing divergence scores $\divergence{}$ of different methods. However, this straightfoward way lacks of references and is not informative since the divergence score can vary significantly across different settings and datasets and it is hard to know whether the performance difference among methods is significant or not. To control the measured performance in the same scale, we use $\divergence{}/B$ as the evaluation metric considering that the maximum possible divergence score cannot be greater than the input budget $B$, and this metric could give better indication on how far the performance of each method is away from the worst possible case.

Figure~\ref{effect:divergence} compares the divergence scores on LastFM and Orkut with different sampling distributions and candidate sizes. Note that different candidate sets on the same dataset correspond to independent cases and thus the optimal $\divergence{}/B$ under different candidate sets can vary notably. \bcmg{} shows very competitive performance compared with \bcexact{} which demonstrates the empirical effectiveness of \bcmg{} which is much better than what its worst-case approximation ratio indicates. However, both of them are notably outperformed by flexible-choices based methods. With \fcinf{} as the reference, the performance of \fcexact{} is generally better under the even-focused sampling distribution than in the micro-focused one. We suspect that \fcexact{} is able to find better pricing scheme from the limited price choices when the degree distribution of candidates is sparser. When candidates have similar degrees, \fcexact{} requires more fine-grained and similar price choices to achieve lower divergence. As for other methods, we do not see any clear impact of sampling distributions on the performance. On the other hand, \fcmws{} significantly outperforms all other methods in all cases, which demonstrates its effectiveness of protecting stakeholders' benefits. 

\input{tex/influence}

\smallskip
\noindent \textbf{Influence comparison}. To better show the influence of campaign plans, we show the influence ratio of the total influence of involved influencers over the optimal influence in the case where we aim to maximize the influence instead of minimizing profit divergence when the price of each influencer $v$ is decided by the standard price rate (i.e., $p_v=\delta(v)$). Such case simulates the brand's estimation on the \emph{ideal} advertising exposure effect based on the public information. To compute the optimal influence in this case, we just need to set the $f()$ score of each influencer equal to the her influence in \bcexact{}. Figure~\ref{effect:influenceratio} shows the influence ratios achieved by different methods. It is interesting to see that \bcexact{} and \bcmg{} with the profit minimization objective achieve very competitive influence compared with \bcexact{} with the influence maxization objective. Furthermore, the performance ranking of \bcexact{} and \bcmg{} under this metric can be indicated from the one under the profit divergence score. For example, when \bcexact{} achieves lower divergence score than \bcmg{} in Figure~\ref{effect:divergence} (c) with $|\candidates{}|=30$, it also achieves greater influence under the same setting. These observations indicate the positive correlations between profit divergence minimization and influence maximization given the same pricing scheme.

On the other hand, flexible-choice based methods are able to achieve better influence ratios since they have greater space for price adjustment and thus hire more candidates. While maintaining very competitive divergence scores, \fcexact{} tends to hire more candidates than \fcinf{} considering its notably greater influencer ratios and the strategy of \fcinf{} which prioritizes hiring influencers with the greatest influence  (e.g., comparing Figure~\ref{effect:divergence} (a) and Figure~\ref{effect:influenceratio} (a) with $|\candidates{}|=30$). It indicates the drawback of \fcinf{} which overly satisfies influencers to a large extent and quickly exhausts the budget, and the effectiveness of \fcexact{} which makes the best strategy given limited integer price choices. Among all methods, \fcmws{} achieves the greatest influence ratios in most cases while maintaining the lowest divergence scores. These observations indicate that protecting benefits of influencers does not necessarily compromise the brand's interest.

\input{tex/investment}
\smallskip
\noindent \textbf{Attracted investment comparison}. Figure~\ref{effect:investment} shows the ratios of the invested budget for hiring candidates over the maximum budget $B$ the brand offers. As mentioned earlier, the invested budget ratio is the least important effectiveness evaluation metric to the agency since protecting benefits of the brand and influencers is the first priority. Even though methods such as \bcexact{} and \fcinf{} slightly outperform \fcmws{} in many cases under this metric, they attract the investment in a way that sacrifices the benefits of the brand or influencers as shown in Figure~\ref{effect:divergence} and Figure~\ref{effect:influenceratio}. Thus, the agency should make comparison between different methods under this metric only when these methods are very competitive in previous evaluation. 


\input{tex/runtime}
\smallskip
\noindent \textbf{Efficiency comparison}. Figure~\ref{effect:efficiency} compares the running time of different methods. \bcmg{} achieves the lowest running time due to its simple strategy and is up to two-orders-of-magnitude faster than \bcexact{}. \fcinf{} and \fcmws{} are ranked as second and third. Despite the notable difference between their time complexity (i.e., $O(|\candidates{}|\log(|\candidates{}|))$ and $O(|\candidates{}|\log(|\candidates{}|) +|\candidates{}|^2)$ ), \fcmws{} is very competitive with \fcinf{} practically since candidate set sizes are usually small. On the other hand, \fcexact{} can be up to six-orders-of-magnitude slower than \bcmg{}, \fcinf{} and \fcmws{}, which is not feasible in real-world scenarios despite its competitive performance compared with many methods.


\input{tex/piece}

\begin{table}[]
\caption{Running time with different $|R|$ on LastFM}~\label{piecetime:lastfm}
\vspace*{-.5em}
\begin{tabular}{cccccc}
\hline
\multirow{2}{*}{Dataset} & \multicolumn{5}{c}{$|R|$} \\ \cline{2-6} 
 & 10 & 20 & 30 & 40 & 50 \\ \hline
Uniform & 1.4E+3 & 3.7E+3 & 5.3E+3 & 5.9E+3 & 6.5E+3 \\
Micro-focused & 1.4E+3 & 3.9E+3 & 5.3E+3 & 6.0E+3 & 6.2E+3 \\ \hline
\end{tabular}
\end{table}

\begin{table}[]
\caption{Running time with different $|R|$ on Orkut}~\label{piecetime:orkut}
\vspace*{-.5em}
\begin{tabular}{cccccc}
\hline
\multirow{2}{*}{Dataset} & \multicolumn{5}{c}{$|R|$} \\ \cline{2-6} 
 & 10 & 20 & 30 & 40 & 50 \\ \hline
Uniform & 9.1E+3 & 3.3E+4 & 6.9E+4 & 1.2E+5 & 1.9E+5 \\
Micro-focused & 8.9E+3 & 3.1E+4 & 6.7E+4 & 1.3E+5 & 1.9E+5 \\ \hline
\end{tabular}
\end{table}


\smallskip
\noindent \textbf{Ablation study on $|R|$ in \fcexact{}}. In order to see the performance limit of \fcexact{} and further demonstrate the effectiveness of \fcmws{}, we gradually increase the size of $R$ for each influencer in \fcexact{}. Figure~\ref{effect:piece} shows the performance of \fcexact{} with different sizes of $R$, where \fcinf Int refers to the version of \fcinf{} allowing integer price choices only. As $|R|$ increases, the performance of \fcexact{} notably increases and converges to a stable state on LaftFM but fails to converge on Orkut within the our time limit (i.e., 60 hours). 
An interesting observation is that, even though \fcexact{} significantly outperforms all methods, it is still outperformed by \fcmws{}. We suspect that it is mainly caused by the fact that \fcexact{} can only work with integer price choices, as evidenced by the notable performance difference between \fcinf{} and \fcinf Int which may even be outperformed by binary-choice based methods. As we can see from Table~\ref{piecetime:lastfm} and Table~\ref{piecetime:orkut}, the running time of \fcexact{} increases drastically as $|R|$ and can be up to eight-orders-of-magnitude slower than other flexible-choice based methods (e.g., comparing with $|\candidates{}|=90$ in Figure~\ref{effect:efficiency}(c) with $|R|=50$), which makes it infeasible to cater for real-world scenarios.














==> imcsnvldb2023 copy/tex/hardness.tex <==
\section{Hardness Analysis}

\begin{figure}[!t]

\centering
\includegraphics[width=0.4\textwidth]{./figures/tree}\hspace{-1em}
%\vspace{-1em}
\caption{An example of a graph constructed based on a set cover instance.} 
\label{fig:tree}
\vspace{-1em}
\end{figure}

In this section, we will show that the \short{} problem is NP-hard via a reduction from the set cover problem defined as below.


\begin{definition}[Set Cover]
Given a set $U$ of elements, a collection $C$ of subsets $A_1,A_2,...,A_{|C|}$ of $U$ where $\cup_{A\in C} =U$, we aim to choose the smallest number of sets from $C$ such that their union is $U$.
\end{definition}


\begin{theorem}
The \short{} is NP-hard.
\end{theorem}

\begin{proof}
To show that \short{} is NP-hard, we will perform reduction from the NP-complete decision problem of set cover, which checks whether we can find $k$ sets from $C$ whose union is $U$, to the special case of \short{} where there is only a single seed user $s$.

Given the collection $C$ of a set cover instance, we construct a deterministic graph with a tree structure where the weight of each edge is 1 as below. First, we find the set $A_{max}$ with the greatest size from $C$ and create a tree with elements in $A_{max}$ as the bottom nodes (at the bottom level). In the second last level, we introduce the set $V'$ of $\lceil |A_{max}|/k  \rceil$ virtual nodes. We next create directed edges from each of virtual node to at most two arbitrary nodes in $A_{max}$ which have not been connected by virtual nodes in $V'$. Afterwards, we create the last third layer based on the last second one by adopting the similar rules. We repeat this step until the root node is constructed. We also create trees for the rest of sets in $C$ similarly. One difference is that, when we create the tree for a set $A$, we need to make sure that the number of virtual nodes in each level is consistent with the corresponding level of the tree constructed based on $A_{max}$. It means that some virtual nodes may not have outgoing neighbors. After we create trees for all sets in $C$, we introduce directed edges from $s$ to all root nodes. 
\begin{example}
Figure~\ref{fig:tree} shows the graph constructed from the set cover instance where $k=2$ and $C=\{ \{a,b,c,d,e\},\{d,e,f\}, \allowbreak \{f,g,h\} \}$. Dash nodes refer to virtual nodes and virtual nodes with the same number come from the tree constructed based on the same set from $C$. Since $A_{max}=\{a,b,c,d,e\}$, the number of virtual nodes in the second last level of all trees are $\lceil |A_{max}|/k  \rceil =3$. 

%In this instance, the challenge of solving the \short{} problem lies in choosing two out of three outgoing edges from $s$, and the optimal solution is to pick edges $(s,1)$ and $(s,3)$.
\end{example}
Since the time cost for creating such a tree is at most $O(|A_{max}| \allowbreak \log_k|A_{max}|  )$, the total reduction process is polynomial in the total size of sets in the collection. To solve the \short{} problem in the constructed graph, we just need to focus on selecting $k$ outgoing edges for the root node $s$ since the out-degree of the rest of nodes in the graph is at most $k$ and edges not incident on $s$ can be all chosen. Considering that the trees constructed from each set in $C$ have the same number of virtual nodes, the quality of outgoing edge selection for $s$ only depends on bottom nodes being reached.  Thus, selecting $k$ outgoing edges for $s$ corresponds to selecting $k$ sets from $C$. Suppose the number of virtual nodes in each tree is $x$. If the optimal influence spread is $k\times x +1+|U|$ (including $s$) which is also the maximum possible influence, we have a `yes' answer to the set cover instance. Otherwise, the answer is `No'.\end{proof}

==> imcsnvldb2023 copy/tex/introduction.tex <==
\section{Introduction}\label{sec:intro}
Social network platforms have been a popular way that allows people to keep in touch with friends and share contents. There are many \emph{open} social networks where the posted content of a user will be available to all followers and even non-followers using search engines. This open sharing model is popular with millennials who are heavily impacted by the Fear Of Missing Out culture and like to put their lives on display and see everything that's going on~\cite{fomo}. 

Recently, \emph{closed} social networks, where sharing is limited to selected persons only, have emerged and are favored by generation Z to cater for privacy issues and information overload in open social networks. At Tencent, the closed sharing model has become a predominant form for sharing information in its numerous applications. For example, users will send a limited number of friends recent news and updates (e.g., COVID-19 statistics and reports of the Olympic winter games) on WeChat, charitable activities on QQ, and event invitations and sales promotion of merchandise on Tencent Shop. Meanwhile, many tech giants (e.g., Facebook, LinkedIn and Pinterest) have started enabling closed sharing models with personalized settings as well~\cite{trend,towardclosed1,towardclosed2,towardclosed3}. Additionally, the closed social network platform WhatsApp recently took the first place from Facebook in downloads~\cite{survery}, which again demonstrates the importance and popularity of the closed sharing model.\let\thefootnote\relax\footnotetext{$^\star$This work was done when the first author did an internship at Tencent.} \let\thefootnote\relax\footnotetext{$^*$Corresponding author.} 


\begin{figure}[!t]

\centering
\includegraphics[width=0.2\textwidth]{./figures/introexample}\hspace{-1em}
%\vspace{-1em}
\caption{The network formed by solid edges is the optimal diffusion network to maximize the influence of $a$ if each user only shares information with up to two friends.}

\label{introexample}
\label{fig:intro}

\end{figure}

On the one hand, in closed social networks, users often do not want to overexpose themselves for various reasons, such as privacy concerns and psychological factors~\cite{expose}, or may have limited sharing opportunities due to resource constraints in events. Therefore, users are likely to share information with only a limited number of friends. 
For example, users in WeChat tend to share their life moments or private matters only with their close friends and families, rather than colleagues with pure business relationships~\cite{block,block2}.
%(2) users who do not like validating existence may share information with whom they think the information is important to, without posting this information to all their friends since this message can be irrelevant to and overwhelm many users; 
%(2) users who spend on online Tencent gaming events may obtain limited virtual coupons for sharing and they need to carefully choose friends to receive the coupons since people who use the coupons can increase the discounts of future purchase of the coupon sender~\cite{gaming}.
Considering that online users have different capabilities of propagating information, as a consequence, the influence spread (i.e., information propagation effect) of a seed user (i.e., a user who releases the content at the very beginning) heavily depends on the friends she chooses to receive the information. Since the information propagation unfolds in a cascading manner, an information receiver can be multiple hops away from the seed and her selected friends for sharing also impacts the influence spread.

On the other hand, users hope that their released information could reach and benefit most of the users. Therefore, to fully realize the social and commercial value of the information with the greatest exposure in closed social networks, an effective strategy of recommending friends to share information is very important. Since each recommendation corresponds to a directed edge in the network, all recommendations constitute a \textit{diffusion network}, which is essentially a subnetwork of the original network and has limit on the number of outgoing edges (i.e., paths from senders to receivers) incident on each node. 

In this paper, we formulate the above recommendation as the problem of Influence Maximization in Closed Social Networks (\short{}), which aims to find the optimal diffusion network via which the seeds' influence spread is the maximum.


\begin{example}
To make this problem more intuitive, we use an example for illustration. Figure~\ref{introexample} shows a toy network where each user will be recommended a limited number of friends, say two, to share information. Suppose we only consider the information diffusion via the friends recommended by the system and ignore the uncontrollable and unpredictable sharing with friends that are not in the recommendation list. Given the seed user $a$ who has three friends $b$, $c$ and $d$, she will send the information to two of her friends, say $c$ and $d$. Afterwards, her friends who receive the information may also choose two of their friends (e.g., the friends $f$ and $g$ of $c$) to receive this information. This process is repeated such that the information diffuses in cascades. If we assume that users will propagate the received information unconditionally, the diffusion network formed by all solid edges refer to the optimal solution where the information from the seed user $a$ can reach the maximum number of users.
\end{example}




%Influence maximization (IM), which leverages information diffusion to select a limited number of seed users with maximum influence spread in social networks, has been extensively studied due to its considerable commercial value and strong application to viral marketing~\cite{Kempe03}. Despite significant progress made, existing studies are built upon an \emph{open} sharing model in the underlying social network (e.g., Twitter) where a message sent from a user will be available to all followers and even non-followers using search engines. Such a model works for millennials who like to put their lives of display and see everything that's going on `FOMO' (i.e., Fear Of Missing Out)~\cite{fomo}. However, generation Z who emphasizes privacy has learned from millennials that oversharing can be risky and thus prefers \emph{closed} social platforms (e.g., WhatsApp, WeChat and QQ) where sharing is limited to only selected persons~\cite{gz}. \bao{You did not posisiton u paper well. Yours is ADS, so after the general motivation above, you should first talk about the needs in tencent, followed by evidence showing other sn platforms are also in this trend!} As evident by a recent survey~\cite{survery}, WhatsApp recently took the first place of Facebook in downloads and there is a trend that open social network platforms (e.g., Facebook, LinkedIn and Pinterest) have started enabling closed sharing models with personalized settings~\cite{trend}.






%In closed networks, seed users will only send the posted content to a limited number of selected friends who will further spread this content to their selected friends. Apart from the privacy concern, the reason of limiting the content recipients is threefold: (1) the posted content targets specific users with special interest or needs, (2) the number of friends of a user can be notably larger than the one that devices or applications (e.g., mobile phones and browsers) can show in a page, \bao{can we remove reason 2? Not straightforward.} and (3) friends may have different capabilities to further spread the influence. Thus, the influence spread of KOLs (i.e., key opinion leaders) or seeds heavily depends on recipients/friends recommended by the platform for further information propagation.

%A good recommendation strategy can help information `reach' the target users, bring considerable social value and increase user activity. For example, a good recommendation strategy can help KOLs effectively 1) spread updates about countries' border requirement caused by COVID-19 to targeted overseas students and citizen with travel needs in WhatsApp and WeChat, 2) release information of new products (e.g., digital devices) to targeted users with purchasing desire or special interests, or 3) activity information (e.g., event invitations and sales promotion of virtual merchandise) to greatly stimulate the user interaction, involvement, and consumption in many applications (e.g., `Ant Forest' - an ecological protection plan of Alibaba and Metaverse in Facebook). 
%Considering the potential benefits above, in this paper, we take the first attempt to study Maximizing Influence in Closed Social Networks (\short{}), which aims to recommend a \emph{limited} number of \emph{existing} outgoing links (i.e., recipients) for users to propagate the information, such that the influence spread of the seeds can be maximized.


Notably, traditional influence maximization~\cite{Kempe03} in open social networks assumes that a user will send information to all her friends, and aims to select a limited number of seeds with the maximum influence spread. Here, we focus on the closed sharing model and selecting a limited number of edges such that the influence spread of \emph{specific seeds} via these \emph{selected edges} is maximized, which is different from the former. Please refer to Section~\ref{sec:relatedwork} for more details.




It is very challenging to solve the \short{} problem  because the choice space is extremely large.
%We prove that the \short{} problem is NP-hard under the classical information diffusion model - Independent Cascade (IC) model~\cite{Kempe03}. \shixun{mention IC in next senetences.}
To solve this problem, we try to insert limited links from the original network into the diffusion network that is initially empty.
%Initially the diffusion network contains only seed users, and we try to insert limited links from the original network into this diffusion network to maximize the seeds' influence under the classical Independent Cascade (IC) model~\cite{Kempe03}. 
Unfortunately, we find that greedily inserting edges with the maximum marginal gains w.r.t. influence of seeds is not effective, due to the non-submodular property of the objective function and the expensive marginal gain computations under the classical Independent Cascade (IC) model~\cite{Kempe03}. Thus, we resort to computing and leveraging influence lower bounds, and by using such lower bounds the submodular property can be preserved. Afterwards, we propose a novel diffusion network augmentation method which consists of two stages, namely the expansion stage and the filling stage. In the expansion stage, we iteratively expand the diffusion network size by incorporating the users and the connections that are important to spreading influence. In the filling stage, we intelligently fill up link recommendations for these involved users. Our contributions are summarized as below:

%Thus, we resort to an existing model called the restrict maximum probability path (RMPP) model~\cite{chaoji2012recommendations} which can efficiently estimate the lower bound of influence under the IC model and preserves submodularity. Despite the simplicity of this model, directly using this model is still not effective since influence is not allowed to spread via any path with more than one inserted edges. As a result,it will restrict the seeds' influence spread within one-hop neighborhood only. 

%To alleviate this issue, we propose a novel diffusion network augmentation method which embraces the benefits of the RMPP model while helping the influence reach considerable online users. Specifically, our method consists of two stages, namely the expansion stage and the filling stage. In the expansion stage, we iteratively treat inserted edges as an original part of the diffusion network, and expand the diffusion network size by incorporating users and connections that are important to spreading influence. In the filling stage, we intelligently fill up link recommendations for incorporated users. Our contributions are summarized as below, and we refer readers to the supplementary file for the proof of all theorems:
 \begin{itemize}[leftmargin=*]
\item We make the first attempt to study and formalize the problem of Influence Maximization in \emph{Closed} Social Networks (\short{}), motivated by numerous practical needs in social network platforms such as Tencent. We also prove its NP-hardness (Section~\ref{sec:preliminary}).

\item With an influence lower bound as the quality measurement, we first propose a network augmentation \emph{sketch} that can produce solutions for a single seed user with theoretical guarantees in a given diffusion network (Section~\ref{sec:methodsingle}.1). 
%However, this sketch is not practical in reality since it suffers from exorbitantly expensive costs of influence estimation caused by every decision making (i.e., each link recommendation). 
To boost the efficiency, we propose an effective yet scalable network augmentation method to avoid marginal gain computations (Section~\ref{sec:methodsingle}.2).  

\item We make some interesting observations in the influence diffusion of multiple seed users and leverage these observations to transform the \short{} problem for multiple seed users into the one for a single `virtual' seed user. Such a transformation enables us to utilize our method for a single seed user with minor adjustments, to produce effective solutions while maintaining high efficiency.

\item We conduct extensive experiments on real-world social networks including the deployment into a Tencent application (Section~\ref{sec:experiment}). We have several exciting findings: 

\noindent 1) In the \short{} problem, the boosted baselines, built upon the diffusion network produced by the expansion stage of our method, can achieve up to five-orders-of-magnitude larger influence spread than their counterparts built upon the initially empty network. Despite that, our full-stage method, which includes both the expansion and filling stages, significantly beats those boosted baselines. 
%\bao{full-stage is not explained earlier. Also think of whetehr we should present the name/acronym of each method, as former contributions keep referring to different methods for different settings, say single seed vs multi seed.}

 2) Our full-stage method is able to identify important connections for spreading influence -- it is able to build a diffusion network where seed users can achieve 90\% of their full influence in the original network and this diffusion network contains only 36\% of edges from the original one.
 
 3) We deploy our solution into an activity of an online Tencent application where each online user will be recommended some friends for interaction.
 We conduct online A/B testing where each user is randomly assigned to one method which produces the recommendation list for this user. Such interaction can unfold in cascades and further trigger more interaction if the recommendation is effective. The online result shows that the recommendation from our solution which achieves a notably better Click-through Rate than the rest of baselines.
 
 
  %where online users will be recommended a list of friends for interaction, our deployed method produces much more effective recommendation against baselines and achieves a notably better Click-through Rate.} \bao{The setting and evaluation of deployed scenario needs more details.}
 
  4) In solving the problem of maximizing the seeds' influence over \emph{open} social networks, by recommending limited \emph{new links}, our method achieves up to five-orders-of-magnitude speedup than the state-of-the-art while maintaining competitive effectiveness. 



\end{itemize}

==> imcsnvldb2023 copy/tex/macro.tex <==
\newcommand{\bao}[1]{{\color{blue}{\bf{Bao:}} \emph{#1}}} 
\newcommand{\junhao}[1]{{\color{CadmiumOrange}{\bf{Junhao:}} \emph{#1}}} 
\newcommand{\wenqing}[1]{{\color{ForestGreen}{\bf{Wenqing:}} \emph{#1}}} 
\newcommand{\shixun}[1]{{\color{WildStrawberry}{\bf{Shixun:}} \emph{#1}}}
\newcommand{\short}{IMCSN}
\newcommand{\ksubnetwork}{$k$-subnetwork}
\newcommand{\method}[1]{\textsf{#1}}
\newcommand{\rppr}[1]{p^{RP}_{#1}}
\newcommand{\sppr}[1]{p^{SP}_{#1}}
\newcommand{\innermethod}{\textsf{PEI}}
\newcommand{\outtermethod}{\textsf{PSNA}}



==> imcsnvldb2023 copy/tex/methodformultiple.tex <==
\section{Solving \short{} for multiple seeds}\label{sec:methodmultiple}
When there is a set $S$ of independent seed nodes, directly adopting the previous idea of inserting at most one incoming edge for each node is not feasible, since the SMPPs from seed nodes to the same node can be different and hence the critical edge for each node is seed-specific. The most straightfoward approach to handle the case is to iteratively insert the edge, which brings the maximum marginal gain to the sum of the influence increment of all seed nodes, until no edges can be inserted into the \ksubnetwork{}. However, this approach is impractical due to expensive marginal gain computation and a huge number of iterations needed to converge.  

\smallskip
\noindent \textbf{Observation 4}. We observe that an edge $(u,v)$ insertion can have different levels of impact on increasing the influence spread of different seed nodes. For example, if $u$ is a neighbor of the seed node $s_1$ but ten hops away from the seed node $s_2$, inserting $(u,v)$ is more likely to bring more influence to $s_1$ than $s_2$. Furthermore, as the iteration goes, the \ksubnetwork{} will be expanded with more topological information during the augmentation process. Thus, we should not `waste' many unnecessary recommendation opportunities in the current stage of the \ksubnetwork{} since they can be saved for better decision making in later iterations. 

Thus, to make the best use of candidate recommendations, we should  focus only on the recommendation which will bring large influence increment to the relevant seed node. Specifically, we define $r(u)=\argmax_{s\in S} \sppr{(s,u)}$ as the \emph{relevant seed node} of $u$ since inserting outgoing edges from $u$ would be more likely to increase the influence of the seed node $r(u)$. For all incoming neighbors of node $v$, we should connect the critical neighbor $u^*_v$ to $v$ which forms the RMPP with the maximum probability from the corresponding seed node $r(u^*_v)$, i.e., $u^*_v=\argmax_{ u\in N_{in}^{G_c}(v) }   \sppr{(r(u),u)} \cdot p_{(u,v)} $. 

Nodes with the same relevant seed node $s$ and SMPPs from $s$ to them naturally form an SMPP-based tree. We can construct the SMPP-based trees based on each seed node and these trees are disjoint (i.e., no node overlap). With these trees, we can compute the subtree size of each node in the corresponding tree and prioritize inserting the nodes with large subtree sizes, because increasing the probability to influence the node $u$ will also increase the probability to influence the descendants of $u$ in the SMPP-based trees.

\begin{figure}[t]
\centering
\subfloat[iteration $i$.]{
\includegraphics[width=0.2\textwidth]{./figures/examplemulti1}\hspace{-1em}
} 
\hspace{0.5mm}
\subfloat[iteration $i+1$.]{
\includegraphics[width=0.2\textwidth]{./figures/examplemulti2}\hspace{-1em}
}

\caption{SMPP-based subgraphs in two iterations.}\label{eg:subgraph}
\label{comparison}

\end{figure}



\begin{example}
Figure~\ref{eg:subgraph} shows an example of the SMPP-based trees of a 2-subnetwork in two consecutive iterations of the \outtermethod{}. Here, $a$, $b$ and $c$ are the seed nodes, all solid edges have a weight of 0.1, nodes with the same color belong to the same SMPP-based trees, and white nodes are candidates for the 2-subnetwork expansion. In iteration $i$, node $g$ is processed before $l$ because $g$ has a larger subtree size (i.e., 2).
We have two candidate incoming edges to node $g$, and $(f,g)$ will be inserted since $f=\argmax_{ u\in \{f,c\} }   \sppr{(r(u),u)} \cdot p_{(u,g)} $ where $r(f)=a$ and $r(c)=c$. In the input 2-subnetwork of iteration $i+1$, the relevant seed nodes of $g$ and $j$ are updated to node $a$ since inserting outgoing edges from them is more likely to increase the influence of $a$. 
\end{example}

The premise of the aforementioned idea requires computing the SMPP between each node $u$ and $r(u)$. A straightforward approach is to enumerate SMPPs from every seed node to $u$ and get the one with the greatest probability. However, this is very expensive in real-world large-scale social networks, especially when $|S|$ is large. To mitigate this issue, we can simply introduce edges with the same influence probability of 1 from a \emph{virtual} node $x$ to every seed node. Afterwards, we only need to adopt a variant of Dijkstra algorithm~\cite{chaoji2012recommendations} to compute the SMPPs from $x$ to the rest of the nodes; the second node in each SMPP must be a seed node, and be the relevant seed node of the end node of this path. With the virtual node $x$, we simplify the case of multiple seed nodes into the case of a single seed node $x$ since edge insertion can be guided by the probability of SMPP from $x$ instead of relevant seed nodes, i.e., 
%$u^*_v=\argmax_{ u\in N_{in}^{G_c}(v) }  1\cdot   \sppr{(r(u),u)} \cdot p_{(u,v)}= \argmax_{ u\in N_{in}^{G_c}(v) }   p_{(x,r(u))} \sppr{(r(u),u)} \cdot p_{(u,v)}=\argmax_{ u\in N_{in}^{G_c}(v) }   \sppr{(x,u)} \cdot p_{(u,v)}$.
$$u^*_v=\argmax_{ u\in N_{in}^{G_c}(v) }  1\cdot   \sppr{(r(u),u)} \cdot p_{(u,v)}=\argmax_{ u\in N_{in}^{G_c}(v) }   \sppr{(x,u)} \cdot p_{(u,v)}$$
%\begin{align*}
%u^*_v&=\argmax_{ u\in N_{in}^{G_c}(v) }  1\cdot   \sppr{(r(u),u)} \cdot p_{(u,v)}=\argmax_{ u\in N_{in}^{G_c}(v) }   \sppr{(x,u)} \cdot p_{(u,v)}\\
%&= \argmax_{ u\in N_{in}^{G_c}(v) }   p_{(x,r(u))}\cdot \sppr{(r(u),u)} \cdot p_{(u,v)}=\argmax_{ u\in N_{in}^{G_c}(v) }   \sppr{(x,u)} \cdot p_{(u,v)}\\
%&=\argmax_{ u\in N_{in}^{G_c}(v) }   \sppr{(x,u)} \cdot p_{(u,v)}
%\end{align*}
 Since we transform the \short{} problem for multiple seed nodes into the one for a single virtual node $x$, we can directly adopt \outtermethod{} for the single seed node with minor adjustments: (1) introduce $O(|S|)$ edges with the same influence probability 1 from a virtual node $x$ to every seed node in the initial \ksubnetwork{}; (2) remove the virtual node and edges between it and seed nodes from the output \ksubnetwork{} of \outtermethod{}. 
 \iffalse
 \begin{enumerate}[leftmargin = *]
 \item introduce $O(|S|)$ edges with the same influence probability 1 from a virtual node $x$ to every seed node in the initial \ksubnetwork{}; 
 \item remove the virtual node and edges between it and seed nodes from the output \ksubnetwork{} of \outtermethod{}. 
 \end{enumerate}
\fi

 \noindent\textbf{Time Complexity}.~Considering that we only change the topology of the \ksubnetwork{}, the previous time complexity analysis for the single case still applies. Thus, the total time complexity is $O(I(|V|+|E|+|S|)\log |V|+|V|d_{m}\log d_{m} )$.


==> imcsnvldb2023 copy/tex/methodforsingle.tex <==
\section{Solving \short{} for a single seed}\label{sec:methodsingle}
To facilitate the illustration of our methodology, we first describe how to solve the \short{} problem for 
a single seed user. In the next section, we will describe how to extend the method to handle multiple seed users. 
Essentially, we try to solve the \short{} problem by inserting edges from the original network into a \ksubnetwork{} which initially contains the seed user only. As mentioned in Section~\ref{sec:intro}, we resort to the influence lower bounds to preserve submodularity, and the lower bounds are computed with the Restricted Maximum Probability Path (RMPP) model~\cite{chaoji2012recommendations} as defined below. 

%Since the marginal gain of inserting an edge w.r.t. influence of the seed under the IC model is not submodular~\cite{chaoji2012recommendations}, the classical greedy which iteratively inserts an edge with the maximum marginal gain does not provide any approximate solution. To solve the \short{} problem efficiently and effectively, we resort to leveraging the Restricted Maximum Probability Path (RMPP) model (defined as below) which provides efficient lowerbound estimation of influence spread under the IC model and preserves the submodularity~\cite{chaoji2012recommendations}. To avoid any confusion, we use $\delta^\triangle()$ as the influence measure under the RMPP model. 


\begin{definition}[Influence Probability of a path]
The influence probability of a path is the product of influence probabilities of all edges in this path.
\end{definition}

\begin{definition}[Restricted Maximum Probability Path (RMPP)~\cite{chaoji2012recommendations}]\label{defn:rmpp}
Given a \ksubnetwork{} $G_k$ where edges are either native (i.e., originally exist) or inserted, and a seed node $s$, the restricted maximum probability path $RMPP(s,u)$ is the directed path from $s$ to $u$ whose probability
$\rppr{(s,u)}$ is the maximum among all paths from $s$ to $u$ containing at most one inserted edge. Ties are broken arbitrarily.
\end{definition}

\begin{definition}[RMPP model~\cite{chaoji2012recommendations}]
In the RMPP model, the influence of a seed node $s$ to a node $u$ is the influence probability $\rppr{(s,u)}$ of $RMPP(s,u)$, and the total influence of $s$ is the sum of influence probabilities of all RMPPs from $s$ to the rest of nodes in the graph.
\end{definition}

\begin{figure}[!t]

\centering
\includegraphics[width=0.2\textwidth]{./figures/rmppexample}\hspace{-1em}
%\vspace{-1em}
\caption{A simple network where dashed edges are candidates for insertion.} 
\label{fig:rmppexample}
\end{figure}



\begin{example}\label{rmpp_example}
As shown in Figure~\ref{fig:rmppexample}, we have a network which contains five nodes and two native edges $(s,b)$ and $(b,c)$ with the same influence probability of 0.5. Suppose the seed node is $s$, three edge candidates $(s,c)$,$(c,d)$ and $(d,e)$ have the same influence probability of 1,  $T_1=\emptyset$ and $T_2=\{(s,c),(c,d)\}$. 
The marginal gain of $(s,c)$ over $T_1$ is 1-0.25=0.75 since $RMPP(s,c)$ is edge $(s,c)$. However, the marginal gain of $(d,e)$ over $T_2$ is 0 since $s$ needs to traverse at least two inserted edges to reach $e$, which is not allowed in the RMPP model. 
\end{example}



\begin{algorithm}[!t]
 %\algsetup{linenosize=\normalsize}
\small
 \caption{\method{SubnetworkAugmentationSketch}}\label{alg:initialframework}
   \SetKwInOut{Input}{Input}
   \SetKwInOut{Output}{Output}
 \Input{The input network $G$, the seed user $s$ and an integer $k$.}
  \Output{The \ksubnetwork{} $G_k$.}
  
$G_k=(V_k.E_k) \leftarrow $ \ksubnetwork{} containing the seed $s$ only\;
%$G_c \leftarrow $ the candidate network which contains all outgoing edges from $s$ in $G$\;
 %$preInf=\delta^\triangle_{G_k}(t)$\;
 
 \While{ $\exists v \in V_k , |N_{out}^{G_k}(v) | < min(k,|N_{out}^{G}(v)| )$   }{
  $G_k=$ {\method{EdgeInsertionSketch}}$(G,G_k,s,k)$\;
 } 
 
  Return $G_k$\; 
\end{algorithm}

RMPP provides an efficient lower bound estimation of influence spread under the IC model and preserves the submodularity~\cite{chaoji2012recommendations}. 
%
Unfortunately, directly adopting the RMPP model to insert edges into the \ksubnetwork{} which initially contains only the seed node $s$ does not help to achieve great influence spread. This is because $s$ has to traverse two inserted edges to reach the nodes that are two hops away, but this is not permitted in the RMPP model, as illustrated in Example~\ref{rmpp_example}. 

To mitigate this issue without missing the opportunity of leveraging the submodularity property of the RMPP model, we propose a subnetwork augmentation sketch in Algorithm~\ref{alg:initialframework}. Specifically, this sketch iteratively calls a strategy called \method{EdgeInsertionSketch} in the pseudocode. This strategy tries to insert edges to increase the influence spread of the seed node $s$ under the RMPP model and uses these inserted edges to update the input \ksubnetwork{} $G_k$. After reaching a termination condition, these \emph{inserted} edges will be treated as \emph{native} edges of $G_k$ in the next iteration, which will help $s$ to influence the nodes that are many hops away. In what follows, we will introduce how the method \method{EdgeInsertionSketch} works and then propose a much more efficient yet practical edge insertion strategy (Section~\ref{sec:edgeinsertion}). Afterwards, we will further optimize this subnetwork augmentation sketch (Section~\ref{sec:augmentation}).



\subsection{Edge Insertion}\label{sec:edgeinsertion}
Given a candidate network $G_c$ that contains candidate edges to be inserted into the current \ksubnetwork{} $G_k$, the most straightforward way to maximize the influence of $s$ is to greedily insert an edge with the maximum marginal gain into $G_k$ without breaking the constraint of \ksubnetwork{}. This approach suffers from serious scalability issues since it needs to update the marginal gain of all candidate edges in each iteration and the marginal gain computation of each edge incurs $O((V_k+E_k)\log V_k)$ time complexity with a variant of Dijkstra algorithm as in~\cite{chaoji2012recommendations}. To address this issue, we first present an edge insertion sketch from the theoretical point of view, followed by a practical insertion method.

%In terms of the limited size of $G_k$ and limited influence spread, the naive approach will try to insert as many edges as possible into the current $G_k$. This behavior has two serious issues. First, nodes in $G_k$ may not be able to reach new nodes in $G$ so as to expand the size of $G_k$ without breaking the \ksubnetwork{} constraint. Second, the recommendation quality based on current $G_k$ may not be better than the one in augmented $G_k$ with more nodes and topological information. 
 
 
 
 \begin{algorithm}[!t]
  % \algsetup{linenosize=\footnotesize}
 \small
  \caption{ \method{EdgeInsertionSketch}}\label{alg:networkaugmentation}
    \SetKwInOut{Input}{Input}
    \SetKwInOut{Output}{Output}
   \Input{The input network $G=(V,E)$, the current \ksubnetwork{} $G_k=(V_k,E_k)$, the seed user $s$ and an integer $k$.}
   \Output{The updated \ksubnetwork{} $G_k$.}
 
 %$G_d \leftarrow $ initialize the diffusion network from $G$ where the out-neighbors of any node is not greater than $k$\;
 $\mathcal{C} \leftarrow $candidate set initialized as $\emptyset$\;
 \ForEach{ node $u \in G_k$}{
   \If{$|N^{G_k}_{out}(u)|<min(k,|N^{G}_{out}(u)|)$}{
     \ForEach{ $(u,v) \in E$ }{
       \If{$(u,v) \notin E_k $ and $v \neq s$}{
         Add $(u,v)$ into $\mathcal{C}$
       }
     
     }
   }
 
 }
 
 $G_c=\{V_c,E_c\} \leftarrow $ construct candidate graph based on $\mathcal{C}$\;
 
 Compute the probabilities of SMPPs from $s$ to all nodes in $G_k$ \;
 
 \ForEach{node $v \in V_c$ with $|N^{G_c}_{in}(v)|>0$}{
   $u^*_v= \argmax_{u \in N^{G_c}_{in}(v)} \sppr{(s,u)} \cdot p_{(u,v)} $\;
 }
 
 \While{$G_c$ has nodes with incoming neighbors}{
        
        $v^*= \argmax_{v \in V_c, |N^{G_c}_{in}(v)|>0}  \delta_{G_k \cup \{(u^*_v,v)\} }^\triangle (s) -  \delta_{G_k}^\triangle (s)$\;
 
 
   
     Remove all incoming edges to $v^*$ from $G_c$\; 
     Insert $(u^*_{v^*},v^*)$ into $G_k$\;
     
     \If{$|N^{G_k}_{out}(u^*_{v^*})|=min(k,|N^{G}_{out}(u^*_{v^*})|)$}{
       \ForEach{$v \in N^{G_c}_{out}(u^*_{v^*})$}{
         \lIf{$u^*_v=u^*_{v^*}$}{
                 Update $u^*_v$
         }
         Remove $(u^*_{v^*},v)$ from $G_c$\;
       }
     }
 }
 
 Mark all inserted edges as native\;
 
 
 \Return $G_k$\;
 
 
 \end{algorithm}
 
 
 \subsubsection{Edge Insertion Sketch}
 
Later in Theorem~\ref{theorem:critical}, we prove that for all candidate edges that share the same destination node, we can carefully insert the \emph{critical} edge (which will be defined in Definition~\ref{defn:criticalneighborandedge}) such that inserting other edges after this critical edge will not increase the influence spread of $s$ under the RMPP model. With this observation, we only need to compare the marginal gain of critical edges with different destination nodes in each iteration. Hence, the cost of marginal gain computation can be greatly reduced. %The correctness of Theorem~\ref{theorem:critical} is established based on Lemma~\ref{theorem:pair} and Lemma~\ref{theorem:marginalgain}. 
To facilitate the presentation of our method, we use $\delta^\triangle()$ as the influence under the RMPP model, and introduce a concept, namely \emph{Strict Maximum Probability Path (SMPP)}. 

\begin{definition}[Strict Maximum Probability Path (SMPP)]\label{def:smpp}
  Given a seed node $s$ and a \ksubnetwork{} $G_k$ where edges are either native or inserted, the strict maximum probability path $SMPP(s,u)$ is a directed path from $s$ to $u$ whose probability $\sppr{(s,u)}$ is the maximum among all the paths from $s$ to $u$ containing native edges only (i.e., a special case of RMPP). Ties are broken arbitrarily.
  \end{definition}
  
 \begin{example}
As shown in Figure~\ref{fig:rmppexample}, $SMPP(s,c)$ consists of two native edges, namely $(s,b)$ and $(b,c)$. $SMPP(s,c)$ remains unchanged even after we insert edge $(s,c)$, since the inserted edge is not native.
 \end{example} 
  



The algorithm to be introduced is based on Theorem~\ref{theorem:critical} which is in turn established upon  Lemma~\ref{theorem:pair} and Lemma~\ref{theorem:marginalgain} below. 

\begin{lemma}\label{theorem:pair}
Given a \ksubnetwork{} $G_k$, a seed node $s$, and two candidate edges $(u,v)$ and $(u',v)$ which are in the candidate network $G_c$ and share the same endpoint $v$, and $\rppr{(s,x)}(u,v)$ which denotes the probability of $RMPP(s,x)$ after inserting the edge $(u,v)$ into $G_k$, if $ \sppr{(s,u)}\cdot p_{(u,v)} \geq \allowbreak \sppr{(s,u')} \cdot p_{(u',v)} ,$
then for any node $x$ which can be reached by $v$ via directed paths, 
$\rppr{(s,x)}(u,v)  \geq \rppr{(s,x)}(u',v) $.
\end{lemma}



\begin{proof}
If the $RMPP(s,x)$ from $s$ to $x$ remains the same after inserting $(u,v)$ and $(u',v)$, the influence probability of $x$ will remain unchanged, i.e., $\rppr{(s,x)}(u,v) = \rppr{(s,x)}(u',v)$.

If the $RMPP(s,x)$ from $s$ to $x$ is changed after inserting $(u,v)$ or $(u',v)$, the $RMPP$ must contain $(u,v)$ or $(u',v)$. Let $RMPP_{(u,v)}$ and $RMPP_{(u',v)}$ denote the \emph{updated} $RMPP$ from $s$ to $x$ by inserting edge $(u,v)$ and $(u',v)$ respectively. Each of these two $RMPP$s consist of two sub-paths. That is, $P_1(RMPP_{(u,v)})=[s,...,u,v]$,  $P_2(RMPP_{(u,v)})=[v,...,x]$, $P_1(RMPP_{(u',v)})=[s,...,u',v]$ and $P_2(RMPP_{(u',v)})=[v,...,x]$. Based on Definition~\ref{defn:rmpp}, the second paths of both 
$RMPP$s do not contain inserted edges. Thus, $P_2(RMPP_{(u,v)})$ and $P_2(RMPP_{(u',v)})$ have the same probability. 
Since $\sppr{(s,u)}\cdot p_{(u,v)}$ and $\sppr{(s,u')}\cdot p_{(u',v)} $ refer to the probability of the first sub-paths of these two RMPPs respectively and the former one is not smaller than the latter, we have $\rppr{(s,x)}(u,v)  \geq \rppr{(s,x)}(u',v)$.
\end{proof}



\begin{lemma}\label{theorem:marginalgain}
Given a \ksubnetwork{} $G_k$, a seed node $s$, and two candidate edges $(u,v)$ and $(u',v)$ which are in the candidate network $G_c$ and share the same endpoint $v$, if $\sppr{(s,u)}p_{(u,v)} \geq \allowbreak \sppr{(s,u')} p_{(u',v)} $, $\delta_{G_k \cup \{(u,v)\}}^\triangle(s)=\delta_{G_k \cup \{(u,v),(u',v) \}}^\triangle(s)$.
\end{lemma}

\begin{proof}
Based on Lemma~\ref{theorem:pair}, for any node $x$ that can be reached by $v$, the influence probability $\rppr{(s,x)}$ of $RMPP(s,x)$ under $G _k\cup \{(u,v)\}$ is never smaller than that under $G_k \cup \{(u',v)\}$. 
Thus, introducing $\{(u',v)\}$ after inserting $(u,v)$ does not contribute to the influence increment of $s$. Thus, $\delta_{G_k \cup \{(u,v)\}}^\triangle(s)=\delta_{G_k \cup \{(u,v),(u',v) \}}^\triangle(s)$.
\end{proof}


To better describe Theorem~\ref{theorem:critical} later, we have the definition below.


\begin{definition}[critical neighbor and edge]\label{defn:criticalneighborandedge}
Given a \ksubnetwork{} $G_k$, the seed node $s$, the candidate network $G_c$ and a node $v$, if $|N^{G_c}_{in}(v)|>0$, the critical neighbor $u^*_v$ of $v$ in $G_c$ is the neighbor whose SMPP path probability $\sppr{(s,u^*_v)}$ times the influence probability $p_{(u^*_v,v)}$ of the edge $(u^*_v,v)$ is the greatest among all the incoming neighbors of $v$ in $G_c$. That is, $u^*_v= \argmax_{ u \in N^{G_c}_{in}(v)} \sppr{(s,u)}\cdot p_{(u,v)}$. Correspondingly, the incoming edge $(u^*_v,v)$ is the critical edge of $v$.

\end{definition}



\begin{theorem}\label{theorem:critical}
Given a \ksubnetwork{} $G_k$, the seed node $s$, a node $v$, a candidate set $E'=\{ (u,v)| u \in N^{G_c}_{in}(v)   \}$ for insertion and the critical edge $(u^*_v,v)$, we have: $\delta^\triangle_{G_k \cup E'}(s)=\delta^\triangle_{G_k \cup \{(u^*_v,v)\}}(s)$.
\end{theorem}


\begin{proof}
Since $(u^*_v,v)$ is the critical edge, $\sppr{(s,u^*_v)}\cdot p_{(u^*_v,v)}$ is the greatest among all the incoming neighbors of $v$ in $G_c$. Based on Lemma~\ref{theorem:marginalgain}, we can know that, after inserting $(u^*_v,v)$, introducing edges sharing the same destination node as $(u^*_v,v)$ will not increase the RMPP-based influence. Thus, this theorem is deduced.
%\sout{Based on Lemma~\ref{theorem:marginalgain}, after inserting $(u^*_v,v)$, introducing edges sharing the same destination node as $(u^*_v,v)$ will not increase the RMPP-based influence. The reason is that, among paths which contain an edge in $E'$ and start from $s$ to any node reached by $v$, the one with the maximum probability must contain $(u^*_v,v)$. Thus, Theorem~\ref{theorem:critical} is deduced.}
\end{proof}







%\begin{proof}
%Please refer to Appendix~\ref{appendix:proofcritical} for details.
%\end{proof}



Algorithm~\ref{alg:networkaugmentation} describes the process of edge insertion sketch by leveraging Theorem~\ref{theorem:critical}. Lines 1-7 construct the candidate graph $G_c$ containing the candidate edges which can be inserted into $G_k$. $G_c$ only contains the edges between nodes in $G_k$ and their neighbors in $G$, since nodes in $G_k$ cannot reach their two-hop neighbors in $G$ with only one inserted edge. Lines 8-10 compute the critical incoming neighbor for each node in $G_c$, and Lines 11-18 iteratively insert the critical edge with the maximum marginal gain into $G_k$ until all the critical edges have been inserted.

\smallskip
\noindent \textbf{Theoretical Guarantee}. Maximizing the influence spread of $s$ in the given $G_k$ under the RMPP model is already a submodular set function maximization problem with partition matroids constraint. That is, we are only allowed to pick a single edge from edges with the same destination/end node. Thus, the greedy approach (i.e., Algorithm~\ref{alg:networkaugmentation}) naturally leads to a 1/2 approximation ratio~\cite{goundan2007revisiting}. 

\smallskip
\noindent \textbf{Time Complexity}.
There are at most $O(|V|)$ iterations and each iteration takes $O(|V| (|V|+|E| )\log |V| )$ to find the critical edge with the maximum marginal gain via a variant of Dijkstra algorithm~\cite{chaoji2012recommendations}. Thus, Algorithm~\ref{alg:networkaugmentation} takes $O(|V|^2  (|V|+|E| )\log |V| )$ time. 

%\noindent \textbf{Time Complexity}. Despite the effectiveness, Algorithm~\ref{alg:networkaugmentation} still suffers from the scalability issue since the size of critical edges can be huge. Specifically, there are at most $O(|V|)$ iterations and each iteration takes $O(|V| (|V|+|E| )\log |V| )$ to compute find the critical edge with the maximum marginal gain via a variant of Dijkstra algorithm~\cite{chaoji2012recommendations}. Thus, Algorithm~\ref{alg:networkaugmentation}, which takes $O(|V|^2  (|V|+|E| )\log |V| )$ time, is infeasible in real-world large-scale social networks. 

%Furthermore, when we consider multiple seed nodes, the critical edge, the probability of SMPPs and RMPPs depend on the specific seed nodes which further make 



\begin{algorithm}[!t] 
%  \algsetup{linenosize=\footnotesize}
\small
 \caption{ \method{PracticalEdgeInsertion (\innermethod{})} }\label{alg:networkaugmentationpractical}
   \SetKwInOut{Input}{Input}
   \SetKwInOut{Output}{Output}
  \Input{The input network $G=(V,E)$, the current \ksubnetwork{} $G_k=(V_k,E_k)$, the seed user $s$ and an integer $k$.}
  \Output{The updated \ksubnetwork{} $G_k$.}

%$G_d \leftarrow $ initialize the diffusion network from $G$ where the out-neighbors of any node is not greater than $k$\;


$G_c=\{V_c,E_c\} \leftarrow $ constructs the candidate graph as in Algorithm~\ref{alg:networkaugmentation}\;

 $L \leftarrow$ nodes in $G_k$ excluding $s$, ranked by their subtree sizes of in the SMPP-based tree in non-increasing order\;
 $L' \leftarrow $ nodes, that are in $G_c$ but not in $G_k$, ranked by their out-degrees in non-increasing order\;
 $L \leftarrow $ Append $L'$ to the end of $L$\;

\ForEach{$v$ in $L$}{
  \lIf{$|N^{G_c}_{in}(v)|=0$}{Continue}

  $u^*_v= \argmax_{u \in N^{G_c}_{in}(v)}  \sppr{(s,u)} \cdot p_{(u,v)} $\;

  Add $(u^*_v,v)$ into $G_k$, and remove $(u^*_v,v)$ from $G_c$\;
    \If{$|N^{G_k}_{out}(u^*_{v})|=min(k,|N^{G}_{out}(u^*_{v})|)$}{
    Delete all outgoing edges of $u^*_v$ from $G_c$.
  
  }
  
  Mark all inserted edges as native\;

}
\Return $G_k$\;

\end{algorithm}


\subsubsection{Practical Edge Insertion}\label{sec:praticaledgeinsertion}
%\sout{Due to the high time complexity,  Algorithm~\ref{alg:networkaugmentation} is infeasible in real-world large-scale social networks. To alleviate this scalability issue, we next present a practical edge insertion strategy which is highly efficient and effective. Particularly, the main bottleneck of Algorithm~\ref{alg:networkaugmentation} lies in iteratively finding and inserting the \emph{critical} edge with the maximum marginal gain. We find that in the ideal case (i.e., Theorem~\ref{theorem:idealcase}), we do not need to compute the marginal gain. Instead, we can directly insert all critical edges identified based on the initial candidate graph $G_c$ to achieve the maximum influence spread.}


Algorithm~\ref{alg:networkaugmentation} suffers from very high time complexity and thus is infeasible in real-world large-scale social networks. In each iteration, Algorithm~\ref{alg:networkaugmentation} tries to insert a critical incoming edge to a node with the maximum marginal gain w.r.t. the influence, and correspondingly update the candidate network which can result in updates of critical edges of the remaining nodes and the marginal gain of each critical edge (Lines 11-18). We observe that the nodes considered across all iterations actually form an order. If the order is known in advance, we can directly follow this order to insert critical edges \emph{without} marginal gain computation and comparison, and hence the whole process can be notably accelerated. Unfortunately, computing this order is the main efficiency bottleneck of Algorithm~\ref{alg:networkaugmentation}. %and requires iteratively updating critical edges of remaining nodes and their marginal gains.

We find that in the special case below (i.e., Theorem~\ref{theorem:idealcase}), there is no need to know this order because, no matter what the order is, the critical edge of any remaining node will not be updated in the iterative insertion process.




\begin{theorem}\label{theorem:idealcase}
Given the original network $G$, a \ksubnetwork{} $G_k$, the initial candidate network $G_c=\{V_c,E_c\}$ (i.e., Line 7 in Algorithm~\ref{alg:networkaugmentation}), the seed node $s$, and $Cr(x)=\{ v |  \forall v \in V_c, x= u^*_v\}  $ which denotes the set of nodes whose critical neighbor is $x$. If $\forall x \in V_c, |Cr(x)| \leq min(k,N^{G}_{out}(x))- N^{G_k}_{out}(x) $, then directly inserting all critical edges leads to the optimal solution with the maximum influence. 
\end{theorem}

\begin{proof}
Since $min(k,N^{G}_{out}(x))$ describes the maximum number of outgoing edges from $x$ allowed in $G_k$,  $ N^{G_k}_{out}(x) $ describes how many of them have already been inserted into $G_k$, and $\forall x \in V_c, |Cr(x)| \\ \leq min(k,N^{G}_{out}(x)) \allowbreak - N^{G_k}_{out}(x) $, inserting all critical edges in $Cr(x)$ will not result in the critical edge/neighbor update of the rest nodes (i.e., Line 17 in Algorithm~\ref{alg:networkaugmentation}). Based on Theorem~\ref{theorem:critical}, directly inserting critical edges of all nodes leads to the maximum influence spread since replacing any critical edges with the remaining edge candidates or inserting more edges will not increase influence.  
\end{proof}

In the special case above, directly inserting all critical edges produces the optimal solution as Algorithm~\ref{alg:networkaugmentation} which does not need to update the critical edges (Line 17) in each iteration. Although this special case is rather rare in practice, it inspires us to find an order which can be easily obtained in prior and follow this order to insert an incoming edge $(u,v)$ for each node $v$ whose $\sppr{(s,u)} \cdot p_{(u,v)}$ is as large as possible. Ideally, this strategy is expected to effectively approximate Algorithm~\ref{alg:networkaugmentation}. We make the following observation to guide us to find such an order.


%Although this ideal case is rather rare in practice, it inspires us to insert an incoming edge $(u,v)$ for each node $v$ whose $\sppr{(s,u)} \cdot p_{(u,v)}$ is as close as possible to the one of $(u^*_v,v )$ identified based on the initial candidate network (i.e., line 7 in Algorithm~\ref{alg:networkaugmentation}). {\color{brown} (highlight for reminding) If we can find a proper order of inserting the incoming edge for each node, it is possible to avoid repeatedly estimating the marginal gain and the solution would effectively approximate Algorithm~\ref{alg:networkaugmentation}.

\smallskip
\noindent \textbf{Observation 1}. If the insertion of an edge $(u,v)$ introduces an $RMPP(s,v)$ with an influence probability greater than that of the $SMPP(s,v)$, for any node $x$ which $s$ needs to reach via $v$, the insertion of $(u,v)$ could also introduce $RMPP(s,x)$ with a greater influence probability than $SMPP(s,x)$.


%If the insertion of an edge $(u,v)$ introduces an $RMPP(s,v)$ with greater influence probability than that of the $SMPP$ from $s$ to $v$, such an edge insertion would also introduce more influential RMPPs from $s$ to nodes reached by $v$ via SMPPs. 

Based on this observation, we should prioritize inserting incoming edges for nodes which \emph{appear} in a large number of SMPPs from $s$ to different nodes since such insertions could potentially increase the influence probabilities of the $RMPPs$ from $s$ to a large number of nodes. Based on Definition~\ref{def:smpp}, the graph formed by all SMPPs is a tree rooted at $s$, namely \emph{SMPP-based tree}, because any two nodes are connected by exactly one path. Thus, we can compute the appearance frequency by estimating the subtree size rooted at each node in the SMPP-based tree, which can be realized by a depth-first search and dynamic programming in $O(|E_k|)$ time. To help the influence spread reach a large number of users, we should also consider nodes in $G_c$ which have not been included in the \ksubnetwork{}. For these nodes, their subtree sizes are set as 0 and ranked based on their out-degrees in the input network $G$ since nodes with greater out-degrees have larger potentials to expand the \ksubnetwork{}. Algorithm~\ref{alg:networkaugmentationpractical} describes the overall process of practical edge insertion.


\begin{figure}[!t]

\centering
\includegraphics[width=0.4\textwidth]{./figures/EIexample}\hspace{-1em}
%\vspace{-1em}
\caption{An example of a candidate network $G_c$ with $k=2$.} 
\label{fig:EIexample}
\end{figure}


\begin{example}\label{example:EI}
Figure~\ref{fig:EIexample} shows a candidate network $G_c$ with $k=2$. The information needed by Algorithm~\ref{alg:networkaugmentationpractical} is listed at the right side. Nodes are ordered by their subtree sizes and then out-degrees. Thus, the node ranking we follow to insert incoming edges is $e,d,f$ and $g$. When we consider node $e$, edge $(b,e)$ will be inserted into $G_k$ and edge $(b,d)$ will be deleted from $G_c$ since $N^{G_k}_{out}(b)$ will become $2=k$. When we consider $d$, edge $(a,d)$ will be inserted. Similarly, edge $(c,f)$ will be inserted but edge $(c,g)$ will be deleted when we consider node $f$ and thus there will not be incoming edge candidates for $g$.
\end{example}



\smallskip
\noindent \textbf{Time Complexity}. In Algorithm~\ref{alg:networkaugmentationpractical}, Line 1 constructs the candidate graph in $O(|V|+|E|)$ time, Lines 2-4 rank nodes based on their subtree sizes in the SMPP-based tree or degrees in $ O((|V|+|E|)\log |V|) $ time, and Lines 5-10 iteratively insert incoming edges for ranked nodes in $O(|V|+|E|)$ time since the probabilities of all SMPPs from $s$ have already been computed when we construct the SMPP-based tree in Line 2. Thus, the total time complexity is $O((|V|+|E|)\log |V|) $. 





%\noindent \textbf{Time Complexity}. Algorithm~\ref{alg:networkaugmentationpractical} describes the overall procedure of the practical edge insertion method called \innermethod{}. Line 1 constructs the candidate graph in $O(|V|+|E|)$ time, lines 2-4 rank nodes based on their subtree sizes in the SMPP-based tree or degrees in $ O((|V|+|E|)\log |V|) $ time, and lines 5-10 iteratively insert incoming edges for ranked nodes in $O(|V|+|E|)$ time since critical edges were already identified when we construct the SMPP-based tree in line 2. Thus, the total time complexity is $O((|V|+|E|)\log |V|) $. 


\begin{algorithm}[!t]
 \algsetup{linenosize=\footnotesize}
\small
 \caption{\method{PracticalSubnetworkAugmentation (\outtermethod{})}}\label{alg:practicalframework}
   \SetKwInOut{Input}{Input}
   \SetKwInOut{Output}{Output}
 \Input{The input network $G$, the seed user $s$, an integer $k$ and an error ratio $\epsilon$.}
  \Output{The \ksubnetwork{} $G_k$.}
  
$G_k=(V_k.E_k) \leftarrow $ \ksubnetwork{} containing the seed $s$ only\;
$G_c=(V_c,E_c) \leftarrow $ all outgoing edges of $s$ in $G$\;
$L' \leftarrow$ all outgoing neighbors of $s$ in $G$\;
%$G_c \leftarrow $ the candidate network which contains all outgoing edges from $s$ in $G$\;
 ${\delta^\triangle_{pre}}=1$\;

 \If(\tcp*[h]{\fontfamily{lmr}\selectfont \small expansion stage}){$G_c$ has edges }{ 
 
  {$G_k$= \innermethod{}$(G,G_k,G_c,s,k,L')$} 
 
  \lIf{$ (\delta^\triangle_{G_k}(s)-\delta^\triangle_{pre})/\delta^\triangle_{pre}\leq \epsilon   $}{
    Break
  }
  \lElse{$\delta^\triangle_{pre}=\delta^\triangle_{G_k}(s)$}
  
  {$G_c, L'=$ \method{UpdateCandidateGraph}$(G,G_k,G_c,s,L')$}\;
  
  
 }
 
$G_k$={ \method{FUR}}$(G,G_k,G_c,s)$\tcp*[h]{\fontfamily{cmr}\selectfont \small filling stage}


  Return $G_k$\; 
\end{algorithm}

\iffalse
\begin{algorithm}[!t]
 \algsetup{linenosize=\footnotesize}
\footnotesize
 \caption{UpdateCandidateGraph}\label{alg:candidateupdate}
   \SetKwInOut{Input}{Input}
   \SetKwInOut{Output}{Output}
 \Input{The input network $G$, the \ksubnetwork{} $G_k$, the candidate graph $G_c$ and the seed user $s$, a set $L'$ of candidate nodes to be included into $G_k$.}
  \Output{The set of candidate nodes for $G_k$ expansion.}
  $L \leftarrow \emptyset$\;
  $L' \leftarrow$ Remove all nodes not in $G_k$ from $L'$ \;
  \ForEach{$u \in L'$}{
  
      \ForEach{$v \in  N^{G}_{out}(u) $}{
        \If{$(u,v) \notin E_k$ and $v \neq s$}{
          \lIf{$v \notin V_k$}{ Add $v$ into $L$}
        
          Add $(u,v)$ into $G_c$\;
        }
      
      
      }
  
  
  
  } 



  Return $L$ \; 
\end{algorithm}
\fi

\begin{algorithm}[!t]
 \algsetup{linenosize=\footnotesize}
\small
 \caption{\method{FillUpRecommendation (FUR)}}\label{alg:fillup}
   \SetKwInOut{Input}{Input}
   \SetKwInOut{Output}{Output}
 \Input{The input network $G$, the \ksubnetwork{} $G_k$, the candidate graph $G_c$ and the seed user $s$.}
  \Output{The updated $G_k$.}
  
  \ForEach{$v \in V_k$ where $|N_{in}^{G_k}(v) |>0$}{
     ${L^{in}[v] }\leftarrow$ a list of incoming neighbors of $v$ in $G_c$ where each neighbor $u$ is sorted by $\sppr{(s,u)} \cdot p_{(u,v)}$ in descending order\; 
    ${I[v]}=1$\;
    
  }
  
  $L \leftarrow$ a list of nodes in $V_k$ ordered by their subtree sizes in the graph formed by SMPPs from $s$ in descending order\;
  
  \While{$L$ is not empty}{
      $L' \leftarrow $ an empty list\;
      
      \ForEach{$v$ in $L$}{
      
        \ForEach{$i$ from $I[v]$ to $|L^{in}[v]|$ }{
          $u=L^{in}[v][i]$\;
          \lIf{$(u,v) \notin E_c$}{ Continue}
          \lIf{ $i \neq |L^{in}[v]|$ }{ Add $v$ into $L'$ }
          $I[v]=i+1$\; 
          Add $(u,v)$ into $G_k$; Remove $(u,v)$ from $G_c$\;
            \If{$|N^{G_k}_{out}(u)|=min(k,|N^{G}_{out}(u)|)$}{
              Delete all outgoing edges of $u$ from $G_c$.
            
            }
           Break\;
        
        }
      
      }
      
      $L=L'$\;
  
  }

  Return $G_k$\; 
\end{algorithm}

\subsection{Subnetwork Augmentation}\label{sec:augmentation}
%Even though Algorithm~\ref{alg:networkaugmentationpractical} achieves high efficiency, the construction of the candidate graph incurs notable overhead. We observe that actually the candidate graph constructed in the current iteration has notable edge overlap with the one in the previous iteration of the subnetwork augmentation sketch. Thus, we just need to capture their difference and partially update the candidate graph. In this section, we will design a practical subnetwork augmentation method which incorporates this idea.  

The subnetwork augmentation sketch (i.e., Algorithm~\ref{alg:initialframework}) suffers from two issues which incur notable computation costs. 
\begin{itemize}[noitemsep,leftmargin=*]
\item Issue 1: the candidate graph in each iteration is constructed from scratch without leveraging the candidate graphs generated in previous iterations. 
\item Issue 2: the number of edge insertions in each iteration is very limited (i.e., at most one incoming edge for each node) such that it may take considerable iterations to fill up the recommendations. 
\end{itemize}

\smallskip
\noindent \textbf{Observation 2}. Regarding Issue 1, we observe that the remaining candidate graph updated by \innermethod{} (i.e., Algorithm~\ref{alg:networkaugmentationpractical}) in the last iteration is a subgraph of the input candidate graph of \innermethod{} in the current iteration. Specifically, the edges newly introduced in the current input candidate graph are outgoing edges which 1) start from nodes newly introduced in $G_k$, and 2) neither appear in $G_k$ nor the remaining $G_c$ updated by \innermethod{} in the last iteration. Based on this observation, we can simply build the candidate graph based on the previous one by only introducing these edges. Due to its simplicity and space limit, please refer to our technical
report~\cite{TR} for the pseudocode. With this update method, the process of constructing the candidate graph from scratch in \innermethod{} can be replaced. 

%Regarding Issue 1, we observe that the remaining candidate graph $G_c^{re}$, at the \emph{end} of \innermethod{} (i.e., Algorithm~\ref{alg:networkaugmentationpractical}) in the \emph{last} iteration of Subnetwork Augementation Sketch (i.e., Algorithm~\ref{alg:initialframework}), is a subgraph of the \emph{initial} candidate graph $G_c^{init}$ of \innermethod{} in the \emph{current} iteration. Specifically, the extra edges of $G_c^{init}$ compared to $G_c^{re}$ are outgoing edges from the nodes that are newly introduced into the \ksubnetwork{} $G^k$ by \innermethod{} in the last iteration. Thus, we propose a method called \method{UpdateCandidateGraph} (Algorithm~\ref{alg:candidateupdate}) to build the candidate graph based on the previous one by only introducing these edges. With this update method, the process of constructing the candidate graph from scratch in \innermethod{} (i.e., Line 1 in Algorithm~\ref{alg:networkaugmentationpractical}) can be replaced.  



%{\color{brown} (Not exist in the submission) Algorithm~\ref{alg:candidateupdate} shows the process of updating the candidate graph where line 2 computes the nodes newly introduced in the last iteration and line 3-7 add outgoing edges from these nodes into the candidate graph. With Algorithm~\ref{alg:candidateupdate}, the process of constructing the candidate graph from scratch in \innermethod{} (i.e., line 1 in Algorithm~\ref{alg:networkaugmentationpractical}) can be removed. }

\smallskip
\noindent \textbf{Observation 3}. Regarding Issue 2, we observe that the influence spread of $s$ will converge after a few iterations (e.g., 6) of the subnetwork augmentation and the \ksubnetwork{} $G_k$ barely includes more nodes from $G$ after convergence (as shown in Figure~\ref{fig:noderatio} in experiments). Considering that we treat all inserted edges as native ones at the end of each iteration, the influence spread of $s$ is actually based on SMPP paths. Therefore, the converged influence also indicates that the SMPPs from $s$ to the rest of nodes barely change, and accordingly the ranking of the nodes based on their subtree sizes in the SMPP-based tree is quite stable.

%Regarding Issue 2, we observe that the influence spread of $s$ will converge after few iterations (e.g., 6) and the \ksubnetwork{} $G_k$ barely includes more nodes from $G$ after convergence (as shown in Figure~\ref{fig:noderatio} in experiments). This also means that \innermethod{} has already identified the nodes important for spreading the influence and hence we can focus on edge insertion among them. Thus, the subtree sizes of nodes in $G_k$ and the node ranking based on the them are rather stable after convergence {\color{blue} since the smpp-based influence barely change, smapps not change thus stable}.
 
As a result, after the convergence, we can leverage the same and converged node ranking for edge insertions in the rest of iterations of the subnetwork augmentation. Furthermore, the candidate graph at the end of the last iteration naturally becomes the initial candidate graph in the current iteration since no more new nodes are considered. With these properties, we propose a method called \method{FillUpRecommendation (FUR)} (Algorithm~\ref{alg:fillup}) which simulates the process of \innermethod{} in the rest of all iterations of the subnetwork augmentation. Specifically, each while loop from Line 6 to 17 corresponds to one iteration where we greedily insert the critical edge for each node in $L$ constructed based on the converged ranking. In each loop, $L'$ is used to store nodes which still have incoming neighbors and thus will be considered in the next iteration, and $I[v]$ is used to efficiently retrieve the critical neighbor by pruning out neighbors which either were considered in previous iterations or cannot be connected to $v$ anymore due to the update of $G_c$ in previous iterations (Lines 14-15). Since each incoming neighbor has been sorted in Line 2, simulating each iteration is very efficient with aforementioned data structures.

\begin{figure}[!t]

\centering
\includegraphics[width=0.4\textwidth]{./figures/FURexample}\hspace{-1em}
%\vspace{-1em}
\caption{An example of a candidate network $G_c$ with $k=2$.} 
\label{fig:FURexample}
\end{figure}

%to avoid candidate graph update and perform fast simulations (i.e., Algorithm~\ref{alg:fillup}) of repeated greedy insertions so as to fill up the recommendations. Specifically, Algorithm~\ref{alg:fillup} works by iteratively processing end nodes based on the converged subtree-size-based node ranking and inserting the critical incoming edge to the current node. Each iteration (i.e., line 5-17 in Algorithm~\ref{alg:fillup}) actually corresponds to the greedy strategy by inserting the critical edge to each node with incoming neighbors based on the ranking.

%\smallskip
%\noindent \textbf{Two stages of \outtermethod{}}. For ease of illustration in our experiments later, we regard the process before convergence as the \emph{expansion stage} (i.e., line 5-9 in Algorithm~\ref{alg:practicalframework}) and the process afterwards as the \emph{filling stage} (i.e., line 10 in Algorithm~\ref{alg:practicalframework}).

\begin{example}\label{example:FUR}
Figure~\ref{fig:FURexample} shows a candidate network $G_c$ with $k=2$. Suppose that the influence spread in $G_k$has converged at iteration $i$ and the converged node ranking is $e$ and $f$. Algorithm~\ref{alg:networkaugmentationpractical} will be executed two more iterations to reach the termination condition (i.e., no edges exist in $G_c$). At iteration $i+1$, edges $(b,e)$, $(b,f)$, $(c,f)$ and $(c,e)$ will be inserted, deleted, inserted and deleted in sequence respectively. The remaining candidate graph becomes the initial candidate graph at iteration $i+2$ where edges $(a,e)$ and $(d,f)$ will be inserted. The method \method{FUR} (Algorithm~\ref{alg:fillup}) is proposed to simulate the iterative process after the convergence and the while loop in \method{FUR} will be executed twice.
\end{example}

\smallskip

\noindent \textbf{Practical Subnetwork Augmentation}. By incorporating the measures for tackling the two issues above, we propose a framework called \method{PracticalSubnetworkAugmentation (\outtermethod{})} (Algorithm~\ref{alg:practicalframework}) where the predefined $\epsilon$ (e.g., $10^{-4}$) controls the convergence point (Line 7) and \method{FUR}, based on the converged subtree-size-based node ranking (Line 10), repeats the process of Lines 5-6 in \outtermethod{} until no edges exist in $G_c$. Note that $L'$ records the new candidate nodes to be incorporated into $G_k$ for graph expansion in the last iteration and is updated by \method{UpdateCandidateGraph} in Line 9. For ease of illustration in our experiments later, we regard the process before convergence as the \emph{expansion stage} (i.e., Lines 5-9) and the process afterwards as the \emph{filling stage} (i.e., Line 10).



%Algorithm~\ref{alg:practicalframework} shows the overall procedure of the practical subnetwork augmentation method (\outtermethod{}) where the predefined $\epsilon$ (e.g., $10^{-4}$) controls the convergence point in line 7 and Algorithm~\ref{alg:fillup} in line 10 simulates the process of line 5-9 in \outtermethod{} in the rest of iterations until no edges can be inserted into $G_k$ based on the converged subtree-size-based node ranking. 

%\sout{Suppose $I$ refers to the number of iteration to converge and $d_m$ refers to the maximum in-degree of nodes in $G$, the total time complexity of Algorithm~\ref{alg:practicalframework} is $O(I(|V|+|E|)\log |V|+|V|d_{m}\log d_{m} )$ which is rather efficient since $I$ is usually small in practice.}

\smallskip
\noindent \textbf{Time Complexity}. Suppose Algorithm~\ref{alg:practicalframework} takes $I$ iterations to converge. Lines 5-9 take $O(I(|V|+|E|)\log |V| )$ time which is acceptable in practice since $I$ is empirically small (e.g., 6). Lines 1-3 in Algorithm~\ref{alg:fillup} take $O(|V|d_{m}\log d_{m} )$ where $d_m$ refers to the maximum in-degree in $G$, and Lines 5-17 take $O(|E|)$ time as each incoming neighbor of each node is visited only once. Thus, the total time complexity of Algorithm~\ref{alg:practicalframework} is $O(I(|V|+|E|)\log |V|+|V|d_{m}\log d_{m} )$.

%Suppose Algorithm~\ref{alg:practicalframework} takes $I$ iterations to converge, line 5-9 takes $O(I(|V|+|E|)\log |V| )$ time which is acceptable in practice since $I$ is empirically small (e.g., 6). Line 1-3 in Algorithm~\ref{alg:fillup} takes $O(|V|d_{m}\log d_{m} )$ where $d_m$ refers to the maximum in-degree in $G$, and line 5-17 takes $O(|E|)$ time as each incoming neighbor of each node is visited only once. Thus, the total time complexity of Algorithm~\ref{alg:practicalframework} is $O(I(|V|+|E|)\log |V|+|V|d_{m}\log d_{m} )$.


==> imcsnvldb2023 copy/tex/multiplebudget.tex <==

\section{PDMFP with multiple campaigns}
In this section, we will discuss our problem in the case there are multiple campaigns implying multiple budgets and each influencer can be assigned to at most one marketing campaign. This problem cater for the scenario where each influencer exclusively collaborate with one brand among all competitors or the influencer only have high alignment with a specific brand. Note that, without the assignment constraint, this problem becomes equivalent to our problem under single budget. Next we will theoretically analyze the hardness of this problem and then outline some directions for solutions. We use $\mathcal{B}$ to denote a set of campaign budgets $\{B_1,B_2,...,B_{|\mathcal{B}|} \}$ and $\scheme{}_{\mathcal{B},\candidates{}} (v,B )$ to denote the hired price of $v$ set by the pricing scheme $\scheme{}_{\mathcal{B},\candidates{}} $ in a campaign with budget $B$. For ease of presentation, we assume that each campaign has an unique budget.

\begin{definition}[\short{} with multiple campaigns]
Given a set $\mathcal{B}$ of campaign budgets, a set $\candidates{}$ of candidates with their profit expectation ( $\sum_{v \in \candidates{}} p^*_v= \sum_{B \in \mathcal{B}}B $) and influence, we aim to propose an optimal \constraint{} pricing scheme $\scheme{}^*_{\mathcal{B},\candidates{}}$ such that the overall profit divergence is minimized, e.g.,
\begin{equation}
\begin{aligned}
&\scheme{}^*_{\mathcal{B},I}=\argmin_{\scheme{}_{\mathcal{B},\candidates{}} \in \mathcal{S}  }  \sum_{v\in I}  | \sum_{B \in \mathcal{B}} \scheme{}_{\mathcal{B},I} (v,B)- p^*_{v} |\\
\text{subject to (1)} \; & \forall B \in \mathcal{B}, \sum_{v\in \candidates{}}\scheme{}_{\mathcal{B},\candidates{}} (v,B) \leq B, \\
\text{(2)} \; & \forall v \in \candidates{}, \text{if } \sum_{B \in \mathcal{B}} \scheme{}_{\mathcal{B},\candidates{}} (v,B)>0, \exists B' \in \mathcal{B},\\ &\scheme{}_{\mathcal{B},\candidates{}} (v,B')=\sum_{B \in \mathcal{B}} \scheme{}_{\mathcal{B},\candidates{}} (v,B),
\end{aligned} 
\end{equation}

\noindent where the second constraint ensures that any influencer will be assigned to at most one campaign.
\end{definition}


\begin{definition}[Simple case with binary choices]\label{mbbc}
 Given a set $\mathcal{B}$ of campaign budgets, a set $\candidates{}$ of candidates with their profit expectation and influence where each influencer $v$ is assigned with a hired price $p_v=\delta(v)$ and a profit expectation $p^*_v$ ( $\sum_{v \in \candidates{}} p^*_v=\sum_{k=1}^{|\mathcal{B}|} B_k $), we aim to hire some influencers from $\candidates{}$ to join different campaigns under their specific budgets such that the divergence score is minimized:
 
 \begin{equation}\label{mbsimple}
 \begin{aligned}
  \text{minimize} \: & \sum_{B \in \mathcal{B}} B - \sum_{v \in \candidates{}} \sum_{B \in \mathcal{B}} x_{v, B} *f(v,p_{v})  ,\\
  \text{where}  \; & \text{(1)} \:  f(v,p_{v}) = \left \{ \begin{aligned}
       & p_{v},  \;\;  \text{if } p^*_{v} > p_{v}\\
       &2p^*_{v} -p_{v}, \;\; \text{if } p^*_{v}\leq p_{v}\\   
     \end{aligned}\right. \\
        & \text{(2)} \: x_{v,B} =0 \; \text{or} \; 1, \\
        & \text{(3)} \: \sum_{v \in \candidates{}}  x_{v,B} \cdot p_{v} \leq B.   
    \end{aligned} 
 \end{equation}
 
 \end{definition}

Next, we will show that our problem under multiple campaigns is NP-hard and NP-hard to approximate via reduction from 3-partition problem. 

\begin{definition}[3-partition problem~\cite{garey1979computers}]
Given a set $\mathcal{A}$ of elements $\{a_1,a_2,...,a_{3m}\}$ and a positive integer $B'$, and a positive size $s(a_i)$ for each $a_i \in \mathcal{A}$ where $s(a_i)$ satisfies $B'/4<s(a_i)<B'/2$ and $\sum_{i=1}^{3m} s(a_i)=mB'$, can $\mathcal{A}$ be partitioned into $m$ disjoint sets $A_1,A_2,...,A_m$ so that for $1\leq j \leq m$, $\sum_{a\in A_j} s(a)=B'$?
\end{definition}


\begin{theorem}
The \short{} with multiple budgets is NP-hard and NP-hard to approximate within any constant factor.
\end{theorem}

\begin{proof}
We prove hardness for the simple case with binary price choices (i.e., Definition~\ref{mbbc}) by using reduction from 3-Partition.

Given any instance of 3-Partition problem, we construct the corresponding instance on our problem as follows. First, we construct the influencer set $\candidates{}=\{v_1,v_2,...,v_{3m}\}$ where the profit expectation and the hired price of the $i$-th candidate are both equal to $s(a_j)$ where $1\leq j \leq 3m$. Next, we construct $m$ budgets $B_1,B_2,...,B_m$ all of which are equal to $B'$. The reduction is achieved in polynomial time since the sizes of influencer set and budgets are bounded by $m$. We next show that if our problem can be solved
in polynomial time, so can 3-PARTITION, implying hardness. Specifically, we claim that any instance of 3-Partition problem is a YES-instance if and only if the divergence score (i.e., Formula~\ref{mbsimple}) in the corresponding instance of our problem is 0.

\noindent ($\Longrightarrow$): Suppose $A_1,A_2,...,A_m$ are disjoint 3-element subsets of $\mathcal{A}$ that each sum to $B'$. For elements in the same subset $A_j \:(1 \leq j\leq m)$, we assign the corresponding influencers into the same campaign with budget $B_j$. This assignment clearly leads to 0 divergence score.

\noindent ($\Longleftarrow$): If the divergence score is 0 in the instance of our problem, all influencers have been hired to join marketing campaigns. Otherwise, the divergence score cannot be 0 based on Formula~\ref{mbsimple}. It also means that the budgets of all campaigns have been fully used, otherwise the divergence score cannot be 0.
Since the $f()$ score of each influencer $v$ is equal to her profit expectation $p^*_v$ which satisfies that $B'/4<s(a_i)<B'/2$ and the budget of each campaign is equal to $B'$, each campaign involves exactly three influencers. For influencers in campaign with budget $B_j \:(1 \leq j\leq m)$, we assign the corresponding elements into the same subset $A_j$. This assignment naturally leads to a YES-instance of the 3-Partition problem. 

We just proved that our problem is NP-hard. To
see hardness of approximation, suppose $\mathcal{Q}$ is an algorithm that approximates
our problem within a factor of $\alpha$. That is,
the divergence score achieved by algorithm $\mathcal{Q}$ on any instance of our problem
is not greater than $\alpha \cdot OPT$, where $OPT$ is the optimal (least) divergence score. Using the same reduction as above, we can see that the optimal divergence score on the reduced instance above is 0. On this instance,
the regret achieved by algorithm $\mathcal{Q}$ is $ \leq \alpha \cdot OPT=0$, which means that algorithm $\mathcal{Q}$ can solve our problem optimally in polynomial time. It is shown above to be impossible unless P = NP.

\end{proof}


\noindent \emph{Solutions on \short{} with multiple campaigns}. The main challenge on our problem with multiple campaigns mainly lies in the assignments of influencers to different campaigns, which is very different from our main problem with a single campaign which focus on pricing influencers. To solve \short{} with multiple campaigns, we can use our proposed methods to price influencers first followed by adopting existing algorithms~\cite{khuri1994zero,chekuri2005polynomial,martello1980solution} on the multiple knapsacks problem for assignment which is a well-studied classical problem. 


\iffalse
\subsection{NP-hardness of problem 2}
 We first formulate two constrained multiple knapsack problems MKPV and MKPVC and prove their NP-hardness. Next, we prove the NP-hardness of problem 1 via reduction flow: MKP to MKPV, MKPV to MKPVC, MKPVC to our problem.

\smallskip
\noindent \textbf{Multiple Knapsack problem (MKP)}. Given a sequence of $i$ items each of which is assigned with non-negative weight $w_h$ and a value $z_h$ $(1 \leq h\leq i)$, and $j$ bags each of which is associated with capacity $\bar{B}_k \; (1 \leq k\leq j)$, we aim to select $j$ disjoint subsets of items so that the total profit of selected items is maximized and each subset can be assigned to a different knapsack whose capacity is no less than the total weight of items in this subset. Formally,

\begin{equation}
\text{maximize} \sum_{h=1}^i \sum_{k=1}^j p_{hk}*z_h
\end{equation}

\noindent subject to the following five constraints:
\begin{enumerate}
\item $\forall h \;(1 \leq h \leq i) \: \text{and} \: k \; (1 \leq h \leq j), p_{hk}=0$ or 1.
\item $\forall h \;(1 \leq h \leq i),  \sum_{k=1}^{j} p_{hk} \leq 1 $.

\item $\forall k \; (1 \leq k\leq j), \sum_{h=1}^{i} p_{hk}\cdot w_h \leq B_k  $.

\end{enumerate}

 \smallskip


\noindent \textbf{Multiple Knapsack problem with value constraints (MKPV)}. Given a sequence of $i$ items each of which is assigned with non-negative weight $w_h$ and a value $z_h$ $(1 \leq h\leq i)$ \emph{smaller than its weight} $(z_h \leq w_h)$, and $j$ bags each of which is associated with capacity $\bar{B}_k \; (1 \leq k\leq j)$, we aim to select $j$ disjoint subsets of items so that the total profit of selected items is maximized and each subset can be assigned to a different knapsack whose capacity is no less than the total weight of items in this subset.

\smallskip

\noindent \textbf{Multiple Knapsack problem with value and budget constraints (MKPVC)}. Given a sequence of $i$ items each of which is assigned with non-negative weight $w_h$ and a value $z_h$ $(1 \leq h\leq i)$ \emph{smaller than its weight} $(z_h \leq w_h)$, and $j$ bags each of which is associated with capacity $\bar{B}_k \; (1 \leq k\leq j)$ such that $\sum_{k=1}^j \bar{B_k} = (\sum_{h=1}^i w_h+z_h)/2$, we aim to select $j$ disjoint subsets of items so that the total profit of selected items is maximized and each subset can be assigned to a different knapsack whose capacity is no less than the total weight of items in this subset.

\smallskip


\begin{lemma}
MKPV is NP-hard.
\end{lemma}
\begin{proof}
To reduce MKP to MKPV, we can multiple all item weights and budgets by a suitable parameter to satisfy the value constraint without effecting the solution, just like we did in Lemma 1.
\end{proof}

\begin{lemma}
MKPVC is NP-hard.
\end{lemma}
\begin{proof}
To reduce MKPV to MKPVC, we can satisfy the budget constraint by introducing a `super useless' or `super useful' item just like we did in Lemma 2. There is one difference. In Lemma 2, we update the capacity when we introducing a `super useful' item. Here, in this reduction from MPKV to MPKVC, we introduce an extra bag with capacity equal to the weight of the `super useful' item.
\end{proof}

\begin{theorem}
Problem 2 is NP-hard to be solved.
\end{theorem}

\begin{proof}
We reduce MKPVC to the special case of problem 1 by mapping $q_{v_h}=(w_h+z_h)/2$, $B_k= \bar{B}_k$ $(1 \leq k \leq j)$, and $c_{v_h}^*=w_h$. Based on this mapping and value and capacity constraint in MKPVC, we have $q_{v_h} \leq c_{v_h}^*$ and $\sum_{h=1}^i q_h= \sum_{k=1}^j B_k$. Based on Equation 7 and 8, the objective is:
$$\text{maximize} \sum_{h=1}^i \sum_{k=1}^j p_{hk} (2q_{v_h}-c_{v_h}^* ) = \sum_{h=1}^i \sum_{k=1}^j p_{hk} \cdot z_h,$$

\noindent which is the same as the objective of MKPVC. The solution of the special case of problem 2 must be the solution of MKPVC and vice versa. Since the reduction is in polynomial time, problem 2 is NP-hard.

\end{proof}


\begin{theorem}
The special case of problem 2 is equivalent to MKP problem.
\end{theorem}

\begin{proof}
We omit the proof since it is rather straightfoward based on similar reduction in Theorem 5.
\end{proof}
\subsection{Non polynomial approximation of problem 2}
First we introduce 3-partition problem which is strongly NP-complete and show that our problem can be reduced from 3-partition problem. Next, we will show the non-approximation of our problem by considering the optimal value of Equation 11 is 0.

\noindent \textbf{3-partition problem~\cite{garey1979computers}}. Given a set $A'$ of elements $A'=\{a_1,a_2,...,a_{3m}\}$ and a positive integer $B'$, and a positive size $s(a_i)$ for each $a_i \in A'$ where $s(a_i)$ satisfies $B'/4<s(a_i)<B'/2$ and $\sum_{i=1}^{3m} s(a_i)=mB'$, can $A'$ be partitioned into $m$ disjoint sets $A'_1,A'_2,...,A'_m$ so that for $1\leq j \leq m$, $\sum_{a\in A'_j} s(a)=B'$?

\begin{lemma}
The special case of problem 2 can be reduced from 3-partition problem.
\end{lemma}
\begin{proof}
Since MKP problem can be reduced from 3-partition problem~\cite{geng1986complexity} and the special case of problem 2 is equivalent to MKP problem, the special case of problem 2 can be reduced from 3-partition problem.
\end{proof}

\begin{theorem}
The special case of problem 2 is NP-hard to approximate in polynomial time. 
\end{theorem}

\begin{proof}
We can reduced a 3-partition instance to the special case of problem 2, by mapping $A=A'$, $m$ budgets $B_1=B_2=...=B_m=B'$, and $c_{v_h}^*=q_{v_h}=s(a_h)$ $(1\leq h \leq 3m)$. 
%Based on the definition and NP-completeness of 3-partition problem, it can be NP-hard to find the optimal allocation strategy even when the optimal value of Equation 11 is 0. 

Suppose we have an approximate algorithm $\mathcal{A}$ that approximates Equation 11 within a factor of $\alpha$. Using the same reduction above, we can see the optimal value on this instance of Equation 11 can be 0. On this instance, the value achieved by algorithm $\mathcal{A}$  is $\leq \alpha \cdot 0=0$, which means that algorithm $\mathcal{A}$ can solve the special case of problem 2 optimally in polynomial time. This is not possible unless $P=NP$.

\end{proof}
\fi

==> imcsnvldb2023 copy/tex/preliminary.tex <==
\section{Problem Formulation}\label{sec:preliminary}
%In this section, we will introduce some definitions and the problem formulation to facilitate the illustration in the rest of the paper. 
In this paper, we consider both directed and undirected social network where the latter can be transformed into the directed one. In an undirected network, each edge represents a friendship between two users. Since information diffusion is directed, each friendship corresponds to two diffusion directions. Thus, we represent the undirected social network as the directed one $G=(V,E)$ where $V$ ($E$) is the node (edge) set, and each directed edge from $u$ to $v$ is denoted as $(u,v)$. We use $N^G_{in}(u)$ and $N^G_{out}(u)$ to denote the set of incoming and outgoing neighbors of $u$, respectively. 


\iffalse
\begin{table}[!t]\center
\caption{Frequently used notations.}


	\begin{adjustbox}{width=0.48\textwidth}
		\begin{tabular}{  |c| c| } 
			\hline
			\textbf{Notation} &\textbf{Description} \\ 
			\hline
			$G_k$ & The \ksubnetwork{}.\\
			$G_c$ & The candidate graph which consists of edge candidates for insertion.\\
			$p_{(u,v)}$& The influence probability of edge $(u,v)$.\\ 
	
			$RMPP(u,v)$ & The restricted maximum probability path from $u$ to $v$.\\
		
			$\rppr{(u,v)}$ & The probability of RMPP from $u$ to $v$.\\
		
			$SMPP(u,v)$ & The strict maximum probability path from $u$ to $v$.\\
		
			$\sppr{(u,v)}$ & The probability of SMPP from $u$ to $v$.\\
	
			$u^*_v$ & The critical incoming neighbor of $v$.\\
	
	        $r(u)$ & The relevant seed of node $u$. \\

			\hline
		\end{tabular}
	\end{adjustbox}
	
	\label{notation}
\vspace{-0.75em}
\end{table}
\fi

\smallskip
\noindent \textbf{The diffusion model}. We focus on a classic and widely-adopted
information diffusion model -- the {\textit{Independent Cascade}} (IC)
model~\cite{Kempe03}.
It originates from the marketing
literature~\cite{goldenberg2001using} and independently assigns each
edge $(u,v)$ with an influence probability $p_{u,v}
\rightarrow [0,1]$. Given a seed node $s$ being active at time step 0 and the influence probabilities, the diffusion unfolds in discrete steps.
Each active node $u$ in time 
step $t \geq 1$ will have a single chance to activate each
outgoing neighbor $v$, that is inactive in step $t-1$, with a probability of $p_{u,v}$.
If an outgoing neighbor $v$ is activated in step $t$, it
will become active in step $t+1$ and then will have a single chance
to activate each of its inactive outgoing neighbors in the next time step.
%Otherwise, the neighbor will stay inactive.
The diffusion instance terminates when no more nodes can
be activated.
The \emph{influence spread} $\delta_G(s)$ in a graph $G$ is the expected number of activated nodes with $s$ as the seed node. Note that our proposed methods are specifically designed for the IC model. The extension on other models (e.g., the Linear Threshold model~\cite{Kempe03}) is out of the scope of this work and will be explored in future work.

\smallskip
In this paper, we aim to select at most $k$ outgoing edges for each online user such that the influence spread of seeds via these selected edges is maximized. These directed edges naturally form a diffusion sub-network defined as below. 
  
\begin{definition}[K-subnetwork]
Given a directed network $G=(V,E)$ and an integer $k$, a k-subnetwork $G_k$ is a subgraph of $G$ where there are at most $k$ outgoing neighbors for each $v\in G_k$. Formally, $G_k=(V_k,E_k)$ where $V_k\subseteq V$, $E_k \subseteq E$ and $\forall v \in V_k, |N^{G_k}_{out}(v)|\leq k$.

\end{definition}  
 
% \begin{example}
For example, in Figure~\ref{introexample}, the network that consists of solid edges only is a 2-subnetwork.
 %\end{example}
%
Notably, based on industry practice, we make three considerations when formulating our problem (i.e., Definition~\ref{defn:problem}): 1) The value of $k$ is the same for all users and is decided by the event operator. However, our solutions can easily work with the scenario where the value of $k$ depends on specific users. 
 %(1) The information receiver is only allowed to share the message with a limited number of friends since (i) the sender has different levels of intimacy with online friends and may not be willing to share the message with arbitrary friends without needs or interests. (here we assume all users are targeted for receiving information for simplicity),
  %and (ii) recommending too many friends to receive the message would harm user experience since it may lead to 
  %too much engagement of users who repeatedly receive the same message from different sources and users' negative attitudes towards the platform~\cite{health};
 2) Seed users are independent since KOLs (i.e., key opinion leaders) may have unpredictable and different information to spread over a long period, and recommendations based on this consideration help maintain a long-term usage of the recommendation system. 
 3) The friend recommendation list for a user is built by considering all seed users instead of being customized for individuals since (i) it is intractable to know, among all seed users sharing the same content, who will activate online users for further information propagation in real-world scenarios, and (ii) fixing the recommendations help increase the interaction rate between users with a laser focus on facilitating information diffusion.
 
 
\begin{definition}[Influence maximization in closed social networks (\short{})]\label{defn:problem}
Given a directed social network $G=(V,E)$, an integer $k$, a set $S$ of independent seed users, we aim to find the optimal diffusion \ksubnetwork{} $G^*_k$ such that the aggregated influence of seed users in $S$ is maximized under $G^*_k$:

$$  G^*_k = \argmax_{G_k \in \mathbb{S}}  \sum_{s \in S} \delta_{G_k} (s) $$ 

\noindent where $\mathbb{S}$ refers to the whole space of all possible k-subnetworks of $G$.
\end{definition}

If $s \notin V_k$,  the influence of $s$ in $G_k$ is 0. When the context is clear, we omit the subscript of $\delta_{G_k}(\cdot)$, and we use the terms `node' and `user', as well as the terms `edge' and `link' interchangeably. %The problem above is formulated based on industry practice and details are in Section~\ref{appendix:consideration} of the supplementary file.


\begin{figure}[!t]

\centering
\includegraphics[width=0.3\textwidth]{./figures/tree}\hspace{-1em}
%\vspace{-1em}
\caption{An example of a graph constructed based on a set cover instance.} 
\label{fig:tree}
\end{figure}



\smallskip
 \noindent \textbf{Hardness analysis of the \short{}}. We will show that the \short{} problem is NP-hard via a reduction from the set cover problem defined as below.


\begin{definition}[Set Cover]
Given a set $U$ of elements, a collection $C$ of subsets $A_1,A_2,...,A_{|C|}$ of $U$ where $\cup_{1\leq i\leq |C|} A_i = U$, we aim to choose the smallest number of sets from $C$ such that their union is $U$.
\end{definition}



\begin{theorem}\label{proof:nphard}
The \short{} problem is NP-hard.
\end{theorem}

\begin{proof}
To show that \short{} is NP-hard, we will perform a reduction from the NP-complete decision problem of set cover, which checks whether we can find $k$ sets from $C$ whose union is $U$, to the special case of \short{} where there is only one seed user $s$.

Given the collection $C$ of a set cover instance, we construct a deterministic graph with a tree structure where the weight of each edge is 1 as below. First, we find the set $A_{max}$ with the greatest size from $C$ and create a tree with elements in $A_{max}$ as the bottom nodes (at the bottom level). In the second to last level, we introduce the set $V'$ of $\lceil |A_{max}|/k  \rceil$ virtual nodes. We next create directed edges from each of the virtual nodes to at most $k$ arbitrary nodes in $A_{max}$ which have not been connected by virtual nodes in $V'$. Afterwards, we create the third to last level based on the second to last level by adopting the similar rules. We repeat this step until the root node is constructed. We also create trees for the rest of the sets in $C$ similarly. One difference is that, when we create the tree for a set $A$, we need to make sure that the number of virtual nodes in each level is consistent with the corresponding level of the tree constructed based on $A_{max}$. It means that some virtual nodes may not have outgoing neighbors. After we create trees for all sets in $C$, we introduce directed edges from $s$ to all root nodes. 


Figure~\ref{fig:tree} shows an example where a graph is constructed from the set cover instance where $k=2$ and $C=\{ \{a,b,c,d,e\},\{d,e,f\}, \allowbreak \{f,g,h\} \}$. Dashed nodes refer to virtual nodes. Virtual nodes with the same number come from the tree constructed based on the same set from $C$. Since $A_{max}=\{a,b,c,d,e\}$, the number of virtual nodes in the second to last level of all trees are $\lceil |A_{max}|/k  \rceil =3$. 

%In this instance, the challenge of solving the \short{} problem lies in choosing two out of three outgoing edges from $s$, and the optimal solution is to pick edges $(s,1)$ and $(s,3)$.

Since the time cost for creating such a tree is at most $O(|A_{max}| \allowbreak \log_k|A_{max}|)$, the total reduction process is polynomial in the total size of the sets in the collection. To solve the \short{} problem in the constructed graph, we only need to focus on selecting $k$ outgoing edges for the root node $s$ since the out-degree of the rest of the nodes in the graph is at most $k$ and edges not incident on $s$ can all be chosen. Considering that the trees constructed from each set in $C$ have the same number of virtual nodes, the quality of the outgoing edge selection for $s$ only depends on bottom nodes being reached. Thus, selecting $k$ outgoing edges for $s$ corresponds to selecting $k$ sets from $C$. Suppose the number of virtual nodes in each tree is $x$. If the optimal influence spread is $k\times x +1+|U|$ (including $s$) which is also the maximum possible influence, we have a `Yes' answer to the set cover instance. Otherwise, the answer is `No'. Therefore, if we can find the optimal solution for the \short{} instance in polynomial time, the set cover problem can be solved in polynomial time which is not possible unless P=NP. Thus, the \short{} problem is NP-hard.
\end{proof}









%\begin{proof}
%Please refer to Appendix~\ref{appendix:hardness} for details.
%\end{proof}



%\noindent \textbf{Remark}. We formulate the \short{} problem by considering industry practice and the property of closed social networks in real life. {\color{red}  Please refer to Section~\ref{appendix:consideration} in supplementary material for details.} \bao{either remove it or combine it with the previous parargraph talking about "same k or not". It is very sudden to have this remark.}







==> imcsnvldb2023 copy/tex/relatedwork.tex <==
\section{Related work}\label{sec:relatedwork}
%We will introduce related work on  influence maximization via node selection and edge insertion.
In this section, we will first describe the difference between closed and open social networks. Afterwards, we will describe the related work on influence maximization in \emph{open} social networks, which can be broadly divided into two categories, influence maximization via node selection and influence maximization via edge insertion, respectively. Then, we will discuss the differences between them and our problem in \emph{closed} social networks.

\smallskip
\noindent \textbf{Open vs. Closed Social Networks}. The two words `open' and `closed' are used to describe the underlying sharing model rather than the topology of the social network. Furthermore, the sharing system applied to the network is decided based on the specific application behind. For example, if Figure~\ref{introexample} describes a subgraph of the Twitter social network, we have an open sharing model by default and a user's post will be available to all online users. On the other hand, if Figure~\ref{introexample} describes a subgraph of the Wechat social network, the closed sharing model will be applied in most cases (as in Example 1) where users will make their messages or posts visible to a limited number of selected friends. For ease of presentation and following the naming convention in this domain~\cite{naming1,naming2}, we directly use `open' and `closed' social networks to refer to the networks with the `open' and `closed' sharing model respectively.


\smallskip
\noindent \textbf{Influence Maximization via node selection}.
This problem refers to the classical influence maximization problem that aims to choose a limited number of seed nodes with the greatest influence spread. Kempe
et al.~\cite{Kempe03} prove the NP-hardness of this problem and propose a Monte Carlo simulation based greedy algorithm which iteratively chooses the node with the greatest marginal gain to the influence. Due to the importance of this problem, many subsequent studies%~\cite{leskovec2007cost,goyal2011celf++,cheng2013staticgreedy,ohsaka2014fast,borgs2014maximizing,nemhauser1978analysis,tang2014influence,jung2012irie} 
~\cite{huang2019finding,huang2021capturing,leskovec2007cost,goyal2011celf++,cheng2013staticgreedy,ohsaka2014fast,borgs2014maximizing,nemhauser1978analysis,tang2014influence,goyal2011simpath,jung2012irie,galhotra2016holistic,chen2010scalable,chen2009efficient,chen2010scalable2,wang2017real,bian2020efficient,huang2020efficient,bevilacqua2021fractional,cautis2019adaptive,zhang2020geodemographic,aslay2018influence,cai2020target,huang2019community,liu2019influence,li2019tiptop,he2019tifim,sun2018multi,wu2018two,minutoli2019fast,banerjee2019combim,han2018efficient,tang2015influence} 
have been proposed to further improve the efficiency and/or effectiveness.  They mainly differ in how the influence spread is defined or estimated. To name a few, \citeauthor{leskovec2007cost}~\cite{leskovec2007cost} adopt the Monte-Carlo simluation to measure the influence spread and speed up the process in~\cite{Kempe03} with an early termination technique based on the submodular property of the influence function. \citeauthor{ohsaka2014fast}~\cite{ohsaka2014fast} measure the influence and marginal gain based on a limited number of subgraphs generated by the flipping-coin technique~\cite{Kempe03}, which further improves the efficiency. \citeauthor{borgs2014maximizing}~\cite{borgs2014maximizing} leverage reverse reachable sets to estimate influence and inspires more recent advanced solutions~\cite{tang2014influence,tang2015influence}.





\smallskip
\noindent \textbf{Influence maximization via edge insertion}.
The work falling in this category aims to insert a limited number of edges into the network so as to maximize influence spread of specific seeds. \citeauthor{d2019recommending}~\cite{d2019recommending} study how to maximize the influence of the seeds under the IC model by adding a limited number of edges incident to these seeds. \citeauthor{coro2021link}~\cite{coro2021link} extend the results of ~\cite{d2019recommending} to the Linear Threshold (LT) model~\cite{granovetter1978threshold}. Specifically, they prove that the objective function under the LT model is submodular and leverage this property to propose an approximate algorithm. 
%The problem studied by these two works is much simpler than ours since (1) they limit that the edges being added must be incident on the seeds which derives good theoretical properties to solve this problem and (2) there is no constraints on the number of inserted edges incident on each node ($k$ in our problem). 
\citeauthor{khalil2014scalable}~\cite{khalil2014scalable} study how to add a limited number of edges to maximize the influence of given seeds under the LT model. 
%Their method cannot handle IC model and does not consider the constraint of edge incidence on any node.
\citeauthor{chaoji2012recommendations}~\cite{chaoji2012recommendations} study how to add edges to maximize the influence spread of seeds under the constraint that at most $k$ inserted edges are incident on any node.
% which is the most similar work to our problem among all study in this category. However, their proposed method cannot directly solve our equivalent problem via edge insertion since their method estimate pairwise influence via constrained paths which can only contain at most one edges being inserted. In our problem setting via edge inserting, the graph is initially empty and will only contain inserted edges after graph update. Furthermore, their method involving costly belief propagation which cannot scale to real-world social networks. 
\citeauthor{yang2019marginal}~\cite{yang2019marginal} and \citeauthor{yang2020boosting}~\cite{yang2020boosting} study how to add a limited number of edges from a candidate set to maximize the seeds' influence under the IC model. \citeauthor{yang2019marginal}~\cite{yang2019marginal} derive a lower and upper bound influence function respectively to approximate the non-submodular influence under the IC model, and they use a sandwich strategy to produce approximate solutions. \citeauthor{yang2020boosting}~\cite{yang2020boosting} derive tighter bounds than \citeauthor{yang2019marginal}~\cite{yang2019marginal} and produce more effective results.

\smallskip 

\emph{Differences}.~The aforementioned studies are drastically different from ours. The main reason is on the problem setting and assumption. 
The studies of the first category focus on selecting \emph{seeds} based on the open social networks where the influence from the seeds is allowed to propagate via \emph{any} edge in the network. On the other hand, we consider the \emph{closed} social networks, and focus on selecting limited \emph{edges} from the original network such that the influence of \emph{specific seeds} via these \emph{selected edges} is maximized. 



%
The studies of the second category focus on inserting a limited number of \emph{new} edges into the \emph{existing} network and assume an \emph{open-sharing} model such that the influence of the seeds will spread via all edges including the inserted ones. 
%
In contrast, we focus on inserting a limited number of \emph{existing} edges from the original network into an initially empty network and consider a \emph{closed-sharing} model such that the influence of seeds will spread \emph{only} via inserted edges. As a consequence, existing work's decision making of edge insertion is based on the current graph structure and cannot be trivially extended to handle our problem, because the network which requires edge insertion in our problem is initially empty. 
%
Additionally, due to different assumptions of the sharing model, the space of candidate edges for insertion that is considered by existing work is significantly smaller than that of our problem. As a result, most existing methods will suffer from serious scalability issue even if they could be extended to handle our case. In particular, the infeasibility of extending existing work can be caused by reasons including but not limited to: (1) Most of these studies do not consider the edge insertion constraint where the number of inserted edges sharing the same source node cannot be greater than $k$. (2) The methods in~\cite{d2019recommending,coro2021link} are designed based on the assumption that the source nodes of all edge candidates must be seeds, which is not the case in our problem. (3) The method in~\cite{khalil2014scalable} is specifically designed for the LT model which has drastically different properties from the IC model we are considering. (4) The method in~\cite{chaoji2012recommendations} cannot help the seed nodes to influence the nodes that are 2-hop away in the initially empty network, because the influence path between any pair of nodes is not allowed to contain more than one inserted edge. (5) The methods in~\cite{yang2019marginal,yang2020boosting} hold a strong assumption that the network is acyclic, which is often not true in real-world scenarios.





%incurs expensive computational costs such that network sizes considered in their experiments are quite small (e.g., up to $|V|=27k$, and $|E|=352k$ in~\cite{yang2020boosting}).

 %\citeauthor{yu2020maximizing}~\cite{yu2020maximizing} leverage the idea of constrained paths in~\cite{chaoji2012recommendations} to derive a submodular influence function, and then use the standard greedy to find the approximate solution. All of these three works do not consider the constraint that at most $k$ added edges can be incident on any node. Furthermore, they consider the number of edges to be added and the candidate edge set size to be quite small. However, in our problem from the perspective of edge insertion, the number of edges to be added is up to $k|V|$ and the candidate edge set consists of all edges in the original network. Furthermore, they can only work for acyclic graphs!


 
\iffalse
\noindent \textbf{ influence maximization via edge deletion}. \citeauthor{kimura2008minimizing}~\cite{kimura2008minimizing} study removing a limited number of edges such that the average influence of all the nodes in the graph is minimized. \citeauthor{khalil2014scalable}~\cite{khalil2014scalable} study removing a limited number of edges to minimize the influence of given seeds.
\citeauthor{wang2020efficient}~\cite{wang2020efficient} study removing a set of edges to minimize the influence of given seeds to a predefined set of users. \citeauthor{medya2019influence}~\cite{medya2019influence} study a similar problem but under the credit distribution model~\cite{goyal2011data} where the influence is much more easier to be computed compared with IC and LT model. \citeauthor{nandi2016methods}~\cite{nandi2016methods} investigate the effectiveness of link removal as an intervention to minimize the spread of infections in a network. They develop four network interdiction models with different objectives and formulate these models as mixed integer linear programs. \citeauthor{pham2018maximizing}~\cite{pham2018maximizing} aim to find a
set of nodes whose removal from a social network maximizes the influence reduction from the source of misinformation within time and budget constraints.

In summary, all work in this category is different from our equivalent problem via edge deletion in two aspects: (1) the objective is different. They all aim to minimize the influence of the seeds in the residue graph whereas we aim to maximize the influence. (2) constraints of the residue graph. Existing work does not have constraints on the structure of the residue graph whereas we require that each node in the residue graph can have at most $k$ out neighbors.
\fi

==> imcsnvldb2023 copy/tex/response.tex <==
\twocolumn
\begin{center}
	\noindent\textbf{Response to Reviewer Comments}
\end{center}

We would like to express our sincere gratitude to the meta-reviewer and the three reviewers who take considerable time to review and comment our paper and acknowledge the technical depth and quality of content of our work. Their constructive comments, suggestions, and advises are all much appreciated. After addressing all the comments, the paper presentation is greatly improved with more descriptions and details (e.g., discussion between closed and open social networks, direction applications of the problem, method introduction, and deployment).


\subsection*{Revision Summary}

Below is a summary of the major revisions that we have made in
the paper. All major revisions have been highlighted using {\color{blue} blue color} in this manuscript.

\vspace{1em}

\noindent\textbf{Major Revision 1 : Discuss the applications of our problem.}

As suggested by Reviewer \#3, we have revised the introduction by adding direct applications of our problem. Please refer to response to Reviewer \#3 - W2, D1 for details.

\vspace{1em}

\noindent\textbf{Major Revision 2 : Discuss the difference between open and closed social networks.}

As suggested by Reviewer \#4, we have added the detailed discussion about the difference in Section~\ref{sec:relatedwork}. Please refer to response to Reviewer \#4 - W2 for details.

\vspace{1em}

\noindent\textbf{Major Revision 3 : Improve the presentation of Section~\ref{sec:methodsingle}.}

As suggested by Reviewer \#3 and \#4, we have revised the presentation of Section~\ref{sec:methodsingle} with multiple revisions (e.g., adding more details into the proofs and intuitions and key observations for method design). Please refer to response to Reviewer \#3 - D3 and Reviewer \#4 - W1, D1, D2, D3 for details.


\vspace{1em}

\noindent\textbf{Major Revision 4 : Provide more details of deployment.}

As suggested by Reviewer \#2, we have added more details of our deployment in Section~\ref{sec:deploy}. Please refer to response to Reviewer \#2 - W1 for details.

\vspace{1em}

\noindent\textbf{Major Revision 5 : Compare efficiency of different methods.}

As suggested by Reviewer \#3, we have included Table~\ref{table:orgvsbsttime} to compare the running time of different methods. Please refer to response to Reviewer \#3 - W3, D7 for details.


\vspace{1em}
\noindent\textbf{Major Revision 6 : Change the acronyms of algorithm names.}

We remove the space among the words in all algorithms' names and thus correspondingly update the acronyms. Specifically, \method{EI} is updated to \innermethod{} for Algorithm~\ref{alg:networkaugmentationpractical} and \method{SNA} is updated to \outtermethod{} for Algorithm~\ref{alg:practicalframework}.

\vspace{1em}

\noindent \textbf{Remark}. Considering that we have added many details in multiple sections and the experiment in Section 6.1 is not primary, we have moved this part into the technical report~\cite{TR} due to space limit. Thus, the section numbers mentioned afterwards refer to the ones in the revised version unless we explicitly mention \emph{`in the original submission'} when locating the section.

\section*{Response to Meta Reviewer}

\vspace{1em}

\noindent\textbf{Meta Reviews.}
\noindent\textit{The reviewers raised some questions or mentioned some weaknesses about this work. They would recommend "revision" for the authors to address the issues. The authors are suggested to look at their reviews (weaknesses and detailed comments) and make a revision. The revision items are R2.W1, R3.D1-D7 and R4. All weaknesses and detailed points.}

\vspace{.5em}

\noindent\textbf{Response:} Thanks for your valuable suggestion. We have revised this paper according to the comments
from three reviews. All major revisions have been presented above.
Next, we will respond to all the comments from individual reviewers.

\vspace{.5em}


\section*{Response to Reviewer \#2}

\vspace{1em}

\noindent\textbf{W1.}
\noindent\textit{More details of deployment on MOBAX could be reported to show the practicality of proposed method.}

\vspace{.5em}

\noindent\textbf{Response:} Thanks for your valuable suggestion. We have added more descriptions on possible behaviors and roles of users, edge weight settings, the underlying diffusion model, how our method generates the diffusion network and why we generate this way, and why we choose Click-Through-Rate (CTR) as the evaluation metric and a discussion on other possible evaluation metrics. Please refer to Section~\ref{sec:deploy} for more details and below is a brief explanation of possible user behaviors and our choice of evaluation metric.

\smallskip
 \noindent \textbf{User behaviors}. In this activity, we do not specifically designate seeds and every user could be a potential and spontaneous seed. Specifically, users who log in the game will see this activity and may perform three possible behaviors: (1) proactively start interactions as a seed, (2) start interactions as a message receiver (i.e., a non-seed) and (3) ignore this activity.

\smallskip
\noindent \textbf{Evaluation metrics}. The number of users who interact with recommended friends directly indicates the quality of the underlying recommendation system and can effectively reflect the potential size of users who are impacted by others to perform interactions. Thus, to evaluate the performance, we adopt the Click-through Rate (CTR) which is a very popular evaluation metric for recommendation systems in industry. Despite the effectiveness of CTR, there still exist some other evaluation metrics (e.g., the actual influence spread of seeds via knowing the propagation paths and who are the seeds) worthy of explorations. However, due to the privacy restriction of this activity, we have no access to the detailed information in user logs to compute the performance under other potential metrics. In future, we would like to see how our proposed method will perform in other activities under various metrics.

\vspace{.5em}


\section*{Response to Reviewer \#3}

\vspace{1em}

\noindent\textbf{W1.}
\noindent\textit{No theoretical guarantee is provided for the result quality.}

\vspace{.5em}

\noindent\textbf{Response:} Thanks for your valuable concern. Our response below will emphasize that it is very challenging to have very efficient methods with theoretical guarantees on our problem; also, we aim for deployment into real-world applications and thus highly efficient and effective heuristic methods like our proposed \outtermethod{}  is desirable.

Studies on influence maximization in open social networks via edge insertions~\cite{d2019recommending,coro2021link,khalil2014scalable,chaoji2012recommendations,yang2019marginal,yang2020boosting} sacrifice efficiency and generality for theoretical guarantees, which is not acceptable in reality. We argue that our problem should be not easier than the aforementioned problem and ensuring the theoretical guarantees is not the first priority when deployment is considered. 

First of all, the size of candidate edges for insertion considered in this paper (i.e., all edges in the original network) is significantly larger than that in existing studies (e.g., only possible edges incident on seed nodes only) on influence maximization via edge insertions under the open sharing model. To achieve theoretical guarantees and meanwhile improve the efficiency, most (if not all) of them have to hold unrealistic assumptions (e.g., the network much be acyclic~\cite{yang2019marginal,yang2020boosting} and candidates must be incident on seeds~\cite{d2019recommending,coro2021link}) as we elaborate in Section~\ref{sec:relatedwork}. Furthermore, even with these assumptions, existing studies can still suffer from serious scalability issues (e.g., the state-of-the-art~\cite{chaoji2012recommendations}, on the problem in Section~6.1 in the original submission, is five-orders-of-magnitude slower than our methods), and some of them~\cite{yang2019marginal,yang2020boosting} did not report the running time in experiments even on very small-scale datasets (e.g., the greatest dataset in~\cite{yang2020boosting} has only 27,770 nodes and 352,807 edges). In other words, considering the very limited scalability of existing studies which consider a very small number of edge candidates and hold unrealistic assumptions, it is not reckless to claim that proposing highly efficient methods with theoretical guarantees on our problem, with a significantly much larger size of edge candidates and no strong assumptions, is very challenging. 

Second, we aim for a deployment of our proposed methods into real-world applications to benefit the society and thus high efficiency is an essential requirement for our methods. 
Third, the effectiveness of our methods is also verified in three different problems (i.e., 
maximizing the influence in \emph{open} social networks via edge insertions, 
our proposed problem \short{}, and
maximizing users' Click-trough Rate in an activity of an online Tencent application). Notably, our method can be very competitive with the state-of-the-art~\cite{chaoji2012recommendations} with theoretical guarantees in solving the problem of maximizing the influence in open social networks (see Section 6.1 in the original submission).

To summarize, we believe the methods we have proposed, although heuristic, are non-trivial technical contributions, and they are both efficient and effective in solving a real problem. 

\vspace{.5em}


\noindent \textbf{W2.}
\noindent \textit{Applications should be well argued.}

\noindent\textbf{D1.}
\noindent\textit{The problem application is not convincing. In the introduction, it is not quite clear why ``users are likely to share information with only a limited number of friend''. The paper discusses motivation and gives an example for the research problem. Some real cases/scenarios are expected to show the direct application of the problem.}

\vspace{.5em}

\noindent\textbf{Response:} Thanks for the suggestion. Besides our deployment into the real application in Section~\ref{sec:deploy}, we add two other real scenarios into the introduction. In scenario 1, users in WeChat tend to share their life moments or private matters only with their close friends and families, rather than colleagues with pure business relationships~\cite{block,block2}.
%(2) users who do not like validating existence may share information with whom they think the information is important to, without posting this information to all their friends since this message can be irrelevant to and overwhelm many users; 
In scenario 2, users who spend on online Tencent gaming events may obtain limited virtual coupons for sharing and they need to carefully choose friends to receive the coupons since people who use the coupons eventually can increase the discounts of future purchase of the coupon sender~\cite{gaming}. 

 %Note that sharing in the closed social networks does not have conflicts with that in open social networks. They complement each other and are applied in different scenarios. 
\vspace{.5em}


\noindent\textbf{D2.}
\noindent\textit{The paper should give running examples for Algorithm~\ref{alg:networkaugmentationpractical} and Algorithm~\ref{alg:fillup}.
}

\vspace{.5em}
\noindent\textbf{Response:} Thanks for the suggestions. We add Example~\ref{example:EI} and Example~\ref{example:FUR} as the running examples for Algorithm~\ref{alg:networkaugmentationpractical} in Section~\ref{sec:edgeinsertion} and Algorithm~\ref{alg:fillup} in Section~\ref{sec:augmentation} respectively.
\vspace{.5em}

\noindent\textbf{D4.}
\noindent\textit{It's better to formally define the critical edge.}

\vspace{.5em}
\noindent\textbf{Response:} Thanks for the valuable suggestion. We add Definition~\ref{defn:criticalneighborandedge} to formally define the critical edge and neighbor in Section~\ref{sec:edgeinsertion}. 
\vspace{.5em}

\noindent\textbf{D5.}
\noindent\textit{In Theorem~\ref{theorem:idealcase}, does ``lead to the optimal solution'' mean the method can produce the same result as Algorithm~\ref{alg:networkaugmentation}?}

\vspace{.5em}
\noindent\textbf{Response:} Yes, to explain this, we add more descriptions in the proof of Theorem~\ref{theorem:idealcase} and more explanation about the theorem right after the proof. Specifically, in the special case (i.e., $\forall x \in V_c, |Cr(x)| \leq min(k,N^{G}_{out}(x))- N^{G_k}_{out}(x) $) specified in Theorem~\ref{theorem:idealcase}, Algorithm~\ref{alg:networkaugmentation} will produce the optimal solution and directly inserting all critical edges will produce the same solution as that of Algorithm~\ref{alg:networkaugmentation}.
\vspace{.5em}


\noindent\textbf{D3.}
\noindent\textit{The presentation  of Section~\ref{sec:methodsingle} can be improved.}

\vspace{.5em}

\noindent\textbf{Response:} Thanks for the valuable suggestions. To improve the presentation of Section~\ref{sec:methodsingle}, we make the following major revisions:


\begin{itemize}[leftmargin=*]


\item Add a road map of Section~\ref{sec:methodsingle} right before Section~\ref{sec:edgeinsertion}.

\item Revise the description in the proof of Lemma~\ref{theorem:marginalgain}.

\item Formally define the critical neighbor and edge in Definition~\ref{defn:criticalneighborandedge}.

\item Revise the description in the proof of Theorem~\ref{theorem:critical}.

\item Revise the observation and motivation of the practical edge insertion method in the beginning of Section~\ref{sec:praticaledgeinsertion}.

\item Revise the description in the proof of Theorem~\ref{theorem:idealcase} and add more explanation of this theorem right after the proof.

\item Enrich the three key observations with more details (Observation 1, Observation 2 and Observation 3).

\item Add two running examples for Algorithm~\ref{alg:networkaugmentationpractical} and Algorithm~\ref{alg:fillup} respectively.

\item Revise some notations in Algorithm~\ref{alg:practicalframework} and Algorithm~\ref{alg:fillup}.

\item Remove the space among words in the names of all Algorithms.

\item Add an acronym for the name of Algorithm~\ref{alg:fillup}, update the acronyms for Algorithm~\ref{alg:networkaugmentationpractical} and Algorithm~\ref{alg:practicalframework}.
\end{itemize}

\vspace{.5em}


\noindent\textbf{D6.}
\noindent\textit{In terms of resulting quality, the advantage of \outtermethod{} is not obvious according to Figure~\ref{fig:diffk}.}

\vspace{.5em}

\noindent\textbf{Response:} Thanks for the comment. The advantage of \outtermethod{} is actually quite significant and we would like to emphasize that, mentioned in Section~\ref{sec:exp-closed} where we described the baselines we used, the performance of boosted baselines over their original counterparts mainly benefit from our proposed \emph{expansion} stage of \outtermethod{} (i.e., Lines 5-9 in Algorithm~\ref{alg:practicalframework}). In other words, proposing these boosted baselines is also our contribution. Next, we will explain why the advantage is significant but not visually distinguishable in Figure~\ref{fig:diffk}. 



As we mentioned in the last paragraph of `Exp3 - Effectiveness comparison with different k', the performance difference in Figure~\ref{fig:diffk} is not easy to distinguish visually due to the log scale of y axis. Furthermore, the difference between influence spread under different $k$ is much larger than that under different $|S|$ as shown in Figure~\ref{fig:diffs}, which increases the range of y axis and further makes it hard to clearly compare the performance. However, Figure~\ref{fig:diffk} is used to show the general trend of influence spread under different $k$ and the comparison among all methods has been conducted already at a finer granularity (i.e., $k=20$ and $k=30$ in Figure~\ref{fig:diffs} and Table~\ref{table:orgvsbst}). For instance, Table~\ref{table:orgvsbst} clearly reports the results of $k=30$ in Figure~\ref{fig:diffk}, and we observe that \outtermethod{} can outperform the second best performer by at least 23\%-39\% on different datasets respectively. Even though such performance gap is hard to be visualized in Figure~\ref{fig:diffk}, it is actually very significant especially compared with studies on the traditional influence maximization problem where 4\% of improvement is already significant~\cite{arora2017debunking}.


\vspace{.5em}


\noindent \textbf{W3.}
\noindent \textit{The efficiency improvement is not clear.}

\noindent\textbf{D7.}
\noindent\textit{Most techniques in the paper are designed to improve efficiency. However, only one experiment (Figure 8) is conducted to evaluate the efficiency. The paper should compare the running time of the proposed method with several baselines.}

\vspace{.5em}

\noindent\textbf{Response:} Thanks for the suggestions. Efficiency needs improvement when existing methods suffer from serious scalability issue (e.g., the state-of-the-art~\cite{chaoji2012recommendations}, in Section~6.1 of the original submission, is five-orders-of-magnitude slower than our methods). Since the recommendation system is for long-term usage, effectiveness is the first priority when methods can produce solutions within reasonable time. Thus, we did not compare the running time of different methods on our own problem because our method \outtermethod{} significantly outperforms the rest in terms of effectiveness and is highly efficient. 
%Thus, we think that it may not be so meaningful to compare their efficiency when they are far less than competitive with \outtermethod{} in terms of effectiveness. 
In the revision, we have taken the reviewer's suggestion to compare the running of our method and boosted baselines under all parameter settings. They show similar results that \outtermethod{} is very competitive with other boosted baselines in terms of running time, because all methods involve the \emph{expansion} stage of \outtermethod{} (i.e., Lines 5-9 in Algorithm~\ref{alg:practicalframework}) which dominates the total computational cost. Due to space limit, we only report the running time with $k=30$ and $|S|=50$ in Table~\ref{table:orgvsbsttime} in the main paper and please refer to the technical report~\cite{TR} for more experiment results. 

\vspace{.5em}


\section*{Response to Reviewer \#4}

\vspace{1em}
\noindent \textbf{W1.}
\noindent \textit{The presentation can be improved. There are some grammatical flaws.}

\noindent \textbf{D1.}
\noindent \textit{In algorithm 4, the font of comment is a little strange.}

\noindent \textbf{D2.}
\noindent \textit{In algorithm 4, there are subfunctions and variable names with too wide letter spacing.}

\noindent \textbf{D3.}
\noindent \textit{Section 6, "In this section, we will conduct experiments on three problems to demonstrate the robustness and effectiveness our methods", missing preposition before "our methods".}

\vspace{.5em}

\noindent\textbf{Response:} Thanks for the valuable suggestions. We have corrected them in the corresponding places and the changes are highlighted.

\vspace{.5em}


\vspace{1em}

\noindent\textbf{W2.}
\noindent\textit{In Section~\ref{sec:relatedwork}, the difference between open social network and closed social network can be described in more details. It might be better to use some examples.}

\vspace{.5em}

\noindent\textbf{Response:} Thanks for the valuable suggestion. We revise the first paragraph and add a paragraph right after that to discuss the difference in Section~\ref{sec:relatedwork}. In a nutshell, the two words `open' and `closed' are used to describe \textit{the underlying sharing model rather than the topology of the social network}. Furthermore, the sharing model applied to the network is decided based on the specific application behind. For example, if Figure~\ref{introexample} describes a subgraph of the Twitter social network, we have an open sharing model by default and a user's post will be available to all online users. On the other hand, if Figure~\ref{introexample} describes a subgraph of the Wechat social network, the closed sharing model will be applied in most cases (as in Example 1) where users will make their messages or posts visible to a limited number of selected friends. For ease of presentation and following the naming convention in this domain~\cite{naming1,naming2}, we directly use `open' and `closed' social networks to refer to the networks with the `open' and `closed' sharing models respectively.  

\vspace{.5em}


\noindent\textbf{W3.}
\noindent\textit{The features of closed social networks could be further utilized in algorithms.}

\vspace{.5em}

\noindent\textbf{Response:} Thanks for the suggestions. As per our response to W2, to our best knowledge, the only difference between open and closed social networks is the underlying sharing model. We believe that we have fully utilized the feature of the closed sharing model, which can be reflected by the two facts (presented in Section~\ref{sec:relatedwork}) that our problem formulation is drastically different from the classical influence maximization problems via node or edge selections, and existing methods cannot be trivially extended to solve our problem.

Specifically, the studies on the influence maximization problem via \emph{node selection} focus on selecting \emph{seeds} based on the open social networks where the influence from the seeds is allowed to propagate via \emph{any} edge in the network. On the other hand, in our problem, the underlying social networks are\emph{closed}, and we focus on selecting limited \emph{edges} from the original network such that the influence of \emph{specific seeds} via these \emph{selected edges} is maximized. 

The studies on the influence maximization problem via \emph{edge selection} focus on inserting a limited number of \emph{new} edges into the \emph{existing} network and assume an \emph{open-sharing} model such that the influence of the seeds will spread via all edges including the inserted ones. 
In contrast, we focus on inserting a limited number of \emph{existing} edges from the original network into an initially empty network and consider a \emph{closed-sharing} model such that the influence of seeds will spread \emph{only} via inserted edges. As a consequence, existing work's decision making of edge insertion is based on the current graph structure and cannot be trivially extended to handle our problem, because the network which requires edge insertion in our problem is initially empty. 
Additionally, due to different assumptions of the sharing model, the space of candidate edges for insertion that is considered by existing work is significantly smaller than that of our problem. As a result, most existing methods will suffer from serious scalability issue even if they could be extended via non-trivial ways to handle our problem. However, such extensions are quite infeasible due to many reasons including but not limited to the ones we elaborated at the end of Section~\ref{sec:relatedwork}.

In summary, we have tried our best to utilize the feature of closed social network to propose highly efficient and effective algorithms to solve a novel research problem which cannot be solved by the state-of-the-art on related but quite different problems.





%Thanks for the suggestions. As we respond to the previous comment, the features of closed social networks mainly lie in the underlying closed sharing model rather than the network topology. In this paper, we utilize the feature of the closed sharing model to formulate an influence maximization problem. Extensive experiments demonstrate the efficient and effectiveness of our methods, and we would like to utilize this feature to explore more advanced solutions with theoretical guarantees in future. 



==> imcsnvldb2023 copy/tex/shortenedexp.tex <==
\section{Experiment}\label{sec:experiment}
{In this section, we will conduct experiments on three problems to demonstrate the robustness and effectiveness of our methods:  }

\begin{itemize}[leftmargin = *]


\item The first is our proposed problem, \short{},  where the extensions of the methods in the first problem are compared (Section~\ref{sec:exp-closed}). Note that the core difference between these two problems has been illustrated and please refer to Section~\ref{sec:relatedwork} for details.

\item The second problem is maximizing users' Click-trough Rate in an activity of an online Tencent application, where we deploy our method and evaluate how it helps improve user retentions and interactions (Section~\ref{sec:deploy}). 

\item The third problem is maximizing the influence in \emph{open} social networks via edge insertions, where existing baselines including the state-of-the-art~\cite{chaoji2012recommendations} are compared. The results show that, compared with~\cite{chaoji2012recommendations}, our method \outtermethod{} achieves very competitive results with up to five-orders-of-magnitude speedup. Please refer to the technical report~\cite{TR} for details.

\end{itemize}


\smallskip
\noindent\textbf{Datasets}. Table~\ref{table:dataset} presents all the real-world undirected social networks used. In particular, MOBA and MOBAX correspond to two friendship networks of Tencent multiplayer online battle arena games, RPG corresponds to a friendship network of a role-playing game, and the other datasets are available in~\cite{konect}. Note that each edge is represented twice since the influence propagation is directed. The first four datasets and the last dataset will be used for the second and the third problem respectively.

%To obtain experimental results in a reasonable time under different problem settings, the first four datasets, the next four datasets and the last dataset will be used for the first, the second and the third problem,  respectively.


\smallskip
\noindent \textbf{Environments}. We conduct all experiments on a Linux server with Intel Xeon E5
(2.60 GHz) CPUs and 512 GB RAM. All algorithms are implemented in
Python and our code is available at~\cite{TR}. 

\begin{table}[]
\caption{Dataset Statistics}\label{table:dataset}
\small
\begin{tabular}{cccc}
\hline
\textbf{Dataset} & \textbf{|V|} & \textbf{|E|} & \textbf{Avg. Degree} \\ \hline
Catster &149,700 & 10,898,550 & 73\\
MOBA & 503,029 & 9,372,022 & 19 \\
RPG  & 2,331,047 & 88,227,562 & 38\\
Orkut & 3,072,441 & 234,369,798 & 76\\
MOBAX & 36,201,207&3,281,207,036&90\\ \hline
\end{tabular}
\end{table}


\iffalse
\begin{table}[]
\caption{Dataset Statistics}\label{table:dataset}
\begin{tabular}{cccc}
\hline
\textbf{Dataset} & \textbf{|V|} & \textbf{|E|} & \textbf{Avg. Degree} \\ \hline
EU-Core & 1,005 & 51,142 & 51 \\
Hamster & 2,426 & 33,261 & 14 \\
CiaoDVD & 4,658 & 80,266 & 17 \\
Brightkite & 58,228 & 428,156 & 7 \\ 
%Livemocha & 104,103 & 4,386,166 & 42\\
Catster &149,700 & 10,898,550 & 73\\
MOBA & 503,029 & 9,372,022 & 19 \\
RPG  & 2,331,047 & 88,227,562 & 38\\
Orkut & 3,072,441 & 234,369,798 & 76\\
MOBAX & 36,201,207&3,281,207,036&90\\ \hline
\end{tabular}
\end{table}
\fi

\iffalse
\subsection{Experiment with the Open Sharing Model}\label{sec:exp-open}
In this section, we study maximizing the influence in open social networks. Here, we insert a set $X'$ of edges from the candidate set $X$ into the original social network such that (1) at most $k$ edges in $X'$ share the same source node and (2) the influence sum of the seed nodes is maximized. The purpose of this section is twofold: 
\begin{itemize}[leftmargin = *]
\item Our proposed method \outtermethod{} is able to effectively maximize the influence of multiple seed nodes, as compared to the state-of-the-art called continuous greedy \method{CG}~\cite{chaoji2012recommendations} on this problem.
 %Specifically, \method{CG}~\cite{chaoji2012recommendations} studies a slightly different problem where at most $k$ edges in $X'$ share the same source \emph{or} end nodes. 
\item Our proposed method \outtermethod{} is robust to different variations of influence maximization via edge recommendations.
\end{itemize}

\smallskip
\noindent \textbf{Baselines}. Baselines are listed below where \method{Degree} and \method{FoF} (i.e., Friend of Friend) were also compared by \method{CG}~\cite{chen2009efficient}. For ease of description, we assume out-degrees of nodes in the original network to be greater than $k$.

\begin{itemize}[leftmargin = *]
\item \method{Degree} based method where, for candidates sharing the same source node, top $k$ edges with the highest degrees of end nodes are selected.

\item \method{FoF} based method where,  for candidates sharing the same source node, top $k$ edges whose source and end nodes share the highest number of common friends are selected.

\item \method{Random} based method where $k$ edges are randomly selected from candidates sharing the same source node. Its performance is reported as the average over five independent runs.

\item \method{CG}~\cite{chaoji2012recommendations} where edges are inserted based on a continuous greedy method followed by randomized rounding. We set all parameters as recommended by the original work.
\end{itemize}


\smallskip
\noindent \textbf{Edge Weight Settings}. We follow the previous work~\cite{chaoji2012recommendations} to adopt the constant model where each edge in the original network and candidate edge for insertion is assigned with a constant influence probability and we set it as 0.1. Note that the constant model and the influence probability setting are also commonly used by existing studies in the classical influence maximization problem~\cite{arora2017debunking,goyal2011celf++,Kempe03}.
 
\smallskip
\noindent \textbf{Parameter Settings}. Considering that \method{CG} is not scalable to a large number of seed nodes and edge candidates, we conduct experiments on small-scale datasets. Specifically, we randomly select five nodes from the top 1\% nodes with the highest degrees in the original network as the seed nodes. Afterwards, we generate 50 outgoing edges from each node within two hops away from the seed nodes as candidates, and these candidates are generated randomly by following the setup of~\cite{chaoji2012recommendations} where an edge candidate can be added between any pair of nodes without group information. We set $k$ as 20, the error ratio $\epsilon$ of \outtermethod{} as $10^{-4}$, and follow the common standard~\cite{arora2017debunking} to estimate the influence of any solution under the IC model via 10,000 Monte Carlo simulations.



\smallskip
\noindent \textbf{Experimental Results}. Table~\ref{table:openinf} compares the influence spread achieved by different methods under the RMPP model  and the IC model, respectively. It is obvious that there is a positive correlation between influence under the RMPP model and the one under the IC model. That is, greater influence under the former one also indicates larger influence under the latter. Hence, the idea of optimizing the RMPP-based influence spread to approximate the IC-based influence is effective. \outtermethod{} significantly outperforms \method{Degree}, \method{FoF} and \method{Random}, and achieves very competitive results with \method{CG}. Furthermore, \outtermethod{} achieves up to five-orders-of-magnitude speedup over \method{CG} as shown in Table~\ref{table:opentime}. These results demonstrate the efficiency, effectiveness and robustness of \outtermethod{}, in terms of maximizing the  influence of multiple seed nodes via edge recommendations/insertions. 



\begin{table}[]
\caption{Comparison of influence achieved by different methods under the RMPP model (RP) and the IC model.}\label{table:openinf}
\begin{tabular}{ccccccccc}
\hline
\multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c}{\textbf{EU-Core}} & \multicolumn{2}{c}{\textbf{Hamster}} & \multicolumn{2}{c}{\textbf{CiaoDVD}} & \multicolumn{2}{c}{\textbf{Brightkite}} \\ \cline{2-9} 
 & \textbf{RP} & \textbf{IC} & \textbf{RP} & \textbf{IC} & \textbf{RP} & \textbf{IC} & \textbf{RP} & \textbf{IC} \\ \hline
Degree & 65 & 2801 & 65 & 2513 & 92 & 5891 & 80 & 8912 \\
FoF & 68 & 3012 & 67 & 2789 & 95 & 6013 & 75 & 8134 \\
Random & 70 & 3189 & 64 & 2445 & 100 & 6231 & 73 & 7986 \\
SNA & 76 & 3684 & 72 & 3142 & 109 & 6618 & 88 & 12034 \\
CG & 78 & 3769 & 74 & 3221 & 109 & 6680 & 89 & 12851 \\ \hline
\end{tabular}
\end{table}



\begin{table}[]
\caption{Running time comparison between CG and SNAF.}\label{table:opentime}
\begin{tabular}{ccccc}
\hline
\textbf{Method} & \textbf{EU-Core} & \textbf{Hamster} & \textbf{CiaoDVD} & \textbf{Brightkite} \\ \hline
SNA & 5.8E-1 & 1.7E-1 & 1.5E0 & 1.7E1 \\
CG & 3.56E4 & 3.0E4 & 5.5E4 & 4.6E4 \\ \hline
\end{tabular}
\end{table}






\fi




\begin{table}[]
\caption{Effectiveness comparison with $k=30$ and $|S|=50$.}\label{table:orgvsbst}
\small
\begin{tabular}{cccccccc}
\hline
\multirow{2}{*}{\textbf{Dataset}} & \multicolumn{2}{c}{\textbf{Degree}} & \multicolumn{2}{c}{\textbf{FoF}} & \multicolumn{2}{c}{\textbf{Random}} & \multirow{2}{*}{\textbf{\outtermethod{}}} \\ \cline{2-7}
 & \textbf{Ori} & \textbf{Bst} & \textbf{Ori} & \textbf{Bst} & \textbf{Ori} & \textbf{Bst} &  \\ \hline
%Livemocha & 6.1E2 & 7.8E5 &7.9E2& 8.0E5&2.9E3&8.3E5&\textbf{9.8E5}\\
Catster & 3.1E2 & 4.2E5 & 3.8E2 & 4.8E5 & 3.6E3 & 6.3E5 & \textbf{8.6E5} \\
MOBA & 5.0E6 & 7.4E6 & 6.5E6 & 7.7E6 & 7.0E6 & 8.0E6 & \textbf{9.8E6} \\
RPG & 1.1E6 &2.1E7 &   2.4E6 &2.2E7 &1.9E7 & 2.4E7 & \textbf{3.2E7} \\
Orkut & 7.0E2 & 5.4E7 & 6.8E2 & 5.6E7 & 9.6E5 & 5.9E7 & \textbf{8.2E7} \\ \hline
\end{tabular}

\end{table}

\iffalse
\begin{table}[]
\caption{Running time comparison with $k=30$ and $|S|=50$ where the numbers in brackets under \outtermethod{} refers to the time cost in the graph expansion stage which is also involved in boosted baselines. Note that the number of common friends is pre-computed in \method{Bst-FoF}.}\label{table:orgvsbsttime}
\small
\begin{tabular}{cccccccc}
\hline
\textbf{Dataset} & \textbf{Bst-Degree} & \textbf{Bst-FoF} & \textbf{Bst-Random} & \textbf{\outtermethod{}} \\ \hline
Catster & 1.1E2 & 1.1E2 & 1.1E2 & 1.3E2 (1.0E2) \\
MOBA & 1.2E2 & 1.1E2 & 1.1E2 & 1.7E2 (1.0E2) \\
RPG & 8.8E2 & 8.1E2 & 8.1E2 & 1.1E3 (7.6E2)\\
Orkut & 4.5E3 & 4.2E3 & 4.2E3 & 5.7E3 (3.9E3)\\ \hline
\end{tabular}

\end{table}
\fi

\begin{table}[]
\caption{Running time (s) with $k=30$ and $|S|=50$ where the numbers in brackets under \outtermethod{} refers to the time cost in the graph expansion stage. Note that the number of common friends is pre-computed in \method{Bst-FoF}.}\label{table:orgvsbsttime}
\small
\begin{tabular}{cccccccc}
\hline
\textbf{Dataset} & \textbf{Bst-Degree} & \textbf{Bst-FoF} & \textbf{Bst-Random} & \textbf{\outtermethod{}} \\ \hline
Catster & 1.1E2 & 1.0E2 & 9.8E1 & 1.2E2 (9.1E1)\\
MOBA &1.4E2& 1.3E2 & 1.2E2 & 1.8E2 (1.3E2)\\
RPG & 9.6E2& 9.1E2 & 8.8E2 & 9.8E2 (7.3E2)\\
Orkut & 4.4E3& 4.2E3& 4.1E3 & 5.1E3 (3.6E3)\\ \hline
\end{tabular}

\end{table}





\subsection{Experiment on the \short{} problem}\label{sec:exp-closed}
 We conduct seven experiments to demonstrate that: (1) the extension of existing baselines on open social networks cannot well address our problem but their performance can be significantly boosted with the help of our method \outtermethod{} (Exp1); (2) \outtermethod{} consistently and significantly outperforms all the boosted baselines with different $|S|$ and $k$ (Exp2-3); (3) how $k$ and $|S|$ impact the convergence of \outtermethod{} (Exp4); (4) \outtermethod{} is highly scalable to handle large-scale datasets (Exp5); (5) the influence convergence is also a good indicator of the node size convergence in the diffusion network (Exp6); (6) the influence of seeds in the diffusion network, produced by \outtermethod{} with a small edge size, is very competitive with the influnce of the seeds in the original network (Exp7).



\begin{figure}[t]
\includegraphics[width=0.4\textwidth]{./drawing2/legend1}
\vspace{-0.25cm}

\centering
\subfloat[Catster]{
\includegraphics[width=0.124\textwidth]{./drawing2/difft_Catster.pdf}\hspace{-1em}
}
\hspace{0.1mm}
\subfloat[MOBA]{
\includegraphics[width=0.124\textwidth]{./drawing2/difft_LOL.pdf}\hspace{-1em}
} 
\hspace{0.1mm}
\subfloat[RPG]{
\includegraphics[width=0.124\textwidth]{./drawing2/difft_RPG.pdf}\hspace{-1em}
}
\hspace{0.1mm}
\subfloat[Orkut]{
\includegraphics[width=0.124\textwidth]{./drawing2/difft_Orkut.pdf}\hspace{-1em}
}

\vspace{-0.7em}
\caption{Performance Comparison with different $|S|$.}\label{fig:diffs}
%\vspace{-2.5em}
\end{figure}

\begin{figure}[t]
\includegraphics[width=0.4\textwidth]{./drawing2/legend1}
\vspace{-0.25cm}

\centering

\subfloat[Catster]{
\includegraphics[width=0.124\textwidth]{./drawing2/diffk_Catster.pdf}\hspace{-1em}
}
\hspace{0.1mm}
\subfloat[MOBA]{
\includegraphics[width=0.124\textwidth]{./drawing2/diffk_LOL.pdf}\hspace{-1em}
} 
\hspace{0.1mm}
\subfloat[RPG]{
\includegraphics[width=0.124\textwidth]{./drawing2/diffk_RPG.pdf}\hspace{-1em}
}
\hspace{0.1mm}
\subfloat[Orkut]{
\includegraphics[width=0.124\textwidth]{./drawing2/diffk_Orkut.pdf}\hspace{-1em}
}

\vspace{-0.7em}
\caption{Performance Comparison with different $k$.}\label{fig:diffk}
%\vspace{-1.5em}

\end{figure}



\iffalse
\begin{table}[]
\caption{The percentage of edges recommended by the expansion stage of \outtermethod{} over the total edge size of the diffusion network produced by boosted baselines with $k=30$ and $|S|$. Note that the total edge size is the same across different boosted baselines since they are built upon the same input diffusion network.}\label{table:edgeparticapation}
\begin{tabular}{cccc}
\hline
\textbf{Livemocha}& \textbf{Catster} & \textbf{MOBA} & \textbf{Orkut} \\ \hline
					27\%		&		19\%				&			17\%&21\% \\ \hline
\end{tabular}
\end{table}
\fi


\smallskip
\noindent \textbf{Baselines}. We compare three baselines (listed below) on open social networks and their boosted versions. Thus, in total, there are six baselines. For ease of description, we assume out-degrees of nodes in the original network to be greater than $k$.

\begin{itemize}[leftmargin = *]
\item \method{Degree} based method where, for candidates sharing the same source node, top $k$ edges with the highest degrees of end nodes are selected.

\item \method{FoF} based method where,  for candidates sharing the same source node, top $k$ edges whose source and end nodes share the highest number of common friends are selected.

\item \method{Random} based method where $k$ edges are randomly selected from candidates sharing the same source node. Its performance is reported as the average over five independent runs.

\end{itemize}

Since each baseline has two versions, original and boosted, we use the prefixes `Ori' and `Bst' to distinguish them. The boosted versions are built upon the diffusion network generated by the \emph{expansion} stage of \outtermethod{} (i.e., Lines 5-9 in Algorithm~\ref{alg:practicalframework}) and work similar to the original ones. The only difference is that, in the boosted version, some important edges have been inserted by \outtermethod{} and these baselines only `fill up' recommendations for those nodes in the generated diffusion network. Hence, if we assume that the out-degrees of nodes in the original network are greater than $k$ and our method has already inserted $h <k$ outgoing edges from $u$, boosted versions just need to select $k-h$ outgoing edges for $u$. 

%For the reason why \method{CG}~\cite{chaoji2012recommendations} cannot be extended, please refer to Section~\ref{sec:relatedwork} and its scalability issue in Section~\ref{sec:exp-open} for details.




\iffalse
\noindent \textbf{Baselines}. Six baselines are listed below. 
%Notably,  \method{Ori-Degree} and \method{Ori-FoF} were also compared by the state-of-the-art~\cite{chaoji2012recommendations} in open social networks. \bao{can remove the previous sentence.} 
For ease of description, we assume that the out-degrees of nodes in the original network are greater than $k$, and emphasize that all edges in the original network are candidates for insertion into the diffusion network which initially contains seed nodes only.

\begin{itemize}[leftmargin=*]
\item \method{Ori-Degree}: for candidates sharing the same source node, top $k$ edges whose end nodes have the highest degrees are selected.

\item \method{Ori-FoF}: for candidates sharing the same source node, top $k$ edges whose source and end nodes share the highest number of common friends are selected.

\item \method{Ori-Random}: $k$ edges are randomly selected from candidates sharing the same source node. Its performance is reported as the average performance over five independent runs.

\item \method{Bst-Degree}, \method{Bst-FoF} and \method{Bst-Random} are the boosted extension of the previous three methods, respectively. The boosted versions are built upon the diffusion network generated by the \emph{expansion} stage of \outtermethod{} (i.e., lines 5-9 in Algorithm~\ref{alg:practicalframework}) and work similarly to the original ones. The only difference is that, in the boosted version, some important edges have already been recommended/inserted by \outtermethod{} and these baselines just `fill up' recommendations for nodes in the generated diffusion network. Hence, if our method has already inserted $h<k$ outgoing edges from $u$, these boosted versions just need to select at $k-h$ outgoing edges for $u$. Since each baseline has two versions, original and boosted, we use the prefixes `Ori' and `Bst' to distinguish them.
\end{itemize}

%The method in~\cite{chaoji2012recommendations} is not considered, because in the input diffusion network which only contains seed nodes, it fails to help seeds influence the nodes that are more than one hop away. Moreover, there is no non-trivial extension of \method{CG} that is scalable to large-scale networks and can notably outperform our proposed method, as evidenced by experiments on a variation of our problem in open social networks~\cite{TR}.
\fi


\smallskip
\noindent \textbf{Edge Weight Settings}. Considering that the influence probability of edges are different in practice, we adopt the commonly used trivalency model~\cite{chen2010scalable} for Catster and Orkut without edge attributes. It randomly assigns a weight for each edge, from $\{10^{-1},10^{-2},10^{-3}\}$. 

For MOBA and RPG, we assign edge weights based on the intimacy of friendship. In MOBA and RPG, each pair of friends has different levels of intimacy which describes the number of interactions (e.g., the number of games they play together, the number of gifts sent from one to another). Since the pair-wise intimacy in both MOBA and RPG is represented as integers, here we transform it into an influence probability within [0,1] for deployment in the IC model. According to the Susceptible-Infected-Recovered (SIR) model~\cite{anderson1992infectious} and heterogeneous mean-filed theory~\cite{newman2002spread,cohen2011resilience,castellano2010thresholds,xie2021detecting}, the lowest influence probability should not be smaller than a constant $\lambda$ times $\beta_c= \sum_{v \in V} |N_{out}(v)| / (\sum_{v \in V} |N_{out}(v)|^2- \sum_{v \in V} |N_{out}(v)|)$, where $\beta_c$ is the epidemic threshold in the SIR model and calculated as 0.024 and 0.001 on MOBA and RPG, respectively. If $\lambda \beta_c$ is too small, the influence of the seeds will be quite limited. If $\lambda \beta_c$ is too large, the influence spread can cover a large percentage of nodes, irrespective of where it originated, and the methods' performance cannot be well compared. By following existing studies~\cite{shu2015numerical,lu2016h}, we
determine $\lambda$ by simulation on real networks. Specifically, we determine $\lambda_1$ and $\lambda_2$ and control the edge weights within the range $[\lambda_1\beta_c, \lambda_2\beta_c]$. Each influence probability $p_{(u,v)}= ((u,v)_{I} - \min_{e\in E} e_{I}) / (\max_{e\in E} e_{I} -\min_{e\in E} e_{I}  ) (\lambda_2 -\lambda_1)\beta_c +\lambda_1\beta_c$ where $(u,v)_{I}$ denotes the intimacy between $u$ and $v$. Note that we have checked several settings of $\lambda_1$ and $\lambda_2$ and these different settings will not affect the conclusion (i.e., performance ranking of methods). To test these methods' robustness to the influence probability distributions, in both MOBA and RPG, we set the range $[\lambda_1\beta_c, \lambda_2\beta_c]$ as $[0.007,0.01]$ which has a dramatically different distribution from the trivalency model deployed for other datasets.





\smallskip
\noindent \textbf{Parameter Settings}. We randomly select $|S|$ (50 by default) nodes from the top 1\% nodes with the highest degrees in the original network as the seed nodes, set $k=20$ and the error ratio $\epsilon=10^{-4}$ by default. We evaluate solution quality based on the IC-based influence spread via 10,000 Monte Carlo simulations. 


\smallskip
\noindent \textit{\textbf{Exp1 - Case study on the two versions of baselines}}. Table~\ref{table:orgvsbst} and Table~\ref{table:orgvsbsttime} compare the effectiveness and efficiency with $k=30$ and $|S|=50$. We have four main observations:
%The main observation is that the boosted versions can achieve about five-order-of-magnitude larger influence than their original counterparts but can be still outperformed by \outtermethod{}. Specifically, \outtermethod{} outperforms the second best performer by at least 23\%-39\% on different datasets respectively. More observations are in Appendix~\ref{appendix:casestudy}. Due to the poor performance of the original baselines, we only use the boosted versions for comparison in the rest of experiments.  
%\subsection{Case study on two versions of baselines}\label{exp:casestudy}
%We have two observations in Table~\ref{table:orgvsbst}:
%(1) the performance gap between original versions of baselines and \outtermethod{} is much more greater than the one in Section 6.1 such that \outtermethod{} can achieve up to five-order-of-magnitude larger influence (e.g., on Orkut). This observation is mainly caused by the significant difference in the topological information of the input diffusion network and the size of edge insertions. Specifically, in Section 6.1, the diffusion network is the original network which contains rich topological information and the size of edge insertions is quite small. On the other hand, in this section, the original versions start from a diffusion network which initially only contains seed nodes and face considerable edge insertions which contribute all influence increment of seeds.
\vspace{-1mm}
\begin{enumerate}[leftmargin = *]
\item \method{Org-Random} is more effective than the original versions of other baselines. The reason is that nodes with high degrees will `attract' much more incoming edges in other strategies (i.e., \method{Org-Degree} and \method{Org-FoF}) which `waste' a lot of recommendation opportunities to repeatedly influence/activate these nodes. 

\item The boosted versions can achieve about five-orders-of-magnitude larger influence than their original counterpart but can still be notably outperformed by \outtermethod{}. Specifically, \outtermethod{} can still outperform the second best performer by at least 23\%-39\% on different datasets respectively, which demonstrates the effectiveness of both two stages (i.e., the expansion and filling stages). 

\item We also compute the constitution of the edges recommended by \outtermethod{} in the boosted baselines, and the result shows that \outtermethod{} only contributes 17\%-27\% of total edges in the diffusion network. The significant performance improvement of baselines with limited involvement of \outtermethod{} further demonstrates the effectiveness of \outtermethod{} in terms of identifying important edges and nodes for increasing the seeds' influence. 

\item \outtermethod{} is very competitive with other boosted baselines in terms of running time, because all methods involve the \emph{expansion} stage of \outtermethod{} (i.e., Lines 5-9 in Algorithm~\ref{alg:practicalframework}) which dominates the total computational cost.
\end{enumerate}
\vspace{-1mm}

Due to the poor performance of the original baselines, we only use the boosted versions for comparison in the rest experiments.  



\smallskip
\noindent \textit{\textbf{Exp2 - Effectiveness comparison with different $|S|$}}. 
%\subsection{Effectiveness Comparison with Different $|S|$}\label{exp:|S|effectiveness}
Figure~\ref{fig:diffs} compares the performance with different $|S|$. Our method \outtermethod{} consistently outperforms other methods across all instances while the performance of other methods is not stable, e.g., \method{Bst-Random} outperforms \method{Bst-Degree} on Catster but the latter is more effective on Orkut. Another interesting observation is that the performance ranking of methods on the same dataset is consistent across different $|S|$. We think that a good edge recommendation for a non-seed user $u$ under an instance with a small $|S|$ can also be an effective recommendation for $u$ as the seed user under an instance with a great $|S|$. Thus, the diffusion networks generated by the expansion stage of \outtermethod{} under different $S$ can be similar such that edges chosen by a specific baseline upon these networks have large overlaps, which explains this observation.


\smallskip
\noindent \textit{\textbf{Exp3 - Effectiveness comparison with different $k$}}. 
%\subsection{Effectiveness comparison with different $k$}\label{exp:keffectiveness}
Figure~\ref{fig:diffk} compares the performance at different $k$ across all datasets. We have four main observations: 
\vspace{-1mm}
\begin{enumerate}[leftmargin = *]
\item \outtermethod{} outperforms the boosted baselines and can achieve up to two-orders-of-magnitude larger influence (e.g., on Orkut). 
\item The performance gap becomes smaller when $k$ is larger. The reason is that all methods make almost the same recommendation strategy to low-degree nodes since their out-degrees are close to or even smaller than $k$. In this case, the number of combinations of $k$ outgoing edges of these nodes is very limited. This observation also explains why the performance gap is larger on datasets with greater average degrees. 
\item When $k$ is small (e.g., 10), all methods achieve similar influence since it is barely possible for any method to achieve large influence with very limited edges. 
\item The performance gap on MOBA and RPG is not as significant as that on other datasets. That is because the average edge weight on MOBA and RPG are notably larger. Thus, regardless of how the diffusion network is generated, seeds can easily influence many nodes with sufficient influence probabilities. 
\end{enumerate}
\vspace{-1mm}
      
Note that the performance difference may not be easily distinguished visually due to the log scale of y axis, but we have shown the notable performance difference with $k=20$ and $k=30$ in Figure~\ref{fig:diffs} and Table~\ref{table:orgvsbst} at a finer granularity already. 

\begin{figure}[t]
\includegraphics[width=0.4\textwidth]{./drawing2/legend2}
\vspace{-0.45cm}

\centering
\subfloat[varing $k$]{
\includegraphics[width=0.2\textwidth]{./drawing2/diffkiter_RMPP.pdf}\hspace{-1em}
} 
\hspace{0.5mm}
\subfloat[varing $|S|$]{
\includegraphics[width=0.2\textwidth]{./drawing2/difftiter_RMPP.pdf}\hspace{-1em}
}

\vspace{-1.em}
\caption{The number of iterations in the expansion stage with different $k$ and $|S|$.}\label{fig:convergence}
%\vspace{-3.em}
\end{figure}


\begin{figure}[t]
\includegraphics[width=0.4\textwidth]{./drawing2/legend2}
\vspace{-0.45cm}

\centering
\subfloat[varing $k$]{
\includegraphics[width=0.21\textwidth]{./drawing2/diffktime_RMPP.pdf}\hspace{-1em}
} 
\hspace{0.5mm}
\subfloat[varing $|S|$]{
\includegraphics[width=0.21\textwidth]{./drawing2/diffttime_RMPP.pdf}\hspace{-1em}
}

\vspace{-1.em}
\caption{Running time of \outtermethod{} with different $k$ and $|S|$.}\label{fig:efficiency}
\end{figure}


\begin{figure}[t]
\includegraphics[width=0.4\textwidth]{./drawing2/legend2}
%\vspace{-0.45cm}

\centering
\includegraphics[width=0.2\textwidth]{./drawing2/nodeparti_RMPP.pdf}\hspace{-1em}

\vspace{-1.5em}
\caption{The percentage of the nodes in the diffusion network over the one in the original network with different iterations in the expansion stage of \outtermethod{}, where the iterations with solid fill refer to the convergence points under different datasets repsectively.}\label{fig:noderatio}
%\vspace{-1.5em}
\end{figure}


\begin{figure}[t]
\includegraphics[width=0.33\textwidth]{./drawing2/legend3}
\vspace{-0.45cm}

\centering
\subfloat[RPG]{
\includegraphics[width=0.2\textwidth]{./drawing2/INEratio_RPG.pdf}\hspace{-1em}
} 
\hspace{0.5mm}
\subfloat[Orkut]{
\includegraphics[width=0.2\textwidth]{./drawing2/INEratio_Orkut.pdf}\hspace{-1em}
}

%\vspace{-1.em}
\caption{The influence ratio (I-Ratio), edge ratio (E-Ratio) and node ratio (N-Ratio) in the diffusion network produced by \outtermethod{} with different $k$.}\label{fig:INERatio} 

\end{figure}







\smallskip
\noindent \textit{\textbf{Exp4 - Impact of $k$ and $|S|$ on \outtermethod{} convergence}}. 
%\subsection{Impact of $k$ and $|S|$ on \outtermethod{} Convergence}\label{exp:convergence}
Figures~\ref{fig:convergence} (a) and (b) show the number of iterations in the expansion stage of \outtermethod{} when varing $k$ and $|S|$ respectively. Interestingly, when $k$ or $|S|$ increases, the number of iterations for convergence is non-increasing. This is because \outtermethod{} will include more nodes into the current \ksubnetwork{} in each iteration such that it may take fewer iterations to identify all important nodes for influence spread.


\smallskip
\noindent \textit{\textbf{Exp5 - Scalability study on \outtermethod{}}}. 
%\subsection{Scalability Study on \outtermethod{}}\label{exp:scalability}
Figures~\ref{fig:efficiency} (a) and (b) show the runtime of our (full-stage) \outtermethod{} when varing $k$ and $|S|$. As $k$ grows, more nodes tend to be included in the diffusion network and more edges tend to be `filled up' in the filling stage, hence costing more time. On the other hand, increasing $|S|$ does not notably incur more computation costs, for two reasons: 1) we transform the case of multiple seeds into the one of a single virtual node by introducing only $|S|$ extra edges into the diffusion network; 2) the size of the diffusion networks generated under instances of different $|S|$ can be similar as discussed earlier. It is obvious to see that \outtermethod{} is highly scalable and efficient, since it can produce good recommendation on datasets with millions of nodes and hundred millions of edges within two hours (e.g., Orkut). This performance is promising since such recommendation is usually deployed for a long-term usage.


\smallskip
\noindent \textit{\textbf{Exp6 - Impact of iterations on the diffusion network node size}}. 
%\subsection{Impact of iterations on the network size}\label{exp:interation}
Figure~\ref{fig:noderatio} shows how the node size of the diffusion network in the expansion stage of \outtermethod{} grows iteratively. Here, the iterations with solid fill refer to the convergence points. Note that the expansion stage is terminated after convergence for other experiments and here we force it to run 10 iterations. It is obvious that, the node size in the diffusion network converges as the influence spread, which indicates the effectiveness of the convergence criteria.
% in \outtermethod{} and its effectiveness in identifying important nodes for spreading influence. 

\smallskip
\noindent \textit{\textbf{Exp7 - Case study with large $k$}}. 
%\subsection{Case Study with Large $k$}\label{exp:largek}
Here, we conduct a case study on the two largest datasets, RPG and Orkut. Our goal is to show how the statistics of the diffusion network produced by \outtermethod{} and influence spread of seed nodes in this network will change when we further increase $k$ up to 50. Specifically, we use the \emph{influence ratio} (I-Ratio) to denote the percentage of the influence of seeds in the diffusion network over their full influence in the original network, \emph{edge ratio} (E-Ratio) and \emph{node ratio} (N-Ratio) to denote the percentage of the edge and node size of the diffusion network over the ones of the original network, respectively. As shown in Figure~\ref{fig:INERatio}, as $k$ increases, \outtermethod{} is able to achieve an I-Ratio of 90\% with only an E-Ratio of 36\%, and an I-Ratio of 94\% with only an E-Ratio of 46\% on RPG and Orkut respectively. These again demonstrate the superiority of \outtermethod{}. 
Furthermore, when the N-Ratio converges, the I-Ratio can still notably increase as $k$ grows, and even the converged N-Ratio can be notably smaller than 1 (e.g., on RPG). These indicate that \outtermethod{} can identify important nodes for spreading the influence. 


\iffalse
\smallskip
\noindent \textbf{More Experiments on open social networks}. We also conduct experiments on the problem of maximizing the seeds' influence in \emph{open} social networks. Specifically, this problem assumes \emph{all} friends to be recipients for further information propagation, and aims to insert a limited number of edges (i.e., constructing new friendships) into the network to maximize the seeds' influence. We compare our method \outtermethod{} with several baselines including the state-of-the-art~\cite{chaoji2012recommendations} with approximation guarantees. The results show that: 1) \outtermethod{} is able to effectively maximize the influence of multiple seed nodes while achieving five-orders-of-magnitude speedups than~\cite{chaoji2012recommendations}; 2) \outtermethod{} is robust to different edge insertion constraints for maximizing the seeds' influence. Please refer to our technical report~\cite{TR} for details.
\fi


\subsection{Deployment}\label{sec:deploy}
In order to demonstrate the practical effectiveness of our \short{} problem, we deployed our solution into an activity in a multi-player online battle arena game of Tencent of which the friendship network is MOBAX in Table~\ref{table:dataset}.

\smallskip
\noindent \textbf{Summary of the activity}.
Users join this activity by interacting (e.g., sending gifts and gaming invitation) with their friends recommended by the system and will obtain rewards via such interactions. This form of interaction could trigger domino effects such that the interactions can stimulate the message receiver to further interact with other users. The aim of this activity is to improve user retention and interactions. Note that, in this activity, we do not specifically designate seeds. Instead, every user could be a potential and spontaneous seed. Specifically, users who log in the game will see this activity and may perform three possible behaviors: (1) proactively start interactions as a seed, (2) start interactions as a message receiver (i.e., a non-seed) and (3) ignore this activity. 

\smallskip

\noindent \textbf{Edge weights and the diffusion model}. We adopt the same settings as we use for generating edge weights on MOBA and RPG, and generate the diffusion network based on the IC model. Note that the IC model is only used for generating the diffusion network but not used for evaluation since it is very likely that the real-world influence will not spread in a way specified by the IC model or any other classical diffusion models (e.g., Linear Threshold model~\cite{Kempe03}).

\smallskip
\noindent \textbf{Methods for comparison}. Four methods, namely \method{Random}, \method{Degree}, \method{FoF} and \outtermethod{}, are deployed. For evaluation, we use an online A/B testing. Specifically, it randomly assigns each online user to one of these four methods which recommend a list of friends for each assigned user.
% and the graph induced by users assigned to \outtermethod{} forms the MOBA dataset in Table~\ref{table:dataset}. 
The list size $k$ is set as 20 for all methods because, in this application, only 20 friends are shown due to several reasons (e.g., the screen size and resolution settings of most mobile devices).
Based on our observations made in Section~\ref{sec:exp-closed}, the k-subnetwork generated based on a given seed set could also be effective for different seed sets.
Thus, for \outtermethod{}, we first generate the \ksubnetwork{} with top 10\% of assigned users with the highest degrees as the seeds, and then use this generated \ksubnetwork{} for this activity where every user could be a potential seed or non-seed.



\smallskip
\noindent \textbf{Experimental results}. The number of users who interact with the recommended friends directly indicates the quality of the underlying recommendation system and can effectively reflect the potential size of users who are impacted by others to perform interactions. 
Thus, to evaluate the performance, we adopt the Click-through Rate (CTR) which is a very popular evaluation metric for recommendation systems in industry. The CTR denotes the number of users who interacted with recommended friends divided by the total number of users who log in the game during this activity. %Since it is intractable to capture the influence spread in practice, CTR is a good alternative metric for evaluation in industry. 
The CTR achieved by \method{Random}, \method{Degree}, \method{FoF} and \outtermethod{} are 81.87\%, 82.73\%, 82.81\% and \textbf{88.14\%} respectively, which again demonstrates the effectiveness of \outtermethod{}. Despite the effectiveness of CTR, there still exist some other evaluation metrics (e.g., the actual influence spread of seeds via knowing the propagation paths and who are the seeds) worthy of explorations. However, due to the privacy restriction of this activity, we have no access to the detailed information in user logs to compute the performance under other potential metrics. In future, we would like to see how our proposed method will perform in other activities under various evaluation metrics.




==> imcsnvldb2023 copy/tex/temp.tex <==

\section{Theoretical Analysis}



\begin{algorithm}[!t] 
  \algsetup{linenosize=\footnotesize}
\footnotesize
 \caption{Naive Greedy}
   \SetKwInOut{Input}{Input}
   \SetKwInOut{Output}{Output}
  \Input{The input network $G$, the target user $t$ and an integer $k$.}
  \Output{A diffusion network.}

$G_d \leftarrow $ initialize the diffusion network from $G$ where the out-neighbors of any node is not greater than $k$\;

\ForEach{ node $v \in G_d$}{
	\lIf{$N^{G_d}_{out}(v)=k$ or $N^{G}_{out}(v)$}{
		Remove edges $(v,\cdot)$ from $G$
	}
	\lElse{
			Remove edges $(v,\cdot)$ in $G_d$ from $G$
	}

}

$G_r \leftarrow G$\;

\While{$G_r$ has edges}{
	$(x,y) = \argmax_{ (u,v) \in G_r}   \delta(t)_{G_d \cup \{(u,v)\}}$\;
	Add $(x,y)$ into $G_d$; remove $(x,y)$ from $G_r$\;
	\lIf{$N^{G_d}_{out}(x)=k$}{
		Remove all edges $(x,\cdot)$ from $G_r$.
	}
	

}



\Return $G_d$\;


\end{algorithm}











\begin{algorithm}[!t] 
  \algsetup{linenosize=\footnotesize}
\footnotesize
 \caption{Dijkstra}
   \SetKwInOut{Input}{Input}
   \SetKwInOut{Output}{Output}
  \Input{The input graph $G$, the target user $t$ and influence probability dictionary $orgPr$.}

  $l \leftarrow$ the set of nodes reached by $t$ in $G_d$\;
  
  \ForEach{node $u \in l$}{ $orgPr[u]=0$ \;
       \lIf{$u=t$}{$orgPr[u]=1$ } }
  $h \leftarrow$ a max heap based on the values of $(u:orgPr(u))$ for all nodes in $l$ and $t$.
  
  \While{$h$ is not empty}{
  		$(u:orgPr(u))=h.pop()$\;
  		\ForEach{$v \in N_{out}(u)$}{
  			\If{$v$ in $h$ and $orgPr(u)* w_{(u,v)} > orgPr(v)$}{
  				$orgPr(v)=orgPr(u)* w_{(u,v)} $\;
  				update existing $(v:orgPr(v))$ in heap $h$\;
  			}		
  		}
  }
  
\end{algorithm}


\begin{algorithm}[!t] 
  \algsetup{linenosize=\footnotesize}
\footnotesize
 \caption{LocalDijkstra}
   \SetKwInOut{Input}{Input}
   \SetKwInOut{Output}{Output}
  \Input{The input graph $G$, an edge candidate $(u,v)$, the probability $orgPr(u)*w_{(u,v)}$ of the maximum probability path from $t$ to $v$ containing $(u,v)$, and influence probability dictionary $curPr$.}
  \Output{The marginal gain of $(u,v)$.}
$pr=orgPr(u)*w_{(u,v)}$ ; $gain=0$ ; $S=\emptyset$\;
  $h \leftarrow$ a max heap initialized with $(v:pr))$; $tempPr \leftarrow$ empty dictionary\;
  \While{$h$ is not empty}{
  		$(u:pr))=h.pop()$; $S=S\cup \{u\}$\;
  		$gain=gain+pr-curPr(u)$\;
  		\ForEach{$v \in N_{out}(u)$}{
  			\If{$(u,v)$ is not an inserted edge and $v \notin S$}{
  			$pr_v= v \text{ exists in } tempPr?\: tempPr(v):curPr(v)$\;
  				  			\If{$pr * w_{(u,v)} > pr_v$}{
  				  				 $tempPr(v)=pr * w_{(u,v)}$\;
  				  			    \lIf{$v$ is not in $h$}{  insert $(v:tempPr(v))$ into $h$}
  				  				\lElse{update existing $(v:tempPr(v))$ in heap $h$}
  				  				
  				  			}	
  			
  			
  			}
  			
  		}
  }
  
\end{algorithm}




\begin{algorithm}[!t] 
  \algsetup{linenosize=\footnotesize}
\footnotesize
 \caption{AutoFill}
   \SetKwInOut{Input}{Input}
   \SetKwInOut{Output}{Output}
 \Input{The input network $G$, the current diffusion network $G_d$ and an integer $k$.}

 $L \leftarrow$ nodes in $G_d$ ranking by the their subtree sizes of the spanning RMPP tree rooted by $t$.
 
 \ForEach{$v \in L$}{
 
	\ForEach{$u \in N_{in}^G(v)$}{
		\If{$u \in G_d$ and $N_{out}^{G_d}(u)<min(N_{out}^{G}(u), k)$}{
			insert $(u,v)$ into $G_d$
		
		}
	
	}
 

 }
 
 
\end{algorithm}

\begin{algorithm}[!t] 
  \algsetup{linenosize=\footnotesize}
\footnotesize
 \caption{AdvancedFill}
   \SetKwInOut{Input}{Input}
   \SetKwInOut{Output}{Output}
 \Input{The input network $G$, the current diffusion network $G_d$ and an integer $k$.}

 $L' \leftarrow$ nodes ranked by their influence probability by $t$ in $G_d$.
 
 
 
 \ForEach{$u \in L'$}{
 	$L^\# \leftarrow$ out-neighbors of $u$ ranked by their the number of edge incidence in ascending order and then subtree size in descending order. // edge incidence of $v$ refers to the number of incoming neighbors of $v$ introduced in this algorithm, initialized as 0\;
 	
 	$L^\# \leftarrow$ first $min(N_{out}^{G_r}(u), k-N_{out}^{G_d}(u) )$ nodes in $L^\#$\;
	\ForEach{$v \in L^\#$}{
	   Add $(u,v)$ into $G_d$\;
	   $Incidence[v]+=1$\;
	
	}
 

 }
 
 
\end{algorithm}




\begin{algorithm}[!t] 
  \algsetup{linenosize=\footnotesize}
\footnotesize
 \caption{DiffusionNetworkAugmentation (DNA2)}
   \SetKwInOut{Input}{Input}
   \SetKwInOut{Output}{Output}
  \Input{The input network $G$, the initial diffusion network $G_d$, the target user $t$ and an integer $k$.}
  \Output{The updated diffusion network $G_d$.}

%$G_d \leftarrow $ initialize the diffusion network from $G$ where the out-neighbors of any node is not greater than $k$\;
$G_r \leftarrow $ empty graph\;
\ForEach{ node $u \in G_d$}{
	\lIf{$N^{G_d}_{out}(u)=k$ or $N^{G}_{out}(u)$}{
		Continue
	}
	\Else{
			\ForEach{$v \in N^{G}_{out}(u)$}{
				\lIf{$(u,v) \notin G_d$ }{  Add $(u,v)$ into $G_r$}}
	}

}

 $L \leftarrow$ nodes in $G_d$ ranking by the their subtree sizes of the spanning RMPP tree rooted by $t$.

\ForEach{$v$ in $L$}{
	$u^*_v= \argmax_{u \in N^{G_r}_{in}(v)}  orgPr(u)*w_{(u,v)} $\;
	\If{$orgPr(u^*_v)*w_{(u^*_v,v)} \leq orgPr(v)$}{Continue}
	Add $(u^*_v,v)$ into $G_d$, and remove $(u^*_v,v)$ from $G_r$\;
	\If{$N^{G_d}_{out}(u^*_v)=k$}{
		Delete all edges $(u^*_v,\cdot)$ from $G_r$.
	
	}

}



\Return $G_d$\;



\end{algorithm}

\begin{algorithm}[!t] 
  \algsetup{linenosize=\footnotesize}
\footnotesize
 \caption{MultiDiffusionNetworkAugmentation (MDNA)}
   \SetKwInOut{Input}{Input}
   \SetKwInOut{Output}{Output}
  \Input{The input network $G$, the initial diffusion network $G_d$, the target user set $S$ and an integer $k$.}
  \Output{The updated diffusion network $G_d$.}

%$G_d \leftarrow $ initialize the diffusion network from $G$ where the out-neighbors of any node is not greater than $k$\;
$G_r \leftarrow $ empty graph\;
\ForEach{ node $u \in G_d$}{
	\lIf{$N^{G_d}_{out}(u)=k$ or $N^{G}_{out}(u)$}{
		Continue
	}
	\Else{
			\ForEach{$v \in N^{G}_{out}(u)$}{
				\lIf{$(u,v) \notin G_d$ }{  Add $(u,v)$ into $G_r$}}
	}

}

 $L \leftarrow$ nodes in $G_d$ ranking by the their subtree sizes of the spanning RMPP tree rooted by the ghost node $x$.

\ForEach{$v$ in $L$}{
	$u^*_v= \argmax_{u \in N^{G_r}_{in}(v)}  orgPr_x(u)*w_{(u,v)} $\;

	Add $(u^*_v,v)$ into $G_d$, and remove $(u^*_v,v)$ from $G_r$\;
	\If{$N^{G_d}_{out}(u^*_v)=k$}{
		Delete all edges $(u^*_v,\cdot)$ from $G_r$.
	
	}

}



\Return $G_d$\;



\end{algorithm}


\begin{algorithm}[!t] 
  \algsetup{linenosize=\footnotesize}
\footnotesize
 \caption{DiffusionNetworkAugmentation (DNA)}
   \SetKwInOut{Input}{Input}
   \SetKwInOut{Output}{Output}
  \Input{The input network $G$, the initial diffusion network $G_d$, the target user $t$ and an integer $k$.}
  \Output{The updated diffusion network $G_d$.}

%$G_d \leftarrow $ initialize the diffusion network from $G$ where the out-neighbors of any node is not greater than $k$\;
$G_r \leftarrow $ empty graph\;
\ForEach{ node $u \in G_d$}{
	\lIf{$N^{G_d}_{out}(u)=k$ or $N^{G}_{out}(u)$}{
		Continue
	}
	\Else{
			\ForEach{$v \in N^{G}_{out}(u)$}{
				\lIf{$(u,v) \notin G_d$ }{  Add $(u,v)$ into $G_r$}}
	}

}

Compute $u^*_v$ for every $v \in G_r$\;

\While{$G_r$ has edges}{
	$v^*=\argmax_{ v\in G_r}  \delta(t)_{G_d \cup \{ (u^*_v,v) \}}-\delta(t)_{G_d}  $\;
	Add $(u^*_{v^*},v^*)$ into $G_d$, remove all edges $(\cdot, v^*)$ from $G_r$\;
		

		\If{$N^{G_d}_{out}(u^*_v)=k$}{
			\ForEach{$x \in N^{G_d}_{out}(u^*_v)$}{
				\If{$u^*_x=u^*_v$}{
					update $u^*_x$\;
				}
			
			}
			Delete all edges $(u^*_v,\cdot)$ from $G_r$.
		
		}

}


\Return $G_d$\;


\end{algorithm}

\section{Related work}
We will introduce related work on targeted influence maximization via edge insertions and edge deletion. 

\noindent \textbf{Targeted influence maximization via edge insertions}. \citeauthor{d2019recommending}~\cite{d2019recommending} introduced the Influence Maximization with Augmentation problem
(IMA) under the IC model which aims to add a limited number of edges incident to a given set
of seeds in order to maximize influence of the seeds. \citeauthor{coro2021link}~\cite{coro2021link} extends the results of ~\cite{d2019recommending} to the LT model. They prove that the objective function under LT model is modular and leverage this property to propose an approximation algorithm. The problem studied by these two works is much simpler than ours since (1) they limit that the edges being added must be incident on the seeds which derives good theoretical properties to solve this problem and (2) there is no constraints on the number of inserted edges incident on each node ($k$ in our problem). 
\citeauthor{khalil2014scalable}~\cite{khalil2014scalable} study adding a limited number of edges to maximize influence of given seeds under LT model. Their method cannot handle IC model and does not consider the constraint of edge incidence on any node.


\citeauthor{chaoji2012recommendations}~\cite{chaoji2012recommendations} study adding edges to maximize the influence spread of seeds under the constraint that at most $k$ inserted edges are incident on any node, which is the most similar work to our problem among all study in this category. However, their proposed method cannot directly solve our equivalent problem via edge insertion since their method estimate pairwise influence via constrained paths which can only contain at most one edges being inserted. In our problem setting via edge inserting, the graph is initially empty and will only contain inserted edges after graph update. Furthermore, their method involving costly belief propagation which cannot scale to real-world social networks. 

\citeauthor{yang2019marginal}~\cite{yang2019marginal}, \citeauthor{yang2020boosting}~\cite{yang2020boosting} and \citeauthor{yu2020maximizing}~\cite{yu2020maximizing} consider adding a limited number of edges from a candidate set to maximize the influence of the seeds under the IC model. \citeauthor{yang2019marginal}~\cite{yang2019marginal}, \citeauthor{yang2020boosting}~\cite{yang2020boosting} derive lower and upper bound influence function to approximate the non-submodular influence in IC model and use a sandwich strategy to approximate the solution. \citeauthor{yang2020boosting}~\cite{yang2020boosting} derives tighter bound than \citeauthor{yang2019marginal}~\cite{yang2019marginal}. \citeauthor{yu2020maximizing}~\cite{yu2020maximizing} leverage the idea of constrained paths in~\cite{chaoji2012recommendations} to derive a submodular influence function, and then use the standard greedy to find the approximate solution. All of these three works do not consider the constraint that at most $k$ added edges can be incident on any node. Furthermore, they consider the number of edges to be added and the candidate edge set size to be quite small. However, in our problem from the perspective of edge insertion, the number of edges to be added is up to $k|V|$ and the candidate edge set consists of all edges in the original network. Furthermore, they can only work for acyclic graphs!


 

\noindent \textbf{Targeted influence maximization via edge deletion}. \citeauthor{kimura2008minimizing}~\cite{kimura2008minimizing} study removing a limited number of edges such that the average influence of all the nodes in the graph is minimized. \citeauthor{khalil2014scalable}~\cite{khalil2014scalable} study removing a limited number of edges to minimize the influence of given seeds.
\citeauthor{wang2020efficient}~\cite{wang2020efficient} study removing a set of edges to minimize the influence of given seeds to a predefined set of users. \citeauthor{medya2019influence}~\cite{medya2019influence} study a similar problem but under the credit distribution model~\cite{goyal2011data} where the influence is much more easier to be computed compared with IC and LT model. \citeauthor{nandi2016methods}~\cite{nandi2016methods} investigate the effectiveness of link removal as an intervention to minimize the spread of infections in a network. They develop four network interdiction models with different objectives and formulate these models as mixed integer linear programs. \citeauthor{pham2018maximizing}~\cite{pham2018maximizing} aim to find a
set of nodes whose removal from a social network maximizes the influence reduction from the source of misinformation within time and budget constraints.

In summary, all work in this category is different from our equivalent problem via edge deletion in two aspects: (1) the objective is different. They all aim to minimize the influence of the target seed nodes in the residue graph whereas we aim to maximize the influence. (2) constraints of the residue graph. Existing work does not have constraints on the structure of the residue graph whereas we require that each node in the residue graph can have at most $k$ out neighbors.

==> imcsnvldb2023 copy/tex/visualization.tex <==
\begin{figure*}[!t]


\subfloat[Hamster]{
\includegraphics[width=0.5\textwidth]{./figures2/Hamster_distance.png}
}
\subfloat[Instagram]{
\includegraphics[width=0.5\textwidth]{./figures2/Instagram_distance.png}
}







\caption{Visualization of pricing schemes FCInf-Greedy and FCMWS-Greedy.}\label{effect:visualization}
\vspace{-0.36cm}
\end{figure*}

==> tex/experiment.tex <==
\section{Experiment}\label{sec:experiment}
{In this section, we will conduct experiments on three problems to demonstrate the robustness and effectiveness of our methods:  }

\begin{itemize}[leftmargin = *]
\item The first problem is maximizing the influence in \emph{open} social networks via edge insertions, where existing baselines including the state-of-the-art~\cite{chaoji2012recommendations} are compared (Section~\ref{sec:exp-open}). 
\item The second is our proposed problem, \short{},  where the extensions of the methods in the first problem are compared (Section~\ref{sec:exp-closed}). Note that the core difference between these two problems has been illustrated and please refer to Section~\ref{sec:relatedwork} for details.
\item The third problem is maximizing users' Click-trough Rate in an activity of an online Tencent application, where we deploy our method and evaluate how it helps improve user retentions and interactions (Section~\ref{sec:deploy}). 
\end{itemize}


\smallskip
\noindent\textbf{Datasets}. Table~\ref{table:dataset} presents all the real-world undirected social networks used. In particular, MOBA and MOBAX correspond to two friendship networks of Tencent multiplayer online battle arena games, RPG corresponds to a friendship network of a role-playing game, and the other datasets are available in~\cite{konect}. Note that each edge is represented twice since the influence propagation is directed. To obtain experimental results in a reasonable time under different problem settings, the first four datasets, the next four datasets and the last dataset will be used for the first, the second and the third problem,  respectively.


\smallskip
\noindent \textbf{Environments}. We conduct all experiments on a Linux server with Intel Xeon E5
(2.60 GHz) CPUs and 512 GB RAM. All algorithms are implemented in
Python and our code is available at~\cite{TR}. 





\begin{table}[]
\caption{Dataset Statistics}\label{table:dataset}
\begin{tabular}{cccc}
\hline
\textbf{Dataset} & \textbf{|V|} & \textbf{|E|} & \textbf{Avg. Degree} \\ \hline
EU-Core & 1,005 & 51,142 & 51 \\
Hamster & 2,426 & 33,261 & 14 \\
CiaoDVD & 4,658 & 80,266 & 17 \\
Brightkite & 58,228 & 428,156 & 7 \\ 
%Livemocha & 104,103 & 4,386,166 & 42\\
Catster &149,700 & 10,898,550 & 73\\
MOBA & 503,029 & 9,372,022 & 19 \\
RPG  & 2,331,047 & 88,227,562 & 38\\
Orkut & 3,072,441 & 234,369,798 & 76\\
MOBAX & 36,201,207&3,281,207,036&90\\ \hline
\end{tabular}
\end{table}


\subsection{Experiment with the Open Sharing Model}\label{sec:exp-open}
In this section, we study maximizing the influence in open social networks. Here, we insert a set $X'$ of edges from the candidate set $X$ into the original social network such that (1) at most $k$ edges in $X'$ share the same source node and (2) the influence sum of the seed nodes is maximized. The purpose of this section is twofold: 
\begin{itemize}[leftmargin = *]
\item Our proposed method \outtermethod{} is able to effectively maximize the influence of multiple seed nodes, as compared to the state-of-the-art called continuous greedy \method{CG}~\cite{chaoji2012recommendations} on this problem.
 %Specifically, \method{CG}~\cite{chaoji2012recommendations} studies a slightly different problem where at most $k$ edges in $X'$ share the same source \emph{or} end nodes. 
\item Our proposed method \outtermethod{} is robust to different variations of influence maximization via edge recommendations.
\end{itemize}

\smallskip
\noindent \textbf{Baselines}. Baselines are listed below where \method{Degree} and \method{FoF} (i.e., Friend of Friend) were also compared by \method{CG}~\cite{chen2009efficient}. For ease of description, we assume out-degrees of nodes in the original network to be greater than $k$.

\begin{itemize}[leftmargin = *]
\item \method{Degree} based method where, for candidates sharing the same source node, top $k$ edges with the highest degrees of end nodes are selected.

\item \method{FoF} based method where,  for candidates sharing the same source node, top $k$ edges whose source and end nodes share the highest number of common friends are selected.

\item \method{Random} based method where $k$ edges are randomly selected from candidates sharing the same source node. Its performance is reported as the average over five independent runs.

\item \method{CG}~\cite{chaoji2012recommendations} where edges are inserted based on a continuous greedy method followed by randomized rounding. We set all parameters as recommended by the original work.
\end{itemize}


\smallskip
\noindent \textbf{Edge Weight Settings}. We follow the previous work~\cite{chaoji2012recommendations} to adopt the constant model where each edge in the original network and candidate edge for insertion is assigned with a constant influence probability and we set it as 0.1. Note that the constant model and the influence probability setting are also commonly used by existing studies in the classical influence maximization problem~\cite{arora2017debunking,goyal2011celf++,Kempe03}.
 
\smallskip
\noindent \textbf{Parameter Settings}. Considering that \method{CG} is not scalable to a large number of seed nodes and edge candidates, we conduct experiments on small-scale datasets. Specifically, we randomly select five nodes from the top 1\% nodes with the highest degrees in the original network as the seed nodes. Afterwards, we generate 50 outgoing edges from each node within two hops away from the seed nodes as candidates, and these candidates are generated randomly by following the setup of~\cite{chaoji2012recommendations} where an edge candidate can be added between any pair of nodes without group information. We set $k$ as 20, the error ratio $\epsilon$ of \outtermethod{} as $10^{-4}$, and follow the common standard~\cite{arora2017debunking} to estimate the influence of any solution under the IC model via 10,000 Monte Carlo simulations.



\smallskip
\noindent \textbf{Experimental Results}. Table~\ref{table:openinf} compares the influence spread achieved by different methods under the RMPP model  and the IC model, respectively. It is obvious that there is a positive correlation between influence under the RMPP model and the one under the IC model. That is, greater influence under the former one also indicates larger influence under the latter. Hence, the idea of optimizing the RMPP-based influence spread to approximate the IC-based influence is effective. \outtermethod{} significantly outperforms \method{Degree}, \method{FoF} and \method{Random}, and achieves very competitive results with \method{CG}. Furthermore, \outtermethod{} achieves up to five-orders-of-magnitude speedup over \method{CG} as shown in Table~\ref{table:opentime}. These results demonstrate the efficiency, effectiveness and robustness of \outtermethod{}, in terms of maximizing the  influence of multiple seed nodes via edge recommendations/insertions. 



\begin{table}[]
\caption{Comparison of influence achieved by different methods under the RMPP model (RP) and the IC model.}\label{table:openinf}
\begin{tabular}{ccccccccc}
\hline
\multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c}{\textbf{EU-Core}} & \multicolumn{2}{c}{\textbf{Hamster}} & \multicolumn{2}{c}{\textbf{CiaoDVD}} & \multicolumn{2}{c}{\textbf{Brightkite}} \\ \cline{2-9} 
 & \textbf{RP} & \textbf{IC} & \textbf{RP} & \textbf{IC} & \textbf{RP} & \textbf{IC} & \textbf{RP} & \textbf{IC} \\ \hline
Degree & 65 & 2801 & 65 & 2513 & 92 & 5891 & 80 & 8912 \\
FoF & 68 & 3012 & 67 & 2789 & 95 & 6013 & 75 & 8134 \\
Random & 70 & 3189 & 64 & 2445 & 100 & 6231 & 73 & 7986 \\
\outtermethod{} & 76 & 3684 & 72 & 3142 & 109 & 6618 & 88 & 12034 \\
CG & 78 & 3769 & 74 & 3221 & 109 & 6680 & 89 & 12851 \\ \hline
\end{tabular}
\end{table}



\begin{table}[]
\caption{Running time comparison between CG and \outtermethod{}.}\label{table:opentime}
\begin{tabular}{ccccc}
\hline
\textbf{Method} & \textbf{EU-Core} & \textbf{Hamster} & \textbf{CiaoDVD} & \textbf{Brightkite} \\ \hline
\outtermethod{} & 5.8E-1 & 1.7E-1 & 1.5E0 & 1.7E1 \\
CG & 3.56E4 & 3.0E4 & 5.5E4 & 4.6E4 \\ \hline
\end{tabular}
\end{table}




\begin{table}[]
\caption{Effectiveness comparison with $k=30$ and $|S|=50$.}\label{table:orgvsbst}
\begin{tabular}{cccccccc}
\hline
\multirow{2}{*}{\textbf{Dataset}} & \multicolumn{2}{c}{\textbf{Degree}} & \multicolumn{2}{c}{\textbf{FoF}} & \multicolumn{2}{c}{\textbf{Random}} & \multirow{2}{*}{\textbf{\outtermethod{}}} \\ \cline{2-7}
 & \textbf{Ori} & \textbf{Bst} & \textbf{Ori} & \textbf{Bst} & \textbf{Ori} & \textbf{Bst} &  \\ \hline
%Livemocha & 6.1E2 & 7.8E5 &7.9E2& 8.0E5&2.9E3&8.3E5&\textbf{9.8E5}\\
Catster & 3.1E2 & 4.2E5 & 3.8E2 & 4.8E5 & 3.6E3 & 6.3E5 & \textbf{8.6E5} \\
MOBA & 5.0E6 & 7.4E6 & 6.5E6 & 7.7E6 & 7.0E6 & 8.0E6 & \textbf{9.8E6} \\
RPG & 1.1E6 &2.1E7 &   2.4E6 &2.2E7 &1.9E7 & 2.4E7 & \textbf{3.2E7} \\
Orkut & 7.0E2 & 5.4E7 & 6.8E2 & 5.6E7 & 9.6E5 & 5.9E7 & \textbf{8.2E7} \\ \hline
\end{tabular}

\end{table}


\iffalse
\begin{table}[]
\caption{Running time (s) comparison with $k=30$ and $|S|=50$ where the numbers in brackets under \outtermethod{} refers to the time cost in the graph expansion stage which is also involved in boosted baselines. Note that the number of common friends is pre-computed in \method{Bst-FoF}.}\label{table:orgvsbsttime}
\small
\begin{tabular}{cccccccc}
\hline
\textbf{Dataset} & \textbf{Bst-Degree} & \textbf{Bst-FoF} & \textbf{Bst-Random} & \textbf{\outtermethod{}} \\ \hline
Catster & 106.16 & 100.85 & 97.82 & 120.22 \\
MOBA &135.99& 129.19 & 125.31 & 177.63 \\
RPG & 957.20& 909.34 & 882.06 & 982.03\\
Orkut & 4436.54& 4214.71 & 4088.27 & 5094.28\\ \hline
\end{tabular}

\end{table}
\fi


\begin{table}[]
\caption{ Running time (s) comparison with $k=30$ and $|S|=50$ where the numbers in brackets under \outtermethod{} refers to the time cost in the graph expansion stage which is also involved in boosted baselines. Note that the number of common friends is pre-computed in \method{Bst-FoF}.}\label{table:orgvsbsttime}
\small
\begin{tabular}{cccccccc}
\hline
\textbf{Dataset} & \textbf{Bst-Degree} & \textbf{Bst-FoF} & \textbf{Bst-Random} & \textbf{\outtermethod{}} \\ \hline
Catster & 1.1E2 & 1.0E2 & 9.8E1 & 1.2E2 (9.1E1)\\
MOBA &1.4E2& 1.3E2 & 1.2E2 & 1.8E2 (1.3E2)\\
RPG & 9.6E2& 9.1E2 & 8.8E2 & 9.8E2 (7.3E2)\\
Orkut & 4.4E3& 4.2E3& 4.1E3 & 5.1E3 (3.6E3)\\ \hline
\end{tabular}

\end{table}





\begin{figure*}[t]
\includegraphics[width=0.5\textwidth]{./drawing2/legend1}
\vspace{-0.25cm}

\centering

\centering


\subfloat[Catster]{
\includegraphics[width=0.24\textwidth]{./drawing2/difft_Catster.pdf}\hspace{-1em}
}
\hspace{0.5mm}
\subfloat[MOBA]{
\includegraphics[width=0.24\textwidth]{./drawing2/difft_LOL.pdf}\hspace{-1em}
} 
\hspace{0.5mm}
\subfloat[RPG]{
\includegraphics[width=0.24\textwidth]{./drawing2/difft_RPG.pdf}\hspace{-1em}
}
\hspace{0.5mm}
\subfloat[Orkut]{
\includegraphics[width=0.24\textwidth]{./drawing2/difft_Orkut.pdf}\hspace{-1em}
}

\vspace{-0.7em}
\caption{Performance Comparison with different $|S|$.}\label{fig:diffs}
\vspace{-2.5em}
\end{figure*}



\begin{figure*}[t]
%\includegraphics[width=0.5\textwidth]{./drawing2/legend1}
%\vspace{-0.25cm}

\centering

\hspace{0.5mm}
\subfloat[Catster]{
\includegraphics[width=0.24\textwidth]{./drawing2/diffk_Catster.pdf}\hspace{-1em}
}
\subfloat[MOBA]{
\includegraphics[width=0.24\textwidth]{./drawing2/diffk_LOL.pdf}\hspace{-1em}
} 
\hspace{0.5mm}
\subfloat[RPG]{
\includegraphics[width=0.24\textwidth]{./drawing2/diffk_RPG.pdf}\hspace{-1em}
}
\hspace{0.5mm}
\subfloat[Orkut]{
\includegraphics[width=0.24\textwidth]{./drawing2/diffk_Orkut.pdf}\hspace{-1em}
}

\vspace{-0.7em}
\caption{Performance Comparison with different $k$.}\label{fig:diffk}
%\vspace{-1.5em}

\end{figure*}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\iffalse
\begin{figure*}[t]
\centering


\subfloat[Catster]{
\includegraphics[width=0.24\textwidth]{./drawing2/difftalltime_Catster.pdf}\hspace{-1em}
}
\hspace{0.5mm}
\subfloat[MOBA]{
\includegraphics[width=0.24\textwidth]{./drawing2/difftalltime_LOL.pdf}\hspace{-1em}
} 
\hspace{0.5mm}
\subfloat[RPG]{
\includegraphics[width=0.24\textwidth]{./drawing2/difftalltime_RPG.pdf}\hspace{-1em}
}
\hspace{0.5mm}
\subfloat[Orkut]{
\includegraphics[width=0.24\textwidth]{./drawing2/difftalltime_Orkut.pdf}\hspace{-1em}
}

\vspace{-0.7em}
\caption{Efficiency Comparison with different $|S|$.}\label{fig:diffsalltime}
\vspace{-2.5em}
\end{figure*}



\begin{figure*}[t]
%\includegraphics[width=0.5\textwidth]{./drawing2/legend1}
%\vspace{-0.25cm}

\centering

\hspace{0.5mm}
\subfloat[Catster]{
\includegraphics[width=0.24\textwidth]{./drawing2/diffkalltime_Catster.pdf}\hspace{-1em}
}
\subfloat[MOBA]{
\includegraphics[width=0.24\textwidth]{./drawing2/diffkalltime_LOL.pdf}\hspace{-1em}
} 
\hspace{0.5mm}
\subfloat[RPG]{
\includegraphics[width=0.24\textwidth]{./drawing2/diffkalltime_RPG.pdf}\hspace{-1em}
}
\hspace{0.5mm}
\subfloat[Orkut]{
\includegraphics[width=0.24\textwidth]{./drawing2/diffkalltime_Orkut.pdf}\hspace{-1em}
}

\vspace{-0.7em}
\caption{Efficiency Comparison with different $k$.}\label{fig:diffkalltime}
%\vspace{-1.5em}

\end{figure*}

\fi




\subsection{Experiment on the \short{} problem}\label{sec:exp-closed}
 We conduct seven experiments to demonstrate that: (1) the extension of existing baselines on open social networks cannot well address our problem but their performance can be significantly boosted with the help of our method \outtermethod{} (Exp1); (2) \outtermethod{} consistently and significantly outperforms all the boosted baselines with different $|S|$ and $k$ (Exp2-3); (3) how $k$ and $|S|$ impact the convergence of \outtermethod{} (Exp4); (4) \outtermethod{} is highly scalable to handle large-scale datasets (Exp5); (5) the influence convergence is also a good indicator of the node size convergence in the diffusion network (Exp6); (6) the influence of seeds in the diffusion network, produced by \outtermethod{} with a small edge size, is very competitive with the influnce of the seeds in the original network (Exp7).




\iffalse
\begin{table}[]
\caption{The percentage of edges recommended by the expansion stage of \outtermethod{} over the total edge size of the diffusion network produced by boosted baselines with $k=30$ and $|S|$. Note that the total edge size is the same across different boosted baselines since they are built upon the same input diffusion network.}\label{table:edgeparticapation}
\begin{tabular}{cccc}
\hline
\textbf{Livemocha}& \textbf{Catster} & \textbf{MOBA} & \textbf{Orkut} \\ \hline
					27\%		&		19\%				&			17\%&21\% \\ \hline
\end{tabular}
\end{table}
\fi



\smallskip
\noindent \textbf{Baselines}. We compare six baselines which include the aforementioned methods, \method{Degree}, \method{FoF} and \method{Random}, as well as their respective boosted versions. Since each baseline has two versions, original and boosted, we use the prefixes `Ori' and `Bst' to distinguish them. The boosted versions are built upon the diffusion network generated by the \emph{expansion} stage of \outtermethod{} (i.e., Lines 5-9 in Algorithm~\ref{alg:practicalframework}) and work similar to the original ones. The only difference is that, in the boosted version, some important edges have been inserted by \outtermethod{} and these baselines only `fill up' recommendations for those nodes in the generated diffusion network. Hence, if we assume that the out-degrees of nodes in the original network are greater than $k$ and our method has already inserted $h <k$ outgoing edges from $u$, these boosted versions just need to select $k-h$ outgoing edges for $u$. For the reason why \method{CG}~\cite{chaoji2012recommendations} cannot be extended, please refer to Section~\ref{sec:relatedwork} and its scalability issue in Section~\ref{sec:exp-open} for details.




\iffalse
\noindent \textbf{Baselines}. Six baselines are listed below. 
%Notably,  \method{Ori-Degree} and \method{Ori-FoF} were also compared by the state-of-the-art~\cite{chaoji2012recommendations} in open social networks. \bao{can remove the previous sentence.} 
For ease of description, we assume that the out-degrees of nodes in the original network are greater than $k$, and emphasize that all edges in the original network are candidates for insertion into the diffusion network which initially contains seed nodes only.

\begin{itemize}[leftmargin=*]
\item \method{Ori-Degree}: for candidates sharing the same source node, top $k$ edges whose end nodes have the highest degrees are selected.

\item \method{Ori-FoF}: for candidates sharing the same source node, top $k$ edges whose source and end nodes share the highest number of common friends are selected.

\item \method{Ori-Random}: $k$ edges are randomly selected from candidates sharing the same source node. Its performance is reported as the average performance over five independent runs.

\item \method{Bst-Degree}, \method{Bst-FoF} and \method{Bst-Random} are the boosted extension of the previous three methods, respectively. The boosted versions are built upon the diffusion network generated by the \emph{expansion} stage of \outtermethod{} (i.e., lines 5-9 in Algorithm~\ref{alg:practicalframework}) and work similarly to the original ones. The only difference is that, in the boosted version, some important edges have already been recommended/inserted by \outtermethod{} and these baselines just `fill up' recommendations for nodes in the generated diffusion network. Hence, if our method has already inserted $h<k$ outgoing edges from $u$, these boosted versions just need to select at $k-h$ outgoing edges for $u$. Since each baseline has two versions, original and boosted, we use the prefixes `Ori' and `Bst' to distinguish them.
\end{itemize}

%The method in~\cite{chaoji2012recommendations} is not considered, because in the input diffusion network which only contains seed nodes, it fails to help seeds influence the nodes that are more than one hop away. Moreover, there is no non-trivial extension of \method{CG} that is scalable to large-scale networks and can notably outperform our proposed method, as evidenced by experiments on a variation of our problem in open social networks~\cite{TR}.
\fi


\smallskip
\noindent \textbf{Edge Weight Settings}. Considering that the influence probability of edges are different in practice, we adopt the commonly used trivalency model~\cite{chen2010scalable} for Catster and Orkut without edge attributes. It randomly assigns a weight for each edge, from $\{10^{-1},10^{-2},10^{-3}\}$. 

For MOBA and RPG, we assign edge weights based on the intimacy of friendship. In MOBA and RPG, each pair of friends has different levels of intimacy which describes the number of interactions (e.g., the number of games they play together, the number of gifts sent from one to another). Since the pair-wise intimacy in both  MOBA and RPG is represented as integers, here we transform it into an influence probability within [0,1] for deployment in the IC model. According to the Susceptible-Infected-Recovered (SIR) model~\cite{anderson1992infectious} and heterogeneous mean-filed theory~\cite{newman2002spread,cohen2011resilience,castellano2010thresholds,xie2021detecting}, the lowest influence probability should not be smaller than a constant $\lambda$ times $\beta_c= \sum_{v \in V} |N_{out}(v)| / (\sum_{v \in V} |N_{out}(v)|^2- \sum_{v \in V} |N_{out}(v)|)$, where $\beta_c$ is the epidemic threshold in the SIR model and calculated as 0.024 and 0.001 on MOBA and RPG, respectively. If $\lambda \beta_c$ is too small, the influence of the seeds will be quite limited. If $\lambda \beta_c$ is too large, the influence spread can cover a large percentage of nodes, irrespective of where it originated, and the methods' performance cannot be well compared. By following existing studies~\cite{shu2015numerical,lu2016h}, we
determine $\lambda$ by simulation on real networks. Specifically, we determine $\lambda_1$ and $\lambda_2$ and control the edge weights within the range $[\lambda_1\beta_c, \lambda_2\beta_c]$. Each influence probability $p_{(u,v)}= ((u,v)_{I} - \min_{e\in E} e_{I}) / (\max_{e\in E} e_{I} -\min_{e\in E} e_{I}  ) (\lambda_2 -\lambda_1)\beta_c +\lambda_1\beta_c$ where $(u,v)_{I}$ denotes the intimacy between $u$ and $v$. Note that we have checked several settings of $\lambda_1$ and $\lambda_2$ and these different settings will not affect the conclusion (i.e., performance ranking of methods). To test these methods' robustness to the influence probability distributions, in both MOBA and RPG, we set the range $[\lambda_1\beta_c, \lambda_2\beta_c]$ as $[0.007,0.01]$ which has a dramatically different distribution from the trivalency model deployed for other datasets.





\smallskip
\noindent \textbf{Parameter Settings}. We randomly select $|S|$ (50 by default) nodes from the top 1\% nodes with the highest degrees in the original network as the seed nodes, set $k=20$ and the error ratio $\epsilon=10^{-4}$ by default. We evaluate solution quality based on the IC-based influence spread via 10,000 Monte Carlo simulations. 


\smallskip
\noindent \textit{\textbf{Exp1 - Case study on the two versions of baselines}}. Table~\ref{table:orgvsbst} and Table~\ref{table:orgvsbsttime} compare the effectiveness and efficiency with $k=30$ and $|S|=50$. We have four main observations:
%The main observation is that the boosted versions can achieve about five-order-of-magnitude larger influence than their original counterparts but can be still outperformed by \outtermethod{}. Specifically, \outtermethod{} outperforms the second best performer by at least 23\%-39\% on different datasets respectively. More observations are in Appendix~\ref{appendix:casestudy}. Due to the poor performance of the original baselines, we only use the boosted versions for comparison in the rest of experiments.  
%\subsection{Case study on two versions of baselines}\label{exp:casestudy}
%We have two observations in Table~\ref{table:orgvsbst}:
%(1) the performance gap between original versions of baselines and \outtermethod{} is much more greater than the one in Section 6.1 such that \outtermethod{} can achieve up to five-order-of-magnitude larger influence (e.g., on Orkut). This observation is mainly caused by the significant difference in the topological information of the input diffusion network and the size of edge insertions. Specifically, in Section 6.1, the diffusion network is the original network which contains rich topological information and the size of edge insertions is quite small. On the other hand, in this section, the original versions start from a diffusion network which initially only contains seed nodes and face considerable edge insertions which contribute all influence increment of seeds.
\vspace{-1mm}
\begin{enumerate}[leftmargin = *]
\item \method{Org-Random} is more effective than the original versions of other baselines. The reason is that nodes with high degrees will `attract' much more incoming edges in other strategies (i.e., \method{Org-Degree} and \method{Org-FoF}) which `waste' a lot of recommendation opportunities to repeatedly influence/activate these nodes. 
\item The boosted versions can achieve about five-orders-of-magnitude larger influence than their original counterpart but can still be notably outperformed by \outtermethod{}. Specifically, \outtermethod{} can still outperform the second best performer by at least 23\%-39\% on different datasets respectively, which demonstrates the effectiveness of both two stages (i.e., the expansion and filling stages). 
\item We also compute the constitution of the edges recommended by \outtermethod{} in the boosted baselines, and the result shows that \outtermethod{} only contributes 17\%-27\% of total edges in the diffusion network. The significant performance improvement of baselines with limited involvement of \outtermethod{} further demonstrates the effectiveness of \outtermethod{} in terms of identifying important edges and nodes for increasing the seeds' influence. 

\item \outtermethod{} is very competitive with other boosted baselines in terms of running time, because all methods involve the \emph{expansion} stage of \outtermethod{} (i.e., Lines 5-9 in Algorithm~\ref{alg:practicalframework}) which dominates the total computational cost. 
\end{enumerate}
\vspace{-1mm}

Due to the poor performance of the original baselines, we only use the boosted versions for comparison in the rest experiments.  



\smallskip
\noindent \textit{\textbf{Exp2 - Effectiveness comparison with different $|S|$}}. 
%\subsection{Effectiveness Comparison with Different $|S|$}\label{exp:|S|effectiveness}
Figure~\ref{fig:diffs} compares the performance with different $|S|$. Our method \outtermethod{} consistently outperforms other methods across all instances while the performance of other methods is not stable, e.g., \method{Bst-Random} outperforms \method{Bst-Degree} on Catster but the latter is more effective on Orkut. Another interesting observation is that the performance ranking of methods on the same dataset is consistent across different $|S|$. We think that a good edge recommendation for a non-seed user $u$ under an instance with a small $|S|$ can also be an effective recommendation for $u$ as the seed user under an instance with a great $|S|$. Thus, the diffusion networks generated by the expansion stage of \outtermethod{} under different $S$ can be similar such that edges chosen by a specific baseline upon these networks have large overlaps, which explains this observation and reflects the superiority of \outtermethod{}.


\smallskip
\noindent \textit{\textbf{Exp3 - Effectiveness comparison with different $k$}}. 
%\subsection{Effectiveness comparison with different $k$}\label{exp:keffectiveness}
Figure~\ref{fig:diffk} compares the performance at different $k$ across all datasets. We have four main observations: 
\vspace{-1mm}
\begin{enumerate}[leftmargin = *]
\item \outtermethod{} outperforms the boosted baselines and can achieve up to two-orders-of-magnitude larger influence (e.g., on Orkut). 
\item The performance gap becomes smaller when $k$ is larger. The reason is that all methods make almost the same recommendation strategy to low-degree nodes since their out-degrees are close to or even smaller than $k$. In this case, the number of combinations of $k$ outgoing edges of these nodes is very limited. This observation also explains why the performance gap is larger on datasets with greater average degrees. 
\item When $k$ is small (e.g., 10), all methods achieve similar influence since it is barely possible for any method to achieve large influence with very limited edges. 
\item The performance gap on MOBA and RPG is not as significant as that on other datasets. That is because the average edge weight on MOBA and RPG are notably larger. Thus, regardless of how the diffusion network is generated, seeds can easily influence many nodes with sufficient influence probabilities. 
\end{enumerate}
\vspace{-1mm}
      
Note that the performance difference may not be easily distinguished visually due to the log scale of y axis, but we have shown the notable performance difference with $k=20$ and $k=30$ in Figure~\ref{fig:diffs} and Table~\ref{table:orgvsbst} at a finer granularity already. 

\begin{figure}[t]
\includegraphics[width=0.4\textwidth]{./drawing2/legend2}
\vspace{-0.45cm}

\centering
\subfloat[varing $k$]{
\includegraphics[width=0.24\textwidth]{./drawing2/diffkiter_RMPP.pdf}\hspace{-1em}
} 
\hspace{0.5mm}
\subfloat[varing $|S|$]{
\includegraphics[width=0.24\textwidth]{./drawing2/difftiter_RMPP.pdf}\hspace{-1em}
}

\vspace{-1.em}
\caption{The number of iterations in the expansion stage with different $k$ and $|S|$.}\label{fig:convergence}
\vspace{-1.em}
\end{figure}


\begin{figure}[t]
%\includegraphics[width=0.4\textwidth]{./drawing2/legend2}
%\vspace{-0.45cm}

\centering
\subfloat[varing $k$]{
\includegraphics[width=0.24\textwidth]{./drawing2/diffktime_RMPP.pdf}\hspace{-1em}
} 
\hspace{0.5mm}
\subfloat[varing $|S|$]{
\includegraphics[width=0.24\textwidth]{./drawing2/diffttime_RMPP.pdf}\hspace{-1em}
}

\vspace{-1.em}
\caption{Running time of \outtermethod{} with different $k$ and $|S|$.}\label{fig:efficiency}
\end{figure}


\begin{figure}[t]
%\includegraphics[width=0.4\textwidth]{./drawing2/legend2}
%\vspace{-0.45cm}

\centering
\includegraphics[width=0.24\textwidth]{./drawing2/nodeparti_RMPP.pdf}\hspace{-1em}

\vspace{-1.5em}
\caption{The percentage of the nodes in the diffusion network over the one in the original network with different iterations in the expansion stage of \outtermethod{}, where the iterations with solid fill refer to the convergence points under different datasets repsectively.}\label{fig:noderatio}

\end{figure}


\begin{figure}[t]
\includegraphics[width=0.33\textwidth]{./drawing2/legend3}
%\vspace{-0.45cm}

\centering
\subfloat[RPG]{
\includegraphics[width=0.24\textwidth]{./drawing2/INEratio_RPG.pdf}\hspace{-1em}
} 
\hspace{0.5mm}
\subfloat[Orkut]{
\includegraphics[width=0.24\textwidth]{./drawing2/INEratio_Orkut.pdf}\hspace{-1em}
}

%\vspace{-1.em}
\caption{The influence ratio (I-Ratio), edge ratio (E-Ratio) and node ratio (N-Ratio) in the diffusion network produced by \outtermethod{} with different $k$.}\label{fig:INERatio} 

\end{figure}







\smallskip
\noindent \textit{\textbf{Exp4 - Impact of $k$ and $|S|$ on \outtermethod{} convergence}}. 
%\subsection{Impact of $k$ and $|S|$ on \outtermethod{} Convergence}\label{exp:convergence}
Figures~\ref{fig:convergence} (a) and (b) show the number of iterations in the expansion stage of \outtermethod{} when varing $k$ and $|S|$ respectively. Interestingly, when $k$ or $|S|$ increases, the number of iterations for convergence is non-increasing. This is because \outtermethod{} will include more nodes into the current \ksubnetwork{} in each iteration such that it may take fewer iterations to identify all important nodes for influence spread.


\smallskip
\noindent \textit{\textbf{Exp5 - Scalability study on \outtermethod{}}}. 
%\subsection{Scalability Study on \outtermethod{}}\label{exp:scalability}
Figures~\ref{fig:efficiency} (a) and (b) show the runtime of our (full-stage) \outtermethod{} when varing $k$ and $|S|$. As $k$ grows, more nodes tend to be included in the diffusion network and more edges tend to be `filled up' in the filling stage, hence costing more time. On the other hand, increasing $|S|$ does not notably incur more computation costs, for two reasons: 1) we transform the case of multiple seeds into the one of a single virtual node by introducing only $|S|$ extra edges into the diffusion network; 2) the size of the diffusion networks generated under instances of different $|S|$ can be similar as discussed earlier. It is obvious to see that \outtermethod{} is highly scalable and efficient, since it can produce good recommendation on datasets with millions of nodes and hundred millions of edges within two hours (e.g., Orkut). This performance is promising since such recommendation is usually deployed for a long-term usage.


\smallskip
\noindent \textit{\textbf{Exp6 - Impact of iterations on the diffusion network node size}}. 
%\subsection{Impact of iterations on the network size}\label{exp:interation}
Figure~\ref{fig:noderatio} shows how the node size of the diffusion network in the expansion stage of \outtermethod{} grows iteratively. Here, the iterations with solid fill refer to the convergence points. Note that the expansion stage is terminated after convergence for other experiments and here we force it to run 10 iterations. It is obvious that, the node size in the diffusion network converges as the influence spread, which indicates the effectiveness of the convergence criteria.
% in \outtermethod{} and its effectiveness in identifying important nodes for spreading influence. 

\smallskip
\noindent \textit{\textbf{Exp7 - Case study with large $k$}}. 
%\subsection{Case Study with Large $k$}\label{exp:largek}
Here, we conduct a case study on the two largest datasets, RPG and Orkut. Our goal is to show how the statistics of the diffusion network produced by \outtermethod{} and influence spread of seed nodes in this network will change when we further increase $k$ up to 50. Specifically, we use the \emph{influence ratio} (I-Ratio) to denote the percentage of the influence of seeds in the diffusion network over their full influence in the original network, \emph{edge ratio} (E-Ratio) and \emph{node ratio} (N-Ratio) to denote the percentage of the edge and node size of the diffusion network over the ones of the original network, respectively. As shown in Figure~\ref{fig:INERatio}, as $k$ increases, \outtermethod{} is able to achieve an I-Ratio of 90\% with only an E-Ratio of 36\%, and an I-Ratio of 94\% with only an E-Ratio of 46\% on RPG and Orkut respectively. These again demonstrate the superiority of \outtermethod{}. 
Furthermore, when the N-Ratio converges, the I-Ratio can still notably increase as $k$ grows, and even the converged N-Ratio can be notably smaller than 1 (e.g., on RPG). These indicate that \outtermethod{} can identify important nodes for spreading the influence. 


\iffalse
\smallskip
\noindent \textbf{More Experiments on open social networks}. We also conduct experiments on the problem of maximizing the seeds' influence in \emph{open} social networks. Specifically, this problem assumes \emph{all} friends to be recipients for further information propagation, and aims to insert a limited number of edges (i.e., constructing new friendships) into the network to maximize the seeds' influence. We compare our method \outtermethod{} with several baselines including the state-of-the-art~\cite{chaoji2012recommendations} with approximation guarantees. The results show that: 1) \outtermethod{} is able to effectively maximize the influence of multiple seed nodes while achieving five-orders-of-magnitude speedups than~\cite{chaoji2012recommendations}; 2) \outtermethod{} is robust to different edge insertion constraints for maximizing the seeds' influence. Please refer to our technical report~\cite{TR} for details.
\fi


\subsection{Deployment}\label{sec:deploy}
In order to demonstrate the practical effectiveness of our \short{} problem, we deployed our solution into an activity in a multi-player online battle arena game of Tencent of which the friendship network is MOBAX in Table~\ref{table:dataset}.

\smallskip
\noindent \textbf{Summary of the activity}.
Users join this activity by interacting (e.g., sending gifts and gaming invitation) with their friends recommended by the system and will obtain rewards via such interactions. This form of interaction could trigger domino effects such that the interactions can stimulate the message receiver to further interact with other users. The aim of this activity is to improve user retention and interactions. Note that, in this activity, we do not specifically designate seeds and every user could be a potential and spontaneous seed. Specifically, users who log in the game will see this activity and may perform three possible behaviors: (1) proactively start interactions as a seed, (2) start interactions as a message receiver (i.e., a non-seed) and (3) ignore this activity. 

\smallskip

{ \noindent \textbf{Edge weights and the diffusion model}. We adopt the same settings as we use for generating edge weights on MOBA and RPG, and generate the diffusion network based on the IC model. Note that the IC model is only used for generating the diffusion network but not used for evaluation since it is very likely that the real-world influence will not spread in a way specified by the IC model or any other classical diffusion models (e.g., Linear Threshold model~\cite{Kempe03}).}

\smallskip
\noindent \textbf{Methods for comparison}. Four methods, namely \method{Random}, \method{Degree}, \method{FoF} and \outtermethod{}, are deployed. For evaluation, we use an online A/B testing. Specifically, it randomly assigns each online user to one of these four methods which recommend a list of friends for each assigned user.
% and the graph induced by users assigned to \outtermethod{} forms the MOBA dataset in Table~\ref{table:dataset}. 
The list size $k$ is set as 20 for all methods because, in this application, only 20 friends are shown due to several reasons (e.g., the screen size and resolution settings of most mobile devices).
{Based on our observations made in Section~\ref{sec:exp-closed}, the k-subnetwork generated based on a given seed set could also be effective for different seed sets.
Thus, for \outtermethod{}, we first generate the \ksubnetwork{} with top 10\% of assigned users with the highest degrees as the seeds, and then use this generated \ksubnetwork{} for this activity where every user could be a potential seed or non-seed.}



\smallskip
\noindent \textbf{Experimental results}. {The number of users who interact with recommended friends directly indicates the quality of the underlying recommendation system and can effectively reflect the potential size of users who are impacted by others to performance interactions. 
Thus, we adopt the Click-through Rate (CTR) to evaluate the performance.} The CTR denotes the number of users who interacted with recommended friends divided by the total number of users who log in the game during this activity. %Since it is intractable to capture the influence spread in practice, CTR is a good alternative metric for evaluation in industry. 
The CTR achieved by \method{Random}, \method{Degree}, \method{FoF} and \outtermethod{} are 81.87\%, 82.73\%, 82.81\% and \textbf{88.14\%} respectively, which again demonstrates the effectiveness of \outtermethod{}. Despite that CTR is a very popular evaluation metric for recommendation systems in industry, there still exist some other evaluation metrics (e.g., the actual influence spread of seeds via knowing the propagation paths and who are the seeds) worthy of explorations. However, due to the privacy restriction of this activity, we have no access to the detailed information in user logs to compute the performance under other potential metrics. In future, we would like to see how our proposed method will perform in other activities under various evaluation metrics.




==> tex/experiment3.tex <==
\section{Experiments}


In this section, we will conduct extensive experiments on real-world datasets to evaluate the quality of \constraint{} pricing schemes produced by different methods according to the interests of stakeholders as shown in Figure~\ref{plan}. Specifically, we outline the following progressive questions to guide our evaluations, with the exact solution \fcexact{} under limited integer price choices as the reference:

\smallskip
Q1. Whether the pricing scheme is able to hire candidates with reasonable prices so as to maintain a good balance between conflict interests of the brand and influencers in the charges on the campaign plan?

\smallskip
Q2. Whether the pricing scheme is able to help the brand to achieve large advertising exposure?

\smallskip 
Q3. Whether the pricing scheme attracts considerable investments from the brand?

\smallskip
Q4. Whether the pricing scheme can be produced efficiently?

\smallskip
Q5. How far the performance of the pricing scheme is away from the converged \fcexact{} with increasingly sizes of price choices?

\smallskip
In Section 8.1, we will systematically analyze the interests of stakeholders and introduce the corresponding evaluation metrics. In Section 8.2, we will use the introduced metrics to evaluate different methods so as to answer the questions above. 

\subsection{Experimental Setup}


\begin{figure}[!t]

\centering

\subfloat[LastFm]{
\includegraphics[width=0.2355\textwidth]{./distributions/Lastfm.pdf}
}
\subfloat[Orkut]{
\includegraphics[width=0.24\textwidth]{./distributions/Orkut.pdf}
}
\vspace{-0.36cm}
\caption{Degree distributions and influencer categorization.}\label{distributions}

\end{figure}

\noindent \textbf{Datasets}. We collect four public undirected real-world datasets~\cite{konect} for experiments whose statistics are shown in Table~\ref{dataset}. Due to consistent observations on the experimental results across datasets, we only report experiments on LastFM and Orkut with drastically different scales where we can better compare the scalability of different methods. Furthermore, the expensive \fcexact{} is able to produce most of the results on these two datasets within our time limit (i.e., 60 hours) such that we can more comprehensively compare methods' performance.

{
\color{red} \noindent \textbf{Influencer categorization}. To test the robustness of our methods to candidate sets with different degree distributions, we coarsely divide influencers into three classes, Macro, Micro and Nano, with the naming convention in this domain~\cite{category}. Specifically, we order online users in non-increasing order of their degrees and group influencers based on this order into the same tier (i.e., Macro, Micro or Nano influencer) if their total degrees constitute 20\% of the total degrees in the social network, as shown in Figure~\ref{distributions}. 

}



\input{tex/datasets.tex}
\smallskip
\noindent \textbf{Methods for comparison}. In this experiments, we use the following methods for comparison.

\begin{enumerate}
 \item  \textbf{\bcexact{}}. The binary-choice based dynamic programming (i.e., Algorithm~\ref{BC-DP}) which produces the minimum divergence score when we can either hire each influencer $v$ with the price equal to her influence (i.e., $p_v=\delta(v)$) or do not hire her (i.e., $p_v=0$).
 
 \item \textbf{\bcmg{}}. The binary-choice and minimum gain based algorithm (i.e., Algorithm~\ref{BC-Greedy}) which approximates the optimal divergence score by computing the complement set of the solution set through iteratively choosing influencers with the minimum gain of $f()$ score per unit price. 
  
  \item \textbf{\fcexact{}}. The flexible-choice based exact algorithm (i.e., Algorithm~\ref{FC-DP}) which is able to find the optimal solution when each influence $v$ is assigned with an integer price choice set $R_v$ which consists of her influence plus a number $num$ of integer prices evenly dividing the continuous range $[0.5*\delta(v), 1.5*\delta(v)]$ in a coarse-grained level. That is, $R_v$ consists of integers which are floors of floats in the set $\{\delta(v)(0.5+1/num), \delta(v)(0.5+2/num),..., \delta(v),..., 1.5\delta(v)   \}$ where $|R_v|$ is set as 10 by default.
  
 \item \textbf{\fcinf{}}. The flexible-choice and influence based greedy algorithm (i.e., Algorithm~\ref{FCInf-Greedy}) which iteratively satisfies the profit expectation of the influencer with the greatest influence given a continuous range of price choices for hiring each influencer. In experiments, we set the range as between zero and the input budget.
 
 \item \textbf{\fcmws{}}. The flexible-choice and maximum-weighted subsequence based algorithm (i.e., Algorithm~\ref{FCMWS-Greedy}) which first finds the subsequence of influencers whose profit expectation can be exactly satisfied with the greatest total $f()$ scores among all qualified subsequences, and then adjusts the remaining influencers' prices and greedily choose them based on their gains of $f()$ scores per unit price. 

 
\end{enumerate}




\smallskip
\noindent \textbf{Parameter settings}. We describe the settings of parameters needed for modeling the fundamental procedure involving all stakeholders in the influencer marketing as shown in Figure~\ref{model}, and they are the maximum investment budget from the brand, the candidate set recommended from the agency and profit expectations of candidate influencers:

\begin{enumerate}
\item \textbf{The investment budget}. The brand offers the maximum budget $B$ it can invest to the agency. The agency then will look for suitable candidature influencers who have high alignments with the brand's product to be promoted, and whose total influence should match with the budget considering the standard price rate (price per follow) in this market~\cite{pricerate}. For simplicity, we assume the standard price rate to be one since it does not impact our judgment on the performance of each method.

 
 \item \textbf{The candidate influencers}. Here we assume that the candidate set has been found since this process is orthogonal to our study. Considering the charges on contracted influencers for agent commission (usually 20\%~\cite{commission}) and that it may not be possible to find suitable candidates perfectly matched with the budget, we create the candidate set $\candidates{}$ by randomly selecting a number of candidates ($|\candidates{}|=90$ by default) from the aforementioned three tiers of influencers (i.e., Macro, Micro and Nano), and set $B$ as 80\% of the total influence of candidates. To show the robustness of our methods to combinations of influencers of different tiers, we create the candidate set with the following different sampling distributions: \{Macro:0.5, Micro:0.25, Nano:0.25\}, \{Macro:0.25, Micro:0.5, Nano:0.25\}, \{Macro:0.25, Micro:0.25, Nano:0.5\} and \{Macro:0.33, Micro:0.33, Nano:0.33\}. For simplicity, we call these four sampling distributions as Macro-focused, Micro-focused, Nano-focused and Uniform sampling distributions respectively. Due to space limit, we only report results under Micro-focused and Uniform sampling distributions, and we have similar observations on the rest.

\item \textbf{Profit Expectation}. Since each candidate influencer $v$ values her own influence differently in reality based on the detail of the campaign contract and personal factors (e.g., exclusive collaboration with this brand, likeness towards the product to be promoted, choices of media channels, etc.)~\cite{pricing,factorreport}, we use the weighted influence sampled from 
 $[\delta(v), 1.5\delta(v)]$ to include these realistic factors. The profit expectation or expected profit sharing of each influencer controlled by the agency is a weighted-influence related percentage over the budget and we compute this percentage as the weighted influence of the influencer over the total one of all candidates.
\end{enumerate}


\smallskip
\noindent \textbf{Interests-oriented evaluation metrics}. We evaluate the performance of different methods by considering the interests of different stakeholders corresponding to Figure~\ref{plan}: 
\begin{enumerate}
\item From the perspective of the brand, the campaign plan should be \constraint{}. Otherwise, the brand will not fully accept the plan or even reject the it. Furthermore, the \constraint{} campaign plan should be budget-friendly and able to achieve large advertising exposure. In terms of the cost of the plan, the agency cannot make the charges on influencers as low as possible to satisfy the brand which will harm influencers' interests. Even though the information of influencers' expectations is not public to the brand, to protect the brand's benefits, the plan should try to  
make sure that the actual charges of influencers match with rather than larger than their controlled expectations, which is measured by the overall profit divergence score. In terms of advertising exposure, the brand expects the plan to be influential which is measured by the total influence of influencers involved in the campaign plan.

\item From the perspective of candidates, the campaign plan should be able to bring them significant profits. Due to the conflicts of interests between the brand and candidates, blindly increasing influencers' prices will compromise the brand's interests. To protect the benefits of both influencers and the brand, the plan should try to make sure that the actual profits match with rather than smaller than the controlled expectations from influencers, which can be also measured by the overall profit divergence score.

\iffalse
to satisfy their profit expectations which is quantified based on the total profit divergence $\divergence{}$. Directly comparing divergence scores of different methods without any reference is not informative since the divergence score can vary significantly across different settings and datasets and it is hard to know whether the performance difference is significant or not. To control the measured performance in the same scale, we use $\divergence{}/B$ as the evaluation metric considering that the maximum possible divergence score cannot be greater than the input budget $B$, and this metric could give better indication on how far the performance of each method is away from the worst possible case. 
\fi

\item From the perspective of the agency, a good \constraint{} campaign plan should be able to attract large investments from the brand besides protecting benefits of the brand and influencers. Large investment will not only bring the agency considerable profit on agent commission and campaign management, but also be beneficial to involving more contracted influencers and satisfying their profit expectations. The level of investment is measured by how much budget is spent by the campaign plan. 

\end{enumerate}



To summarize, we compare effectiveness of different methods based on three metrics, namely the overall divergence score, the total influence of hired candidates and the invested budget. The importance of these three metrics is ranked as the same order as the aforementioned one since protecting of benefits and improving the satisfaction of involved candiates and the brand is the first priority of the agency. Due to the timeliness of marketing, efficiency also plays a critical role in ensuring success of the business and thus a method which is very effective but incurs exorbitantly computational time is not acceptable.





\smallskip
\noindent \textbf{Environments}. We conduct all experiments on a Linux server with Intel Xeon E5 (2.60 GHz) CPUs and 512 GB RAM. All codes are implemented in Python and any method which cannot finish within 60 hours will be terminated. 

\subsection{Experimental Results}
In this section, we will evaluate the extent to which different methods protect benefits and improve satisfaction of different stakeholders under four evaluation metrics (i.e., divergence score, influence of involved influencers, the invested budget and efficiency). Furthermore, we will conduct ablation study on the impact of the size of price choices on \fcexact{} to demonstrate the effectiveness of \fcexact{} and \fcmws{}.

\input{tex/smalldataset}

\smallskip
\noindent \textbf{Profit divergence comparison}. One simple way for this evaluation is to directly comparing divergence scores $\divergence{}$ of different methods. However, this straightfoward way lacks of references and is not informative since the divergence score can vary significantly across different settings and datasets and it is hard to know whether the performance difference among methods is significant or not. To control the measured performance in the same scale, we use $\divergence{}/B$ as the evaluation metric considering that the maximum possible divergence score cannot be greater than the input budget $B$, and this metric could give better indication on how far the performance of each method is away from the worst possible case.

Figure~\ref{effect:divergence} compares the divergence scores on LastFM and Orkut with different sampling distributions and candidate sizes. Note that different candidate sets on the same dataset correspond to independent cases and thus the optimal $\divergence{}/B$ under different candidate sets can vary notably. \bcmg{} shows very competitive performance compared with \bcexact{} which demonstrates the empirical effectiveness of \bcmg{} which is much better than what its worst-case approximation ratio indicates. However, both of them are notably outperformed by flexible-choices based methods. With \fcinf{} as the reference, the performance of \fcexact{} is generally better under the even-focused sampling distribution than in the micro-focused one. We suspect that \fcexact{} is able to find better pricing scheme from the limited price choices when the degree distribution of candidates is sparser. When candidates have similar degrees, \fcexact{} requires more fine-grained and similar price choices to achieve lower divergence. As for other methods, we do not see any clear impact of sampling distributions on the performance. On the other hand, \fcmws{} significantly outperforms all other methods in all cases, which demonstrates its effectiveness of protecting stakeholders' benefits. 

\input{tex/influence}

\smallskip
\noindent \textbf{Influence comparison}. To better show the influence of campaign plans, we show the influence ratio of the total influence of involved influencers over the optimal influence in the case where we aim to maximize the influence instead of minimizing profit divergence when the price of each influencer $v$ is decided by the standard price rate (i.e., $p_v=\delta(v)$). Such case simulates the brand's estimation on the \emph{ideal} advertising exposure effect based on the public information. To compute the optimal influence in this case, we just need to set the $f()$ score of each influencer equal to the her influence in \bcexact{}. Figure~\ref{effect:influenceratio} shows the influence ratios achieved by different methods. It is interesting to see that \bcexact{} and \bcmg{} with the profit minimization objective achieve very competitive influence compared with \bcexact{} with the influence maxization objective. Furthermore, the performance ranking of \bcexact{} and \bcmg{} under this metric can be indicated from the one under the profit divergence score. For example, when \bcexact{} achieves lower divergence score than \bcmg{} in Figure~\ref{effect:divergence} (c) with $|\candidates{}|=30$, it also achieves greater influence under the same setting. These observations indicate the positive correlations between profit divergence minimization and influence maximization given the same pricing scheme.

On the other hand, flexible-choice based methods are able to achieve better influence ratios since they have greater space for price adjustment and thus hire more candidates. While maintaining very competitive divergence scores, \fcexact{} tends to hire more candidates than \fcinf{} considering its notably greater influencer ratios and the strategy of \fcinf{} which prioritizes hiring influencers with the greatest influence  (e.g., comparing Figure~\ref{effect:divergence} (a) and Figure~\ref{effect:influenceratio} (a) with $|\candidates{}|=30$). It indicates the drawback of \fcinf{} which overly satisfies influencers to a large extent and quickly exhausts the budget, and the effectiveness of \fcexact{} which makes the best strategy given limited integer price choices. Among all methods, \fcmws{} achieves the greatest influence ratios in most cases while maintaining the lowest divergence scores. These observations indicate that protecting benefits of influencers does not necessarily compromise the brand's interest.

\input{tex/investment}
\smallskip
\noindent \textbf{Attracted investment comparison}. Figure~\ref{effect:investment} shows the ratios of the invested budget for hiring candidates over the maximum budget $B$ the brand offers. As mentioned earlier, the invested budget ratio is the least important effectiveness evaluation metric to the agency since protecting benefits of the brand and influencers is the first priority. Even though methods such as \bcexact{} and \fcinf{} slightly outperform \fcmws{} in many cases under this metric, they attract the investment in a way that sacrifices the benefits of the brand or influencers as shown in Figure~\ref{effect:divergence} and Figure~\ref{effect:influenceratio}. Thus, the agency should make comparison between different methods under this metric only when these methods are very competitive in previous evaluation. 


\input{tex/runtime}
\smallskip
\noindent \textbf{Efficiency comparison}. Figure~\ref{effect:efficiency} compares the running time of different methods. \bcmg{} achieves the lowest running time due to its simple strategy and is up to two-orders-of-magnitude faster than \bcexact{}. \fcinf{} and \fcmws{} are ranked as second and third. Despite the notable difference between their time complexity (i.e., $O(|\candidates{}|\log(|\candidates{}|))$ and $O(|\candidates{}|\log(|\candidates{}|) +|\candidates{}|^2)$ ), \fcmws{} is very competitive with \fcinf{} practically since candidate set sizes are usually small. On the other hand, \fcexact{} can be up to six-orders-of-magnitude slower than \bcmg{}, \fcinf{} and \fcmws{}, which is not feasible in real-world scenarios despite its competitive performance compared with many methods.


\input{tex/piece}

\begin{table}[]
\caption{Running time with different $|R|$ on LastFM}~\label{piecetime:lastfm}
\vspace*{-.5em}
\begin{tabular}{cccccc}
\hline
\multirow{2}{*}{Dataset} & \multicolumn{5}{c}{$|R|$} \\ \cline{2-6} 
 & 10 & 20 & 30 & 40 & 50 \\ \hline
Uniform & 1.4E+3 & 3.7E+3 & 5.3E+3 & 5.9E+3 & 6.5E+3 \\
Micro-focused & 1.4E+3 & 3.9E+3 & 5.3E+3 & 6.0E+3 & 6.2E+3 \\ \hline
\end{tabular}
\end{table}

\begin{table}[]
\caption{Running time with different $|R|$ on Orkut}~\label{piecetime:orkut}
\vspace*{-.5em}
\begin{tabular}{cccccc}
\hline
\multirow{2}{*}{Dataset} & \multicolumn{5}{c}{$|R|$} \\ \cline{2-6} 
 & 10 & 20 & 30 & 40 & 50 \\ \hline
Uniform & 9.1E+3 & 3.3E+4 & 6.9E+4 & 1.2E+5 & 1.9E+5 \\
Micro-focused & 8.9E+3 & 3.1E+4 & 6.7E+4 & 1.3E+5 & 1.9E+5 \\ \hline
\end{tabular}
\end{table}


\smallskip
\noindent \textbf{Ablation study on $|R|$ in \fcexact{}}. In order to see the performance limit of \fcexact{} and further demonstrate the effectiveness of \fcmws{}, we gradually increase the size of $R$ for each influencer in \fcexact{}. Figure~\ref{effect:piece} shows the performance of \fcexact{} with different sizes of $R$, where \fcinf Int refers to the version of \fcinf{} allowing integer price choices only. As $|R|$ increases, the performance of \fcexact{} notably increases and converges to a stable state on LaftFM but fails to converge on Orkut within the our time limit (i.e., 60 hours). 
An interesting observation is that, even though \fcexact{} significantly outperforms all methods, it is still outperformed by \fcmws{}. We suspect that it is mainly caused by the fact that \fcexact{} can only work with integer price choices, as evidenced by the notable performance difference between \fcinf{} and \fcinf Int which may even be outperformed by binary-choice based methods. As we can see from Table~\ref{piecetime:lastfm} and Table~\ref{piecetime:orkut}, the running time of \fcexact{} increases drastically as $|R|$ and can be up to eight-orders-of-magnitude slower than other flexible-choice based methods (e.g., comparing with $|\candidates{}|=90$ in Figure~\ref{effect:efficiency}(c) with $|R|=50$), which makes it infeasible to cater for real-world scenarios.














==> tex/hardness.tex <==
\section{Hardness Analysis}

\begin{figure}[!t]

\centering
\includegraphics[width=0.4\textwidth]{./figures/tree}\hspace{-1em}
%\vspace{-1em}
\caption{An example of a graph constructed based on a set cover instance.} 
\label{fig:tree}
\vspace{-1em}
\end{figure}

In this section, we will show that the \short{} problem is NP-hard via a reduction from the set cover problem defined as below.


\begin{definition}[Set Cover]
Given a set $U$ of elements, a collection $C$ of subsets $A_1,A_2,...,A_{|C|}$ of $U$ where $\cup_{A\in C} =U$, we aim to choose the smallest number of sets from $C$ such that their union is $U$.
\end{definition}


\begin{theorem}
The \short{} is NP-hard.
\end{theorem}

\begin{proof}
To show that \short{} is NP-hard, we will perform reduction from the NP-complete decision problem of set cover, which checks whether we can find $k$ sets from $C$ whose union is $U$, to the special case of \short{} where there is only a single seed user $s$.

Given the collection $C$ of a set cover instance, we construct a deterministic graph with a tree structure where the weight of each edge is 1 as below. First, we find the set $A_{max}$ with the greatest size from $C$ and create a tree with elements in $A_{max}$ as the bottom nodes (at the bottom level). In the second last level, we introduce the set $V'$ of $\lceil |A_{max}|/k  \rceil$ virtual nodes. We next create directed edges from each of virtual node to at most two arbitrary nodes in $A_{max}$ which have not been connected by virtual nodes in $V'$. Afterwards, we create the last third layer based on the last second one by adopting the similar rules. We repeat this step until the root node is constructed. We also create trees for the rest of sets in $C$ similarly. One difference is that, when we create the tree for a set $A$, we need to make sure that the number of virtual nodes in each level is consistent with the corresponding level of the tree constructed based on $A_{max}$. It means that some virtual nodes may not have outgoing neighbors. After we create trees for all sets in $C$, we introduce directed edges from $s$ to all root nodes. 
\begin{example}
Figure~\ref{fig:tree} shows the graph constructed from the set cover instance where $k=2$ and $C=\{ \{a,b,c,d,e\},\{d,e,f\}, \allowbreak \{f,g,h\} \}$. Dash nodes refer to virtual nodes and virtual nodes with the same number come from the tree constructed based on the same set from $C$. Since $A_{max}=\{a,b,c,d,e\}$, the number of virtual nodes in the second last level of all trees are $\lceil |A_{max}|/k  \rceil =3$. 

%In this instance, the challenge of solving the \short{} problem lies in choosing two out of three outgoing edges from $s$, and the optimal solution is to pick edges $(s,1)$ and $(s,3)$.
\end{example}
Since the time cost for creating such a tree is at most $O(|A_{max}| \allowbreak \log_k|A_{max}|  )$, the total reduction process is polynomial in the total size of sets in the collection. To solve the \short{} problem in the constructed graph, we just need to focus on selecting $k$ outgoing edges for the root node $s$ since the out-degree of the rest of nodes in the graph is at most $k$ and edges not incident on $s$ can be all chosen. Considering that the trees constructed from each set in $C$ have the same number of virtual nodes, the quality of outgoing edge selection for $s$ only depends on bottom nodes being reached.  Thus, selecting $k$ outgoing edges for $s$ corresponds to selecting $k$ sets from $C$. Suppose the number of virtual nodes in each tree is $x$. If the optimal influence spread is $k\times x +1+|U|$ (including $s$) which is also the maximum possible influence, we have a `yes' answer to the set cover instance. Otherwise, the answer is `No'.\end{proof}

==> tex/multiplebudget.tex <==

\section{PDMFP with multiple campaigns}
In this section, we will discuss our problem in the case there are multiple campaigns implying multiple budgets and each influencer can be assigned to at most one marketing campaign. This problem cater for the scenario where each influencer exclusively collaborate with one brand among all competitors or the influencer only have high alignment with a specific brand. Note that, without the assignment constraint, this problem becomes equivalent to our problem under single budget. Next we will theoretically analyze the hardness of this problem and then outline some directions for solutions. We use $\mathcal{B}$ to denote a set of campaign budgets $\{B_1,B_2,...,B_{|\mathcal{B}|} \}$ and $\scheme{}_{\mathcal{B},\candidates{}} (v,B )$ to denote the hired price of $v$ set by the pricing scheme $\scheme{}_{\mathcal{B},\candidates{}} $ in a campaign with budget $B$. For ease of presentation, we assume that each campaign has an unique budget.

\begin{definition}[\short{} with multiple campaigns]
Given a set $\mathcal{B}$ of campaign budgets, a set $\candidates{}$ of candidates with their profit expectation ( $\sum_{v \in \candidates{}} p^*_v= \sum_{B \in \mathcal{B}}B $) and influence, we aim to propose an optimal \constraint{} pricing scheme $\scheme{}^*_{\mathcal{B},\candidates{}}$ such that the overall profit divergence is minimized, e.g.,
\begin{equation}
\begin{aligned}
&\scheme{}^*_{\mathcal{B},I}=\argmin_{\scheme{}_{\mathcal{B},\candidates{}} \in \mathcal{S}  }  \sum_{v\in I}  | \sum_{B \in \mathcal{B}} \scheme{}_{\mathcal{B},I} (v,B)- p^*_{v} |\\
\text{subject to (1)} \; & \forall B \in \mathcal{B}, \sum_{v\in \candidates{}}\scheme{}_{\mathcal{B},\candidates{}} (v,B) \leq B, \\
\text{(2)} \; & \forall v \in \candidates{}, \text{if } \sum_{B \in \mathcal{B}} \scheme{}_{\mathcal{B},\candidates{}} (v,B)>0, \exists B' \in \mathcal{B},\\ &\scheme{}_{\mathcal{B},\candidates{}} (v,B')=\sum_{B \in \mathcal{B}} \scheme{}_{\mathcal{B},\candidates{}} (v,B),
\end{aligned} 
\end{equation}

\noindent where the second constraint ensures that any influencer will be assigned to at most one campaign.
\end{definition}


\begin{definition}[Simple case with binary choices]\label{mbbc}
 Given a set $\mathcal{B}$ of campaign budgets, a set $\candidates{}$ of candidates with their profit expectation and influence where each influencer $v$ is assigned with a hired price $p_v=\delta(v)$ and a profit expectation $p^*_v$ ( $\sum_{v \in \candidates{}} p^*_v=\sum_{k=1}^{|\mathcal{B}|} B_k $), we aim to hire some influencers from $\candidates{}$ to join different campaigns under their specific budgets such that the divergence score is minimized:
 
 \begin{equation}\label{mbsimple}
 \begin{aligned}
  \text{minimize} \: & \sum_{B \in \mathcal{B}} B - \sum_{v \in \candidates{}} \sum_{B \in \mathcal{B}} x_{v, B} *f(v,p_{v})  ,\\
  \text{where}  \; & \text{(1)} \:  f(v,p_{v}) = \left \{ \begin{aligned}
       & p_{v},  \;\;  \text{if } p^*_{v} > p_{v}\\
       &2p^*_{v} -p_{v}, \;\; \text{if } p^*_{v}\leq p_{v}\\   
     \end{aligned}\right. \\
        & \text{(2)} \: x_{v,B} =0 \; \text{or} \; 1, \\
        & \text{(3)} \: \sum_{v \in \candidates{}}  x_{v,B} \cdot p_{v} \leq B.   
    \end{aligned} 
 \end{equation}
 
 \end{definition}

Next, we will show that our problem under multiple campaigns is NP-hard and NP-hard to approximate via reduction from 3-partition problem. 

\begin{definition}[3-partition problem~\cite{garey1979computers}]
Given a set $\mathcal{A}$ of elements $\{a_1,a_2,...,a_{3m}\}$ and a positive integer $B'$, and a positive size $s(a_i)$ for each $a_i \in \mathcal{A}$ where $s(a_i)$ satisfies $B'/4<s(a_i)<B'/2$ and $\sum_{i=1}^{3m} s(a_i)=mB'$, can $\mathcal{A}$ be partitioned into $m$ disjoint sets $A_1,A_2,...,A_m$ so that for $1\leq j \leq m$, $\sum_{a\in A_j} s(a)=B'$?
\end{definition}


\begin{theorem}
The \short{} with multiple budgets is NP-hard and NP-hard to approximate within any constant factor.
\end{theorem}

\begin{proof}
We prove hardness for the simple case with binary price choices (i.e., Definition~\ref{mbbc}) by using reduction from 3-Partition.

Given any instance of 3-Partition problem, we construct the corresponding instance on our problem as follows. First, we construct the influencer set $\candidates{}=\{v_1,v_2,...,v_{3m}\}$ where the profit expectation and the hired price of the $i$-th candidate are both equal to $s(a_j)$ where $1\leq j \leq 3m$. Next, we construct $m$ budgets $B_1,B_2,...,B_m$ all of which are equal to $B'$. The reduction is achieved in polynomial time since the sizes of influencer set and budgets are bounded by $m$. We next show that if our problem can be solved
in polynomial time, so can 3-PARTITION, implying hardness. Specifically, we claim that any instance of 3-Partition problem is a YES-instance if and only if the divergence score (i.e., Formula~\ref{mbsimple}) in the corresponding instance of our problem is 0.

\noindent ($\Longrightarrow$): Suppose $A_1,A_2,...,A_m$ are disjoint 3-element subsets of $\mathcal{A}$ that each sum to $B'$. For elements in the same subset $A_j \:(1 \leq j\leq m)$, we assign the corresponding influencers into the same campaign with budget $B_j$. This assignment clearly leads to 0 divergence score.

\noindent ($\Longleftarrow$): If the divergence score is 0 in the instance of our problem, all influencers have been hired to join marketing campaigns. Otherwise, the divergence score cannot be 0 based on Formula~\ref{mbsimple}. It also means that the budgets of all campaigns have been fully used, otherwise the divergence score cannot be 0.
Since the $f()$ score of each influencer $v$ is equal to her profit expectation $p^*_v$ which satisfies that $B'/4<s(a_i)<B'/2$ and the budget of each campaign is equal to $B'$, each campaign involves exactly three influencers. For influencers in campaign with budget $B_j \:(1 \leq j\leq m)$, we assign the corresponding elements into the same subset $A_j$. This assignment naturally leads to a YES-instance of the 3-Partition problem. 

We just proved that our problem is NP-hard. To
see hardness of approximation, suppose $\mathcal{Q}$ is an algorithm that approximates
our problem within a factor of $\alpha$. That is,
the divergence score achieved by algorithm $\mathcal{Q}$ on any instance of our problem
is not greater than $\alpha \cdot OPT$, where $OPT$ is the optimal (least) divergence score. Using the same reduction as above, we can see that the optimal divergence score on the reduced instance above is 0. On this instance,
the regret achieved by algorithm $\mathcal{Q}$ is $ \leq \alpha \cdot OPT=0$, which means that algorithm $\mathcal{Q}$ can solve our problem optimally in polynomial time. It is shown above to be impossible unless P = NP.

\end{proof}


\noindent \emph{Solutions on \short{} with multiple campaigns}. The main challenge on our problem with multiple campaigns mainly lies in the assignments of influencers to different campaigns, which is very different from our main problem with a single campaign which focus on pricing influencers. To solve \short{} with multiple campaigns, we can use our proposed methods to price influencers first followed by adopting existing algorithms~\cite{khuri1994zero,chekuri2005polynomial,martello1980solution} on the multiple knapsacks problem for assignment which is a well-studied classical problem. 


\iffalse
\subsection{NP-hardness of problem 2}
 We first formulate two constrained multiple knapsack problems MKPV and MKPVC and prove their NP-hardness. Next, we prove the NP-hardness of problem 1 via reduction flow: MKP to MKPV, MKPV to MKPVC, MKPVC to our problem.

\smallskip
\noindent \textbf{Multiple Knapsack problem (MKP)}. Given a sequence of $i$ items each of which is assigned with non-negative weight $w_h$ and a value $z_h$ $(1 \leq h\leq i)$, and $j$ bags each of which is associated with capacity $\bar{B}_k \; (1 \leq k\leq j)$, we aim to select $j$ disjoint subsets of items so that the total profit of selected items is maximized and each subset can be assigned to a different knapsack whose capacity is no less than the total weight of items in this subset. Formally,

\begin{equation}
\text{maximize} \sum_{h=1}^i \sum_{k=1}^j p_{hk}*z_h
\end{equation}

\noindent subject to the following five constraints:
\begin{enumerate}
\item $\forall h \;(1 \leq h \leq i) \: \text{and} \: k \; (1 \leq h \leq j), p_{hk}=0$ or 1.
\item $\forall h \;(1 \leq h \leq i),  \sum_{k=1}^{j} p_{hk} \leq 1 $.

\item $\forall k \; (1 \leq k\leq j), \sum_{h=1}^{i} p_{hk}\cdot w_h \leq B_k  $.

\end{enumerate}

 \smallskip


\noindent \textbf{Multiple Knapsack problem with value constraints (MKPV)}. Given a sequence of $i$ items each of which is assigned with non-negative weight $w_h$ and a value $z_h$ $(1 \leq h\leq i)$ \emph{smaller than its weight} $(z_h \leq w_h)$, and $j$ bags each of which is associated with capacity $\bar{B}_k \; (1 \leq k\leq j)$, we aim to select $j$ disjoint subsets of items so that the total profit of selected items is maximized and each subset can be assigned to a different knapsack whose capacity is no less than the total weight of items in this subset.

\smallskip

\noindent \textbf{Multiple Knapsack problem with value and budget constraints (MKPVC)}. Given a sequence of $i$ items each of which is assigned with non-negative weight $w_h$ and a value $z_h$ $(1 \leq h\leq i)$ \emph{smaller than its weight} $(z_h \leq w_h)$, and $j$ bags each of which is associated with capacity $\bar{B}_k \; (1 \leq k\leq j)$ such that $\sum_{k=1}^j \bar{B_k} = (\sum_{h=1}^i w_h+z_h)/2$, we aim to select $j$ disjoint subsets of items so that the total profit of selected items is maximized and each subset can be assigned to a different knapsack whose capacity is no less than the total weight of items in this subset.

\smallskip


\begin{lemma}
MKPV is NP-hard.
\end{lemma}
\begin{proof}
To reduce MKP to MKPV, we can multiple all item weights and budgets by a suitable parameter to satisfy the value constraint without effecting the solution, just like we did in Lemma 1.
\end{proof}

\begin{lemma}
MKPVC is NP-hard.
\end{lemma}
\begin{proof}
To reduce MKPV to MKPVC, we can satisfy the budget constraint by introducing a `super useless' or `super useful' item just like we did in Lemma 2. There is one difference. In Lemma 2, we update the capacity when we introducing a `super useful' item. Here, in this reduction from MPKV to MPKVC, we introduce an extra bag with capacity equal to the weight of the `super useful' item.
\end{proof}

\begin{theorem}
Problem 2 is NP-hard to be solved.
\end{theorem}

\begin{proof}
We reduce MKPVC to the special case of problem 1 by mapping $q_{v_h}=(w_h+z_h)/2$, $B_k= \bar{B}_k$ $(1 \leq k \leq j)$, and $c_{v_h}^*=w_h$. Based on this mapping and value and capacity constraint in MKPVC, we have $q_{v_h} \leq c_{v_h}^*$ and $\sum_{h=1}^i q_h= \sum_{k=1}^j B_k$. Based on Equation 7 and 8, the objective is:
$$\text{maximize} \sum_{h=1}^i \sum_{k=1}^j p_{hk} (2q_{v_h}-c_{v_h}^* ) = \sum_{h=1}^i \sum_{k=1}^j p_{hk} \cdot z_h,$$

\noindent which is the same as the objective of MKPVC. The solution of the special case of problem 2 must be the solution of MKPVC and vice versa. Since the reduction is in polynomial time, problem 2 is NP-hard.

\end{proof}


\begin{theorem}
The special case of problem 2 is equivalent to MKP problem.
\end{theorem}

\begin{proof}
We omit the proof since it is rather straightfoward based on similar reduction in Theorem 5.
\end{proof}
\subsection{Non polynomial approximation of problem 2}
First we introduce 3-partition problem which is strongly NP-complete and show that our problem can be reduced from 3-partition problem. Next, we will show the non-approximation of our problem by considering the optimal value of Equation 11 is 0.

\noindent \textbf{3-partition problem~\cite{garey1979computers}}. Given a set $A'$ of elements $A'=\{a_1,a_2,...,a_{3m}\}$ and a positive integer $B'$, and a positive size $s(a_i)$ for each $a_i \in A'$ where $s(a_i)$ satisfies $B'/4<s(a_i)<B'/2$ and $\sum_{i=1}^{3m} s(a_i)=mB'$, can $A'$ be partitioned into $m$ disjoint sets $A'_1,A'_2,...,A'_m$ so that for $1\leq j \leq m$, $\sum_{a\in A'_j} s(a)=B'$?

\begin{lemma}
The special case of problem 2 can be reduced from 3-partition problem.
\end{lemma}
\begin{proof}
Since MKP problem can be reduced from 3-partition problem~\cite{geng1986complexity} and the special case of problem 2 is equivalent to MKP problem, the special case of problem 2 can be reduced from 3-partition problem.
\end{proof}

\begin{theorem}
The special case of problem 2 is NP-hard to approximate in polynomial time. 
\end{theorem}

\begin{proof}
We can reduced a 3-partition instance to the special case of problem 2, by mapping $A=A'$, $m$ budgets $B_1=B_2=...=B_m=B'$, and $c_{v_h}^*=q_{v_h}=s(a_h)$ $(1\leq h \leq 3m)$. 
%Based on the definition and NP-completeness of 3-partition problem, it can be NP-hard to find the optimal allocation strategy even when the optimal value of Equation 11 is 0. 

Suppose we have an approximate algorithm $\mathcal{A}$ that approximates Equation 11 within a factor of $\alpha$. Using the same reduction above, we can see the optimal value on this instance of Equation 11 can be 0. On this instance, the value achieved by algorithm $\mathcal{A}$  is $\leq \alpha \cdot 0=0$, which means that algorithm $\mathcal{A}$ can solve the special case of problem 2 optimally in polynomial time. This is not possible unless $P=NP$.

\end{proof}
\fi

==> tex/response.tex <==
\twocolumn
\begin{center}
	\noindent\textbf{Response to Reviewer Comments}
\end{center}

We would like to express our sincere gratitude to the meta-reviewer and the three reviewers who take considerable time to review and comment our paper and acknowledge the technical depth and quality of content of our work. Their constructive comments, suggestions, and advises are all much appreciated. After addressing all the comments, the paper presentation is greatly improved with more descriptions and details (e.g., discussion between closed and open social networks, direction applications of the problem, method introduction, and deployment).


\subsection*{Revision Summary}

Below is a summary of the major revisions that we have made in
the paper. All major revisions have been highlighted using {\color{blue} blue color} in this manuscript.

\vspace{1em}

\noindent\textbf{Major Revision 1 : Discuss the applications of our problem.}

As suggested by Reviewer \#3, we have revised the introduction by adding direct applications of our problem. Please refer to response to Reviewer \#3 - W2, D1 for details.

\vspace{1em}

\noindent\textbf{Major Revision 2 : Discuss the difference between open and closed social networks.}

As suggested by Reviewer \#4, we have added the detailed discussion about the difference in Section~\ref{sec:relatedwork}. Please refer to response to Reviewer \#4 - W2 for details.

\vspace{1em}

\noindent\textbf{Major Revision 3 : Improve the presentation of Section~\ref{sec:methodsingle}.}

As suggested by Reviewer \#3 and \#4, we have revised the presentation of Section~\ref{sec:methodsingle} with multiple revisions (e.g., adding more details into the proofs and intuitions and key observations for method design). Please refer to response to Reviewer \#3 - D3 and Reviewer \#4 - W1, D1, D2, D3 for details.


\vspace{1em}

\noindent\textbf{Major Revision 4 : Provide more details of deployment.}

As suggested by Reviewer \#2, we have added more details of our deployment in Section~\ref{sec:deploy}. Please refer to response to Reviewer \#2 - W1 for details.

\vspace{1em}

\noindent\textbf{Major Revision 5 : Compare efficiency of different methods.}

As suggested by Reviewer \#3, we have included Table~\ref{table:orgvsbsttime} to compare the running time of different methods. Please refer to response to Reviewer \#3 - W3, D7 for details.


\vspace{1em}
\noindent\textbf{Major Revision 6 : Change the acronyms of algorithm names.}

We remove the space among the words in all algorithms' names and thus correspondingly update the acronyms. Specifically, \method{EI} is updated to \innermethod{} for Algorithm~\ref{alg:networkaugmentationpractical} and \method{SNA} is updated to \outtermethod{} for Algorithm~\ref{alg:practicalframework}.

\vspace{1em}

\noindent \textbf{Remark}. Considering that we have added many details in multiple sections and the experiment in Section 6.1 is not primary, we have moved this part into the technical report~\cite{TR} due to space limit. Thus, the section numbers mentioned afterwards refer to the ones in the revised version unless we explicitly mention \emph{`in the original submission'} when locating the section.

\section*{Response to Meta Reviewer}

\vspace{1em}

\noindent\textbf{Meta Reviews.}
\noindent\textit{The reviewers raised some questions or mentioned some weaknesses about this work. They would recommend "revision" for the authors to address the issues. The authors are suggested to look at their reviews (weaknesses and detailed comments) and make a revision. The revision items are R2.W1, R3.D1-D7 and R4. All weaknesses and detailed points.}

\vspace{.5em}

\noindent\textbf{Response:} Thanks for your valuable suggestion. We have revised this paper according to the comments
from three reviews. All major revisions have been presented above.
Next, we will respond to all the comments from individual reviewers.

\vspace{.5em}


\section*{Response to Reviewer \#2}

\vspace{1em}

\noindent\textbf{W1.}
\noindent\textit{More details of deployment on MOBAX could be reported to show the practicality of proposed method.}

\vspace{.5em}

\noindent\textbf{Response:} Thanks for your valuable suggestion. We have added more descriptions on possible behaviors and roles of users, edge weight settings, the underlying diffusion model, how our method generates the diffusion network and why we generate this way, and why we choose Click-Through-Rate (CTR) as the evaluation metric and a discussion on other possible evaluation metrics. Please refer to Section~\ref{sec:deploy} for more details and below is a brief explanation of possible user behaviors and our choice of evaluation metric.

\smallskip
 \noindent \textbf{User behaviors}. In this activity, we do not specifically designate seeds and every user could be a potential and spontaneous seed. Specifically, users who log in the game will see this activity and may perform three possible behaviors: (1) proactively start interactions as a seed, (2) start interactions as a message receiver (i.e., a non-seed) and (3) ignore this activity.

\smallskip
\noindent \textbf{Evaluation metrics}. The number of users who interact with recommended friends directly indicates the quality of the underlying recommendation system and can effectively reflect the potential size of users who are impacted by others to perform interactions. Thus, to evaluate the performance, we adopt the Click-through Rate (CTR) which is a very popular evaluation metric for recommendation systems in industry. Despite the effectiveness of CTR, there still exist some other evaluation metrics (e.g., the actual influence spread of seeds via knowing the propagation paths and who are the seeds) worthy of explorations. However, due to the privacy restriction of this activity, we have no access to the detailed information in user logs to compute the performance under other potential metrics. In future, we would like to see how our proposed method will perform in other activities under various metrics.

\vspace{.5em}


\section*{Response to Reviewer \#3}

\vspace{1em}

\noindent\textbf{W1.}
\noindent\textit{No theoretical guarantee is provided for the result quality.}

\vspace{.5em}

\noindent\textbf{Response:} Thanks for your valuable concern. Our response below will emphasize that it is very challenging to have very efficient methods with theoretical guarantees on our problem; also, we aim for deployment into real-world applications and thus highly efficient and effective heuristic methods like our proposed \outtermethod{}  is desirable.

Studies on influence maximization in open social networks via edge insertions~\cite{d2019recommending,coro2021link,khalil2014scalable,chaoji2012recommendations,yang2019marginal,yang2020boosting} sacrifice efficiency and generality for theoretical guarantees, which is not acceptable in reality. We argue that our problem should be not easier than the aforementioned problem and ensuring the theoretical guarantees is not the first priority when deployment is considered. 

First of all, the size of candidate edges for insertion considered in this paper (i.e., all edges in the original network) is significantly larger than that in existing studies (e.g., only possible edges incident on seed nodes only) on influence maximization via edge insertions under the open sharing model. To achieve theoretical guarantees and meanwhile improve the efficiency, most (if not all) of them have to hold unrealistic assumptions (e.g., the network much be acyclic~\cite{yang2019marginal,yang2020boosting} and candidates must be incident on seeds~\cite{d2019recommending,coro2021link}) as we elaborate in Section~\ref{sec:relatedwork}. Furthermore, even with these assumptions, existing studies can still suffer from serious scalability issues (e.g., the state-of-the-art~\cite{chaoji2012recommendations}, on the problem in Section~6.1 in the original submission, is five-orders-of-magnitude slower than our methods), and some of them~\cite{yang2019marginal,yang2020boosting} did not report the running time in experiments even on very small-scale datasets (e.g., the greatest dataset in~\cite{yang2020boosting} has only 27,770 nodes and 352,807 edges). In other words, considering the very limited scalability of existing studies which consider a very small number of edge candidates and hold unrealistic assumptions, it is not reckless to claim that proposing highly efficient methods with theoretical guarantees on our problem, with a significantly much larger size of edge candidates and no strong assumptions, is very challenging. 

Second, we aim for a deployment of our proposed methods into real-world applications to benefit the society and thus high efficiency is an essential requirement for our methods. 
Third, the effectiveness of our methods is also verified in three different problems (i.e., 
maximizing the influence in \emph{open} social networks via edge insertions, 
our proposed problem \short{}, and
maximizing users' Click-trough Rate in an activity of an online Tencent application). Notably, our method can be very competitive with the state-of-the-art~\cite{chaoji2012recommendations} with theoretical guarantees in solving the problem of maximizing the influence in open social networks (see Section 6.1 in the original submission).

To summarize, we believe the methods we have proposed, although heuristic, are non-trivial technical contributions, and they are both efficient and effective in solving a real problem. 

\vspace{.5em}


\noindent \textbf{W2.}
\noindent \textit{Applications should be well argued.}

\noindent\textbf{D1.}
\noindent\textit{The problem application is not convincing. In the introduction, it is not quite clear why ``users are likely to share information with only a limited number of friend''. The paper discusses motivation and gives an example for the research problem. Some real cases/scenarios are expected to show the direct application of the problem.}

\vspace{.5em}

\noindent\textbf{Response:} Thanks for the suggestion. Besides our deployment into the real application in Section~\ref{sec:deploy}, we add two other real scenarios into the introduction. In scenario 1, users in WeChat tend to share their life moments or private matters only with their close friends and families, rather than colleagues with pure business relationships~\cite{block,block2}.
%(2) users who do not like validating existence may share information with whom they think the information is important to, without posting this information to all their friends since this message can be irrelevant to and overwhelm many users; 
In scenario 2, users who spend on online Tencent gaming events may obtain limited virtual coupons for sharing and they need to carefully choose friends to receive the coupons since people who use the coupons eventually can increase the discounts of future purchase of the coupon sender~\cite{gaming}. 

 %Note that sharing in the closed social networks does not have conflicts with that in open social networks. They complement each other and are applied in different scenarios. 
\vspace{.5em}


\noindent\textbf{D2.}
\noindent\textit{The paper should give running examples for Algorithm~\ref{alg:networkaugmentationpractical} and Algorithm~\ref{alg:fillup}.
}

\vspace{.5em}
\noindent\textbf{Response:} Thanks for the suggestions. We add Example~\ref{example:EI} and Example~\ref{example:FUR} as the running examples for Algorithm~\ref{alg:networkaugmentationpractical} in Section~\ref{sec:edgeinsertion} and Algorithm~\ref{alg:fillup} in Section~\ref{sec:augmentation} respectively.
\vspace{.5em}

\noindent\textbf{D4.}
\noindent\textit{It's better to formally define the critical edge.}

\vspace{.5em}
\noindent\textbf{Response:} Thanks for the valuable suggestion. We add Definition~\ref{defn:criticalneighborandedge} to formally define the critical edge and neighbor in Section~\ref{sec:edgeinsertion}. 
\vspace{.5em}

\noindent\textbf{D5.}
\noindent\textit{In Theorem~\ref{theorem:idealcase}, does ``lead to the optimal solution'' mean the method can produce the same result as Algorithm~\ref{alg:networkaugmentation}?}

\vspace{.5em}
\noindent\textbf{Response:} Yes, to explain this, we add more descriptions in the proof of Theorem~\ref{theorem:idealcase} and more explanation about the theorem right after the proof. Specifically, in the special case (i.e., $\forall x \in V_c, |Cr(x)| \leq min(k,N^{G}_{out}(x))- N^{G_k}_{out}(x) $) specified in Theorem~\ref{theorem:idealcase}, Algorithm~\ref{alg:networkaugmentation} will produce the optimal solution and directly inserting all critical edges will produce the same solution as that of Algorithm~\ref{alg:networkaugmentation}.
\vspace{.5em}


\noindent\textbf{D3.}
\noindent\textit{The presentation  of Section~\ref{sec:methodsingle} can be improved.}

\vspace{.5em}

\noindent\textbf{Response:} Thanks for the valuable suggestions. To improve the presentation of Section~\ref{sec:methodsingle}, we make the following major revisions:


\begin{itemize}[leftmargin=*]


\item Add a road map of Section~\ref{sec:methodsingle} right before Section~\ref{sec:edgeinsertion}.

\item Revise the description in the proof of Lemma~\ref{theorem:marginalgain}.

\item Formally define the critical neighbor and edge in Definition~\ref{defn:criticalneighborandedge}.

\item Revise the description in the proof of Theorem~\ref{theorem:critical}.

\item Revise the observation and motivation of the practical edge insertion method in the beginning of Section~\ref{sec:praticaledgeinsertion}.

\item Revise the description in the proof of Theorem~\ref{theorem:idealcase} and add more explanation of this theorem right after the proof.

\item Enrich the three key observations with more details (Observation 1, Observation 2 and Observation 3).

\item Add two running examples for Algorithm~\ref{alg:networkaugmentationpractical} and Algorithm~\ref{alg:fillup} respectively.

\item Revise some notations in Algorithm~\ref{alg:practicalframework} and Algorithm~\ref{alg:fillup}.

\item Remove the space among words in the names of all Algorithms.

\item Add an acronym for the name of Algorithm~\ref{alg:fillup}, update the acronyms for Algorithm~\ref{alg:networkaugmentationpractical} and Algorithm~\ref{alg:practicalframework}.
\end{itemize}

\vspace{.5em}


\noindent\textbf{D6.}
\noindent\textit{In terms of resulting quality, the advantage of \outtermethod{} is not obvious according to Figure~\ref{fig:diffk}.}

\vspace{.5em}

\noindent\textbf{Response:} Thanks for the comment. The advantage of \outtermethod{} is actually quite significant and we would like to emphasize that, mentioned in Section~\ref{sec:exp-closed} where we described the baselines we used, the performance of boosted baselines over their original counterparts mainly benefit from our proposed \emph{expansion} stage of \outtermethod{} (i.e., Lines 5-9 in Algorithm~\ref{alg:practicalframework}). In other words, proposing these boosted baselines is also our contribution. Next, we will explain why the advantage is significant but not visually distinguishable in Figure~\ref{fig:diffk}. 



As we mentioned in the last paragraph of `Exp3 - Effectiveness comparison with different k', the performance difference in Figure~\ref{fig:diffk} is not easy to distinguish visually due to the log scale of y axis. Furthermore, the difference between influence spread under different $k$ is much larger than that under different $|S|$ as shown in Figure~\ref{fig:diffs}, which increases the range of y axis and further makes it hard to clearly compare the performance. However, Figure~\ref{fig:diffk} is used to show the general trend of influence spread under different $k$ and the comparison among all methods has been conducted already at a finer granularity (i.e., $k=20$ and $k=30$ in Figure~\ref{fig:diffs} and Table~\ref{table:orgvsbst}). For instance, Table~\ref{table:orgvsbst} clearly reports the results of $k=30$ in Figure~\ref{fig:diffk}, and we observe that \outtermethod{} can outperform the second best performer by at least 23\%-39\% on different datasets respectively. Even though such performance gap is hard to be visualized in Figure~\ref{fig:diffk}, it is actually very significant especially compared with studies on the traditional influence maximization problem where 4\% of improvement is already significant~\cite{arora2017debunking}.


\vspace{.5em}


\noindent \textbf{W3.}
\noindent \textit{The efficiency improvement is not clear.}

\noindent\textbf{D7.}
\noindent\textit{Most techniques in the paper are designed to improve efficiency. However, only one experiment (Figure 8) is conducted to evaluate the efficiency. The paper should compare the running time of the proposed method with several baselines.}

\vspace{.5em}

\noindent\textbf{Response:} Thanks for the suggestions. Efficiency needs improvement when existing methods suffer from serious scalability issue (e.g., the state-of-the-art~\cite{chaoji2012recommendations}, in Section~6.1 of the original submission, is five-orders-of-magnitude slower than our methods). Since the recommendation system is for long-term usage, effectiveness is the first priority when methods can produce solutions within reasonable time. Thus, we did not compare the running time of different methods on our own problem because our method \outtermethod{} significantly outperforms the rest in terms of effectiveness and is highly efficient. 
%Thus, we think that it may not be so meaningful to compare their efficiency when they are far less than competitive with \outtermethod{} in terms of effectiveness. 
In the revision, we have taken the reviewer's suggestion to compare the running of our method and boosted baselines under all parameter settings. They show similar results that \outtermethod{} is very competitive with other boosted baselines in terms of running time, because all methods involve the \emph{expansion} stage of \outtermethod{} (i.e., Lines 5-9 in Algorithm~\ref{alg:practicalframework}) which dominates the total computational cost. Due to space limit, we only report the running time with $k=30$ and $|S|=50$ in Table~\ref{table:orgvsbsttime} in the main paper and please refer to the technical report~\cite{TR} for more experiment results. 

\vspace{.5em}


\section*{Response to Reviewer \#4}

\vspace{1em}
\noindent \textbf{W1.}
\noindent \textit{The presentation can be improved. There are some grammatical flaws.}

\noindent \textbf{D1.}
\noindent \textit{In algorithm 4, the font of comment is a little strange.}

\noindent \textbf{D2.}
\noindent \textit{In algorithm 4, there are subfunctions and variable names with too wide letter spacing.}

\noindent \textbf{D3.}
\noindent \textit{Section 6, "In this section, we will conduct experiments on three problems to demonstrate the robustness and effectiveness our methods", missing preposition before "our methods".}

\vspace{.5em}

\noindent\textbf{Response:} Thanks for the valuable suggestions. We have corrected them in the corresponding places and the changes are highlighted.

\vspace{.5em}


\vspace{1em}

\noindent\textbf{W2.}
\noindent\textit{In Section~\ref{sec:relatedwork}, the difference between open social network and closed social network can be described in more details. It might be better to use some examples.}

\vspace{.5em}

\noindent\textbf{Response:} Thanks for the valuable suggestion. We revise the first paragraph and add a paragraph right after that to discuss the difference in Section~\ref{sec:relatedwork}. In a nutshell, the two words `open' and `closed' are used to describe \textit{the underlying sharing model rather than the topology of the social network}. Furthermore, the sharing model applied to the network is decided based on the specific application behind. For example, if Figure~\ref{introexample} describes a subgraph of the Twitter social network, we have an open sharing model by default and a user's post will be available to all online users. On the other hand, if Figure~\ref{introexample} describes a subgraph of the Wechat social network, the closed sharing model will be applied in most cases (as in Example 1) where users will make their messages or posts visible to a limited number of selected friends. For ease of presentation and following the naming convention in this domain~\cite{naming1,naming2}, we directly use `open' and `closed' social networks to refer to the networks with the `open' and `closed' sharing models respectively.  

\vspace{.5em}


\noindent\textbf{W3.}
\noindent\textit{The features of closed social networks could be further utilized in algorithms.}

\vspace{.5em}

\noindent\textbf{Response:} Thanks for the suggestions. As per our response to W2, to our best knowledge, the only difference between open and closed social networks is the underlying sharing model. We believe that we have fully utilized the feature of the closed sharing model, which can be reflected by the two facts (presented in Section~\ref{sec:relatedwork}) that our problem formulation is drastically different from the classical influence maximization problems via node or edge selections, and existing methods cannot be trivially extended to solve our problem.

Specifically, the studies on the influence maximization problem via \emph{node selection} focus on selecting \emph{seeds} based on the open social networks where the influence from the seeds is allowed to propagate via \emph{any} edge in the network. On the other hand, in our problem, the underlying social networks are\emph{closed}, and we focus on selecting limited \emph{edges} from the original network such that the influence of \emph{specific seeds} via these \emph{selected edges} is maximized. 

The studies on the influence maximization problem via \emph{edge selection} focus on inserting a limited number of \emph{new} edges into the \emph{existing} network and assume an \emph{open-sharing} model such that the influence of the seeds will spread via all edges including the inserted ones. 
In contrast, we focus on inserting a limited number of \emph{existing} edges from the original network into an initially empty network and consider a \emph{closed-sharing} model such that the influence of seeds will spread \emph{only} via inserted edges. As a consequence, existing work's decision making of edge insertion is based on the current graph structure and cannot be trivially extended to handle our problem, because the network which requires edge insertion in our problem is initially empty. 
Additionally, due to different assumptions of the sharing model, the space of candidate edges for insertion that is considered by existing work is significantly smaller than that of our problem. As a result, most existing methods will suffer from serious scalability issue even if they could be extended via non-trivial ways to handle our problem. However, such extensions are quite infeasible due to many reasons including but not limited to the ones we elaborated at the end of Section~\ref{sec:relatedwork}.

In summary, we have tried our best to utilize the feature of closed social network to propose highly efficient and effective algorithms to solve a novel research problem which cannot be solved by the state-of-the-art on related but quite different problems.





%Thanks for the suggestions. As we respond to the previous comment, the features of closed social networks mainly lie in the underlying closed sharing model rather than the network topology. In this paper, we utilize the feature of the closed sharing model to formulate an influence maximization problem. Extensive experiments demonstrate the efficient and effectiveness of our methods, and we would like to utilize this feature to explore more advanced solutions with theoretical guarantees in future. 



==> tex/temp.tex <==

\section{Theoretical Analysis}



\begin{algorithm}[!t] 
  \algsetup{linenosize=\footnotesize}
\footnotesize
 \caption{Naive Greedy}
   \SetKwInOut{Input}{Input}
   \SetKwInOut{Output}{Output}
  \Input{The input network $G$, the target user $t$ and an integer $k$.}
  \Output{A diffusion network.}

$G_d \leftarrow $ initialize the diffusion network from $G$ where the out-neighbors of any node is not greater than $k$\;

\ForEach{ node $v \in G_d$}{
	\lIf{$N^{G_d}_{out}(v)=k$ or $N^{G}_{out}(v)$}{
		Remove edges $(v,\cdot)$ from $G$
	}
	\lElse{
			Remove edges $(v,\cdot)$ in $G_d$ from $G$
	}

}

$G_r \leftarrow G$\;

\While{$G_r$ has edges}{
	$(x,y) = \argmax_{ (u,v) \in G_r}   \delta(t)_{G_d \cup \{(u,v)\}}$\;
	Add $(x,y)$ into $G_d$; remove $(x,y)$ from $G_r$\;
	\lIf{$N^{G_d}_{out}(x)=k$}{
		Remove all edges $(x,\cdot)$ from $G_r$.
	}
	

}



\Return $G_d$\;


\end{algorithm}











\begin{algorithm}[!t] 
  \algsetup{linenosize=\footnotesize}
\footnotesize
 \caption{Dijkstra}
   \SetKwInOut{Input}{Input}
   \SetKwInOut{Output}{Output}
  \Input{The input graph $G$, the target user $t$ and influence probability dictionary $orgPr$.}

  $l \leftarrow$ the set of nodes reached by $t$ in $G_d$\;
  
  \ForEach{node $u \in l$}{ $orgPr[u]=0$ \;
       \lIf{$u=t$}{$orgPr[u]=1$ } }
  $h \leftarrow$ a max heap based on the values of $(u:orgPr(u))$ for all nodes in $l$ and $t$.
  
  \While{$h$ is not empty}{
  		$(u:orgPr(u))=h.pop()$\;
  		\ForEach{$v \in N_{out}(u)$}{
  			\If{$v$ in $h$ and $orgPr(u)* w_{(u,v)} > orgPr(v)$}{
  				$orgPr(v)=orgPr(u)* w_{(u,v)} $\;
  				update existing $(v:orgPr(v))$ in heap $h$\;
  			}		
  		}
  }
  
\end{algorithm}


\begin{algorithm}[!t] 
  \algsetup{linenosize=\footnotesize}
\footnotesize
 \caption{LocalDijkstra}
   \SetKwInOut{Input}{Input}
   \SetKwInOut{Output}{Output}
  \Input{The input graph $G$, an edge candidate $(u,v)$, the probability $orgPr(u)*w_{(u,v)}$ of the maximum probability path from $t$ to $v$ containing $(u,v)$, and influence probability dictionary $curPr$.}
  \Output{The marginal gain of $(u,v)$.}
$pr=orgPr(u)*w_{(u,v)}$ ; $gain=0$ ; $S=\emptyset$\;
  $h \leftarrow$ a max heap initialized with $(v:pr))$; $tempPr \leftarrow$ empty dictionary\;
  \While{$h$ is not empty}{
  		$(u:pr))=h.pop()$; $S=S\cup \{u\}$\;
  		$gain=gain+pr-curPr(u)$\;
  		\ForEach{$v \in N_{out}(u)$}{
  			\If{$(u,v)$ is not an inserted edge and $v \notin S$}{
  			$pr_v= v \text{ exists in } tempPr?\: tempPr(v):curPr(v)$\;
  				  			\If{$pr * w_{(u,v)} > pr_v$}{
  				  				 $tempPr(v)=pr * w_{(u,v)}$\;
  				  			    \lIf{$v$ is not in $h$}{  insert $(v:tempPr(v))$ into $h$}
  				  				\lElse{update existing $(v:tempPr(v))$ in heap $h$}
  				  				
  				  			}	
  			
  			
  			}
  			
  		}
  }
  
\end{algorithm}




\begin{algorithm}[!t] 
  \algsetup{linenosize=\footnotesize}
\footnotesize
 \caption{AutoFill}
   \SetKwInOut{Input}{Input}
   \SetKwInOut{Output}{Output}
 \Input{The input network $G$, the current diffusion network $G_d$ and an integer $k$.}

 $L \leftarrow$ nodes in $G_d$ ranking by the their subtree sizes of the spanning RMPP tree rooted by $t$.
 
 \ForEach{$v \in L$}{
 
	\ForEach{$u \in N_{in}^G(v)$}{
		\If{$u \in G_d$ and $N_{out}^{G_d}(u)<min(N_{out}^{G}(u), k)$}{
			insert $(u,v)$ into $G_d$
		
		}
	
	}
 

 }
 
 
\end{algorithm}

\begin{algorithm}[!t] 
  \algsetup{linenosize=\footnotesize}
\footnotesize
 \caption{AdvancedFill}
   \SetKwInOut{Input}{Input}
   \SetKwInOut{Output}{Output}
 \Input{The input network $G$, the current diffusion network $G_d$ and an integer $k$.}

 $L' \leftarrow$ nodes ranked by their influence probability by $t$ in $G_d$.
 
 
 
 \ForEach{$u \in L'$}{
 	$L^\# \leftarrow$ out-neighbors of $u$ ranked by their the number of edge incidence in ascending order and then subtree size in descending order. // edge incidence of $v$ refers to the number of incoming neighbors of $v$ introduced in this algorithm, initialized as 0\;
 	
 	$L^\# \leftarrow$ first $min(N_{out}^{G_r}(u), k-N_{out}^{G_d}(u) )$ nodes in $L^\#$\;
	\ForEach{$v \in L^\#$}{
	   Add $(u,v)$ into $G_d$\;
	   $Incidence[v]+=1$\;
	
	}
 

 }
 
 
\end{algorithm}




\begin{algorithm}[!t] 
  \algsetup{linenosize=\footnotesize}
\footnotesize
 \caption{DiffusionNetworkAugmentation (DNA2)}
   \SetKwInOut{Input}{Input}
   \SetKwInOut{Output}{Output}
  \Input{The input network $G$, the initial diffusion network $G_d$, the target user $t$ and an integer $k$.}
  \Output{The updated diffusion network $G_d$.}

%$G_d \leftarrow $ initialize the diffusion network from $G$ where the out-neighbors of any node is not greater than $k$\;
$G_r \leftarrow $ empty graph\;
\ForEach{ node $u \in G_d$}{
	\lIf{$N^{G_d}_{out}(u)=k$ or $N^{G}_{out}(u)$}{
		Continue
	}
	\Else{
			\ForEach{$v \in N^{G}_{out}(u)$}{
				\lIf{$(u,v) \notin G_d$ }{  Add $(u,v)$ into $G_r$}}
	}

}

 $L \leftarrow$ nodes in $G_d$ ranking by the their subtree sizes of the spanning RMPP tree rooted by $t$.

\ForEach{$v$ in $L$}{
	$u^*_v= \argmax_{u \in N^{G_r}_{in}(v)}  orgPr(u)*w_{(u,v)} $\;
	\If{$orgPr(u^*_v)*w_{(u^*_v,v)} \leq orgPr(v)$}{Continue}
	Add $(u^*_v,v)$ into $G_d$, and remove $(u^*_v,v)$ from $G_r$\;
	\If{$N^{G_d}_{out}(u^*_v)=k$}{
		Delete all edges $(u^*_v,\cdot)$ from $G_r$.
	
	}

}



\Return $G_d$\;



\end{algorithm}

\begin{algorithm}[!t] 
  \algsetup{linenosize=\footnotesize}
\footnotesize
 \caption{MultiDiffusionNetworkAugmentation (MDNA)}
   \SetKwInOut{Input}{Input}
   \SetKwInOut{Output}{Output}
  \Input{The input network $G$, the initial diffusion network $G_d$, the target user set $S$ and an integer $k$.}
  \Output{The updated diffusion network $G_d$.}

%$G_d \leftarrow $ initialize the diffusion network from $G$ where the out-neighbors of any node is not greater than $k$\;
$G_r \leftarrow $ empty graph\;
\ForEach{ node $u \in G_d$}{
	\lIf{$N^{G_d}_{out}(u)=k$ or $N^{G}_{out}(u)$}{
		Continue
	}
	\Else{
			\ForEach{$v \in N^{G}_{out}(u)$}{
				\lIf{$(u,v) \notin G_d$ }{  Add $(u,v)$ into $G_r$}}
	}

}

 $L \leftarrow$ nodes in $G_d$ ranking by the their subtree sizes of the spanning RMPP tree rooted by the ghost node $x$.

\ForEach{$v$ in $L$}{
	$u^*_v= \argmax_{u \in N^{G_r}_{in}(v)}  orgPr_x(u)*w_{(u,v)} $\;

	Add $(u^*_v,v)$ into $G_d$, and remove $(u^*_v,v)$ from $G_r$\;
	\If{$N^{G_d}_{out}(u^*_v)=k$}{
		Delete all edges $(u^*_v,\cdot)$ from $G_r$.
	
	}

}



\Return $G_d$\;



\end{algorithm}


\begin{algorithm}[!t] 
  \algsetup{linenosize=\footnotesize}
\footnotesize
 \caption{DiffusionNetworkAugmentation (DNA)}
   \SetKwInOut{Input}{Input}
   \SetKwInOut{Output}{Output}
  \Input{The input network $G$, the initial diffusion network $G_d$, the target user $t$ and an integer $k$.}
  \Output{The updated diffusion network $G_d$.}

%$G_d \leftarrow $ initialize the diffusion network from $G$ where the out-neighbors of any node is not greater than $k$\;
$G_r \leftarrow $ empty graph\;
\ForEach{ node $u \in G_d$}{
	\lIf{$N^{G_d}_{out}(u)=k$ or $N^{G}_{out}(u)$}{
		Continue
	}
	\Else{
			\ForEach{$v \in N^{G}_{out}(u)$}{
				\lIf{$(u,v) \notin G_d$ }{  Add $(u,v)$ into $G_r$}}
	}

}

Compute $u^*_v$ for every $v \in G_r$\;

\While{$G_r$ has edges}{
	$v^*=\argmax_{ v\in G_r}  \delta(t)_{G_d \cup \{ (u^*_v,v) \}}-\delta(t)_{G_d}  $\;
	Add $(u^*_{v^*},v^*)$ into $G_d$, remove all edges $(\cdot, v^*)$ from $G_r$\;
		

		\If{$N^{G_d}_{out}(u^*_v)=k$}{
			\ForEach{$x \in N^{G_d}_{out}(u^*_v)$}{
				\If{$u^*_x=u^*_v$}{
					update $u^*_x$\;
				}
			
			}
			Delete all edges $(u^*_v,\cdot)$ from $G_r$.
		
		}

}


\Return $G_d$\;


\end{algorithm}

\section{Related work}
We will introduce related work on targeted influence maximization via edge insertions and edge deletion. 

\noindent \textbf{Targeted influence maximization via edge insertions}. \citeauthor{d2019recommending}~\cite{d2019recommending} introduced the Influence Maximization with Augmentation problem
(IMA) under the IC model which aims to add a limited number of edges incident to a given set
of seeds in order to maximize influence of the seeds. \citeauthor{coro2021link}~\cite{coro2021link} extends the results of ~\cite{d2019recommending} to the LT model. They prove that the objective function under LT model is modular and leverage this property to propose an approximation algorithm. The problem studied by these two works is much simpler than ours since (1) they limit that the edges being added must be incident on the seeds which derives good theoretical properties to solve this problem and (2) there is no constraints on the number of inserted edges incident on each node ($k$ in our problem). 
\citeauthor{khalil2014scalable}~\cite{khalil2014scalable} study adding a limited number of edges to maximize influence of given seeds under LT model. Their method cannot handle IC model and does not consider the constraint of edge incidence on any node.


\citeauthor{chaoji2012recommendations}~\cite{chaoji2012recommendations} study adding edges to maximize the influence spread of seeds under the constraint that at most $k$ inserted edges are incident on any node, which is the most similar work to our problem among all study in this category. However, their proposed method cannot directly solve our equivalent problem via edge insertion since their method estimate pairwise influence via constrained paths which can only contain at most one edges being inserted. In our problem setting via edge inserting, the graph is initially empty and will only contain inserted edges after graph update. Furthermore, their method involving costly belief propagation which cannot scale to real-world social networks. 

\citeauthor{yang2019marginal}~\cite{yang2019marginal}, \citeauthor{yang2020boosting}~\cite{yang2020boosting} and \citeauthor{yu2020maximizing}~\cite{yu2020maximizing} consider adding a limited number of edges from a candidate set to maximize the influence of the seeds under the IC model. \citeauthor{yang2019marginal}~\cite{yang2019marginal}, \citeauthor{yang2020boosting}~\cite{yang2020boosting} derive lower and upper bound influence function to approximate the non-submodular influence in IC model and use a sandwich strategy to approximate the solution. \citeauthor{yang2020boosting}~\cite{yang2020boosting} derives tighter bound than \citeauthor{yang2019marginal}~\cite{yang2019marginal}. \citeauthor{yu2020maximizing}~\cite{yu2020maximizing} leverage the idea of constrained paths in~\cite{chaoji2012recommendations} to derive a submodular influence function, and then use the standard greedy to find the approximate solution. All of these three works do not consider the constraint that at most $k$ added edges can be incident on any node. Furthermore, they consider the number of edges to be added and the candidate edge set size to be quite small. However, in our problem from the perspective of edge insertion, the number of edges to be added is up to $k|V|$ and the candidate edge set consists of all edges in the original network. Furthermore, they can only work for acyclic graphs!


 

\noindent \textbf{Targeted influence maximization via edge deletion}. \citeauthor{kimura2008minimizing}~\cite{kimura2008minimizing} study removing a limited number of edges such that the average influence of all the nodes in the graph is minimized. \citeauthor{khalil2014scalable}~\cite{khalil2014scalable} study removing a limited number of edges to minimize the influence of given seeds.
\citeauthor{wang2020efficient}~\cite{wang2020efficient} study removing a set of edges to minimize the influence of given seeds to a predefined set of users. \citeauthor{medya2019influence}~\cite{medya2019influence} study a similar problem but under the credit distribution model~\cite{goyal2011data} where the influence is much more easier to be computed compared with IC and LT model. \citeauthor{nandi2016methods}~\cite{nandi2016methods} investigate the effectiveness of link removal as an intervention to minimize the spread of infections in a network. They develop four network interdiction models with different objectives and formulate these models as mixed integer linear programs. \citeauthor{pham2018maximizing}~\cite{pham2018maximizing} aim to find a
set of nodes whose removal from a social network maximizes the influence reduction from the source of misinformation within time and budget constraints.

In summary, all work in this category is different from our equivalent problem via edge deletion in two aspects: (1) the objective is different. They all aim to minimize the influence of the target seed nodes in the residue graph whereas we aim to maximize the influence. (2) constraints of the residue graph. Existing work does not have constraints on the structure of the residue graph whereas we require that each node in the residue graph can have at most $k$ out neighbors.

==> tex/visualization.tex <==
\begin{figure*}[!t]


\subfloat[Hamster]{
\includegraphics[width=0.5\textwidth]{./figures2/Hamster_distance.png}
}
\subfloat[Instagram]{
\includegraphics[width=0.5\textwidth]{./figures2/Instagram_distance.png}
}







\caption{Visualization of pricing schemes FCInf-Greedy and FCMWS-Greedy.}\label{effect:visualization}
\vspace{-0.36cm}
\end{figure*}
